Algorithms for reconstruction over single and multiple deletion channels

Recent advances in DNA sequencing technology and DNA storage systems have rekindled the interest in deletion channels. Multiple recent works have looked at variants of sequence reconstruction over a single and over multiple deletion channels, a notoriously difficult problem due to its highly combinatorial nature. Although works in theoretical computer science have provided algorithms which guarantee perfect reconstruction with multiple independent observations from the deletion channel, they are only applicable in the large blocklength regime and more restrictively, when the number of observations is also large. Indeed, with only a few observations, perfect reconstruction of the input sequence may not even be possible in most cases. In such situations, maximum likelihood (ML) and maximum aposteriori (MAP) estimates for the deletion channels are natural questions that arise and these have remained open to the best of our knowledge. In this work, we take steps to answer the two aforementioned questions. Specifically: 1. We show that solving for the ML estimate over the single deletion channel (which can be cast as a discrete optimization problem) is equivalent to solving its relaxation, a continuous optimization problem; 2. We exactly compute the symbolwise posterior distributions (under some assumptions on the priors) for both the single as well as multiple deletion channels. As part of our contributions, we also introduce tools to visualize and analyze error events, which we believe could be useful in other related problems concerning deletion channels.

==> Sections/OLD/intro_Oct11.tex <==


\section{Introduction}
\label{sec:intro}



Sequence reconstruction over deletion channels, both with and without a codebook, has received considerable attention in the information theory as well as in the theoretical computer science literature. From an information theory perspective, reconstruction over the deletion channel, or more specifically a  maximum-likelihood (ML) argument for the deletion channel, would give further insight on the capacity of the deletion channel, a long-standing open problem (see \cite{mitzenmacher2009survey}). To quote \cite{mitzenmacher2009survey} -- ``at the very least, progress in this direction would likely surpass previous results on the capacity of the deletion channels''. Yet, there are no results on reconstruction over a deletion channel with statistical guarantees -- in this work, we take a step in this direction.

On the other hand, the problem of \textit{trace reconstruction}, as introduced in \cite{Batu2004}, has received renewed interest in the past few years (see \cite{Holenstein2008}, \cite{Peres2017}, \cite{De2017}, \cite{holden18}, \cite{Nazarov:2017}, \cite{holden2018lower}, \cite{chase2019new}). The problem of trace reconstruction can be stated simply as follows: consider a sequence $X$ which is simultaneously passed through $t$ independent deletion channels to yield $t$ deleted observations (also called \textit{traces}) of $X$ (see Fig.~\ref{fig:tdeletion}). How many such traces are needed to reconstruct $X$ perfectly? A variety of upper and lower bounds for this problem have been proposed, both for worst case and average case reconstruction. Our problem definition, stated in the following paragraph, is closely related to the average case trace reconstruction.
 
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.2]{tdeletion.pdf}
\caption{$t$-deletion channel model:  sequence $X$ passed through $t$ independent deletion channels to yield $t$ \textit{traces}. We aim to estimate $X$ from the $Y^{(i)}$s.}
\label{fig:tdeletion}
\end{center}
\end{figure}
 
\noindent \textbf{Problem definition.}  Given an input sequence of length $n$ (known apriori), the independently and identically distributed (i.i.d.) deletion channel deletes each input symbol indepedently with probability $\delta$, producing at its output a subsequence of the input sequence. Consider a sequence $X$ passed through $t$ ($t$ is fixed) such deletion
channels as shown in
Fig.~\ref{fig:tdeletion}. We call this the $t$-deletion channel model. We ask two questions:
\begin{enumerate}
\item For $t=1$ (see Fig.~\ref{fig:1deletion}, also called the single deletion channel model), and when $X_i \sim\ \text{ind. Ber}(p_i)$, compute the posterior distributions of $X_i$ given the trace $Y$.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.25]{1deletion.pdf}
\caption{The single deletion channel model. We assume $X_i \sim\ \text{ind. Ber}(p_i)$.}
\label{fig:1deletion}
\end{center}
\end{figure}
\item In the $t$ deletion channel model, for a fixed $t$ assume that $X_i \sim\ \text{i.i.d. Ber}(0.5)$ and compute the posterior distributions of $X_i$ given all traces $Y^{(1)}, Y^{(2)},...,Y^{(t)}$. 
\end{enumerate}
Note that solving 1) above doesn't lead to a natural solution for 2). This is because for a memoryless channel, we have $Y^{(j)} - X_i - Y^{(k)}$ and hence $\Pr(X_i=\alpha|Y^{(j)}, Y^{(k)}) \propto \Pr(X_i=\alpha|Y^{(j)}) \Pr(X_i=\alpha|Y^{(k)})$; so one could independently combine the posterior probabilities from each noisy observation. This is not the case for deletion channels since the markov chain $Y^{(j)} - X_i - Y^{(k)}$ no longer holds. More intuitively, one needs to first ``align'' the traces for computing the likelihoods. 
%, where every channel independently deletes each bit with probability $\delta$.


We point out that the problem considered in 2) asks a question complementary to the trace reconstruction: given a fixed (possibly a few) number of traces, what is our ``best'' guess of $X$? We provide algorithms which do this. Unlike trace reconstruction, we are not concerned with perfect reconstruction (since perfect reconstruction may not be possible with just a few traces), although it should also be obvious that performance guarantees for our algorithms (not a part of this work) would naturally lead to upper bounds for trace reconstruction.

Deletion channel by itself is known to be notoriously difficult to analyse. As stated earlier, the capacity of a single deletion channel is still unknown (\cite{diggavi2007capacity,diggavi2006information,diggavi2001transmission}); as are optimal coding schemes. Recent works have looked at the design of codes for deletion channels (\cite{ratzer2005marker,ratzer2000codes,thomas2017polar}); these works consider use of a codebook (we do not). As a result, statistical estimation over deletion channels is also a difficult problem due its highly combinatorial nature. To the best of our knowledge, as yet there are no efficient estimation algorithms over deletion channels with statistical guarantees; not even for ML over a single deletion channel.


\noindent \textbf{Biological motivation.} Trace reconstruction in itself was motivated, in part, by problems DNA sequence reconstruction. One such problem was to infer the DNA sequence of a common ancestor from the samples of its descendants. We argue that our problem definition fits more naturally in such a scenario since perfect reconstruction may not be feasible or even possible. Our motivation for considering this problem also comes from a recent DNA sequencing technology called \textit{nanopore sequencing}. The $t$-deletion channel model is a simplistic model to approximately capture the process of a DNA sequence passed through a nanopore sequencer\footnote{As seen in
  \cite{Mao2017},\cite{MDK17} there are more complicated effects of
  the nanopore reader not captured in this simple 
  representation.}.  
  
Very recently, a variant of the trace reconstruction problem called \textit{coded trace reconstruction} has been proposed, motivated by portable DNA-based data storage systems using DNA nanopores (see \cite{abroshan2019coding}, \cite{cheraghchi2019coded}, \cite{brakensiek2019coded}) and we believe that the ideas in this work may prove useful in such a setting.

There are other works on sequence assembly (see for example, \cite{Li09fastand}, \cite{Shomorony2016}),
where multiple short reads (from different segments of a sequence) are used to reconstruct the bigger
sequence. This work differs from sequence assembly since we are interested to infer the entire length sequence and not  just small segments of it (which are then ``stitched'' together in sequence assembly).

\noindent \textbf{Tools and techniques.} In terms of theoretical tools, the series of books by Lothaire (\cite{lothaire1997combinatorics,lothaire2002algebraic,lothaire2005applied}) extensively use algebraic tools  for problems in the combinatorics of sequences (or \textit{words}), and our work is inspired by such techniques. We borrow many of their notations and results for our work.


\noindent \textbf{Contributions.} {\color{red}} Our main contribution is to provide tools to visualize and analyze error events (described in the next section) for the multiple deletion channel model in Fig.~\ref{fig:tdeletion}. We also provide algorithms to solve the problems stated in 1) and 2) earlier in the section.
\begin{itemize}[wide=5pt]
\item In section~\ref{sec:1deletion}, for the single deletion channel model, we provide an  $O(n^2)$  algorithm to calculate the symbolwise posterior probabilities  $\Pr(X_i=1|Y)\ \forall\ i$ when $X_i \sim \text{ind. Ber}(p_i)$.
 \item  In Section~\ref{sec:exactsmap}, for the $t$-deletion channel model, we give an $O(2^t n^{t+2})$ algorithm to calculate the symbolwise posterior probabilities $\Pr(X_i = 1|Y_1,...,Y_t)$ when $X_i \sim \text{ind. Ber}(0.5)$.
\end{itemize}





==> Sections/OLD/notation_Oct12.tex <==

\section{Notation and Tools}
\label{sec:notations}
\noindent \textbf{Basic notations:} In this work, we borrow a majority of the notation and tools from \cite{lothaire1997combinatorics} which deals with non-commutative algebra. We restate the definitions here for convenience. Calligraphic letters refer to sets, capitalized letters
correspond to random variables and bold letters are used for functions.  Let $\mathcal{A}$ be the set of all
symbols. Throughout this work, we will focus on the case where $\mathcal{A}=\{0,1\}$,
though  our methods extend to arbitrarily large sets of finite size. Define
$\mathcal{A}^n$ to be the set of all $n$-length sequences and $\mathcal{A}^*$ to be the set of all finite length sequences with
symbols in $\mathcal{A}$. For a sequence $f$, $|f|$ denotes the length
of $f$. For integers $i,j$, we define $[i:j] \triangleq \{i,i+1,...,j\}$ if $j\geq i$ and $[i:j] \triangleq \emptyset$ otherwise. Also define $[i] \triangleq [1:i]$.\\

\noindent \textbf{Binomial coefficient:} Given sequences $f$ and $g$ in $\mathcal{A}^*$, the number of
subsequence patterns of $f$ that are equal to $g$ is called the
\textit{binomial coefficient} of $g$ in $f$ and is denoted by $f
\choose g$.  For example, ${'apple' \choose 'ape'} = 2$ since $'ape'$ can be obtained from two (overlapping) subsequences of $'apple'$.


When the alphabet $\mathcal{A}$ is of cardinality 1, ${f
  \choose g} = {|f| \choose |g|}$, the classical binomial coefficient
with their respective lengths as the parameters. This definition hence
could be thought of as a generalization of the classical binomial
coefficients. We will denote by $e$ the sequence of length 0, and {define ${f
  \choose e} \triangleq 1\ \forall\ f\ \in\ \mathcal{A}^*$.} We also define the classical binomial coefficient ${a \choose b}\triangleq 0,$ whenever $b>a$ or $b<0$ for ease of use.

The binomial coefficient is an integral aspect of this work and for analyzing error events in deletion channels because the input-output relation for a deletion channel (with deletion probability $\delta$, input $X$ and output $Y$) can be expressed as 
\begin{equation}
\label{eq:in-out_relation}
\Pr(Y=y|X=x) = {x \choose y} \delta^{|x|-|y|} (1-\delta)^{|y|}.
\end{equation}
The proof is straight-forward -- the number of distinct error events that give rise to $y$ from $x$ is exactly the number of  subsequences of $x$ which are equal to $y$. Each of these error events has a probability $\delta^{|x|-|y|} (1-\delta)^{|y|}$, wherein the exponent of $\delta$ corresponds to the deleted symbols and the exponent of  $1-\delta$ to the undeleted symbols. 

Given the definition of the binomial coefficient, the maximum-likelihood (ML) estimate over a deletion channel with observed output $Y$ can be cast in the following form:
\begin{align*}
\argmax_{x \in \mathcal C}  {x \choose Y},\numberthis
\label{eq:ML_deletion}
\end{align*}
where $\mathcal C$ is the chosen codebook. In the case of multiple deletion channels with observed traces $Y^{(1)},...,Y^{(t)}$, the ML formulation is similar:
\begin{align*}
\argmax_{x \in \mathcal C}  \prod_{j=1}^{t} {x \choose Y^{(j)}}.\numberthis
\label{eq:ML_multiple_deletion}
\end{align*}
As yet, there is no known efficient way to come up with a solution for the above two formulations, even for \eqref{eq:ML_deletion} with $\mathcal C = \{0,1\}^n$ (see \cite{mitzenmacher2009survey}). In this work, we attempt to take a step in this direction by showing that a continuous relaxation of \eqref{eq:ML_deletion} is equivalent to \eqref{eq:ML_deletion}. However, an efficient algorithm to solve the optimization \eqref{eq:ML_deletion} remains open. In the context of trace reconstruction, the ultimate pursuit would be an algorithm for \eqref{eq:ML_multiple_deletion} with $\mathcal C = \{0,1\}^n$ and error analysis thereof.


\noindent We now describe a function which can be thought of as a real-valued extension of the binomial coefficient. This function is used in sections~\ref{sec:1deletion_ML} and \ref{sec:1deletion}. Consider the function $\mathbf F(\cdot)$ defined as:
\begin{definition}
\label{def:f}
\begin{align*}
&\mathbf F: \mathbb{R}^k \times \{0,1\}^l \rightarrow \mathbb{R},\\
\mathbf F(q,  v)\triangleq &\begin{cases} 
      \sum\limits_{\substack{\mathcal S|\mathcal S\subseteq [k],\\|\mathcal S|=l}} \quad \prod\limits_{i=1}^l q_{\mathcal S_i}^{v_i} (1-q_{\mathcal S_i})^{1-v_i} & 1 \leq l\leq k \\
	  1 &  0=l\leq k \\
      0 & \text{else}.  
   \end{cases}
\end{align*}
\noindent An alternate definition is as follows: consider a random vector $Z\in\{0,1\}^k$ such that $Z_i\sim$ ind. Ber$(q_i)$, let $q$ be the vector of probabilities of length $k$, $\mathcal S\subseteq [k]$ a subset of the indices of size $l$, and ${v}$ a binary vector of length $l$. Then, $$\mathbf F(q,v)=\sum_{\substack{\mathcal S||\mathcal S|=l}} \Pr(Z_{\mathcal S}= v).$$ Note that if $q$ is a vector of $0$'s and $1$'s, then $\mathbf F( q,  v)={q \choose v}$, the binomial coefficient of $v$ in $q$. Thus, $\mathbf F(\cdot)$ could be interpreted as an extension of the binomial coefficient where one of the parameters can take values in $[0,1]^n$ instead of $\{0,1\}^n$.
\end{definition}
Though at first sight, $\mathbf F(q,v)$ sums over an exponential number of subsets, a dynamic programming approach can be used to compute it in $O(|v|^2)$ time complexity. The dynamic program is described in section~\ref{sec:1deletion}.

\iffalse
%\subsection{Definitions and preliminary results}
\noindent \textbf{Edit distance:} The edit distance  $d_e(f,g)$  measures similarity between two sequences of
possibly different lengths \cite{Navarro2001}. $d_e(f,g)$ is the minimum number of operations
needed to transform $f$ to $g$, where the permitted operations are
insertion, deletion or substitution of a symbol. In this work, we
quantify the performance of algorithms in Section \ref{sec:Numerics}
using the edit distance metric.

\fi

The following definitions and ideas are relevant only for \ref{sec:exactsmap} and can be omitted  for the sections on single deletion channel. Before getting to the mathematical definitions, we first state a result of ours that aids in thinking about error events in multiple deletion channels. 

\subsection{An alternate interpretation of multiple deletion channel model}

The events occurring in the $t$-deletion channel model can be categorized into two groups:
\begin{enumerate}
\item an input symbol is deleted in \textit{all} the $t$-traces,
\item an input symbol is reflected in at least one of the traces.
\end{enumerate}
The error events of the first kind are in some sense ``not correctable" or even ``detectable" since it is impossible to tell what and where the deleted symbol could have been (although the probabilities need not be uniform). The events of the second kind, however, can still be detected although they could likely be confused with a large set of similar events. This thought process gives rise to a natural decomposition of the $t$-deletion channel model into a cascade of two channels: the first one being a deletion channel which captures error events of the first kind and the second one is what we call the \textit{remnant channel} which captures events of the second kind (see Fig.~\ref{fig:channel_equiv}). More precisely, the remnant channel is defined as follows:
\begin{definition}
\textit{Remnant channel:} an input symbol to the remnant channel is reflected in $k>0$ given outputs and deleted in the rest with a probability $\frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}$. 
\end{definition}
It is easy to note that probability of the union of all possible events here is $\sum_{k=1}^t {t \choose k} \frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}=1$, validating our definition.

\begin{restatable}{theorem}{channelequiv}
\label{thm:channel_equiv}
The $t$-deletion channel model and the cascade of the deletion channel with remnant channel shown in Fig.~\ref{fig:channel_equiv} are probabilistically equivalent, i.e., 
$$\Pr({Y}^{(1)},{Y}^{(2)},...,{Y}^{(t)}|X = x) = \Pr(\tilde{Y}^{(1)},\tilde{Y}^{(2)},...,\tilde{Y}^{(t)}|X = x).$$
\end{restatable}
The formal proof of the theorem requires few more definitions and is relegated to the appendix.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.4]{channel_equiv.pdf}
\caption{A channel equivalence result: the $t$-deletion channel model in (a) is probabilistically equivalent to the the cascade of a deletion channel with the \textit{remnant channel} ($ \mathcal C_2$) in (b).}
\label{fig:channel_equiv}
\end{center}
\end{figure}




\noindent\textbf{Edit graph} (as defined in \cite{Gusfield1997}): We now define a graph construct which is closely related to  the error events in the remnant channel. We start with a simple case and generalize subsequently. Define an \textit{edit graph} given two sequences $f$ and $g$, where every path connecting the ``origin'' to the ``destination'' on the edit graph yields a supersequence $h$ of $f,g$, where $h$ is ``covered'' by $f,g$ -- i.e.,  each symbol of $h$ comes from either $f$ or $g$ or
both. In other words, given that $f$ and $g$ are the outputs of the remnant channel (with two outputs), each path from the origin of the edit graph to the destination corresponds to a possible input $h$ to the remnant channel and to an error event  which resulted in $f$ and $g$ with  input $h$.


For $f$ and $g$ in $\mathcal
A^*$, we form a graph $\mathcal{G}(f,g)$ with $(|f|+1)(|g|+1)$
vertices each labelled with a distinct pair $(i,j), 0\leq i\leq
|f|,\ 0\leq j\leq |g|$. A directed edge
$(i_1,j_1)\rightarrow(i_2,j_2)$ exists iff at least one of the following
holds: 
%\vspace{-1mm}
\begin{enumerate}
\item$i_2-i_1=1$ and $j_1=j_2$, or
\item $j_2-j_1=1$ and $i_1=i_2$, or
\item  $i_2-i_1=1$, $j_2-j_1=1$ and $f_{i_2}=g_{j_2}$, 
\end{enumerate}
%\vspace{-1mm}
where $f_i$ is the $i^{th}$ symbol of the sequence $f$. The origin is the vertex $(0,0)$ and the destination $(|f|,|g|)$.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap1.pdf}
\caption{ Edit graph for sequences $f=$ `001' and $g=$ `101'. An easy way to think about this is to write down $f$ vertically with each symbol aligned to a vertical set of edges and $g$ horizontally likewise. A diagonal edge in a small square exists if the corresponding $f$ and $g$ symbols are equal. The thick red edges form a path from the origin to the destination; this path corresponds to the sequence `0101' -- append the corresponding symbol at the left of an edge if it's vertical or diagonal, otherwise append the symbol at the top. It is also easy to verify that 0101 is a supersequence of both $f$ and $g$, and could be obtained as a covering of $f$ and $g$; the path itself gives one such covering. This covering also corresponds to an error event in the remnant channel which would result in outputs $f$ and $g$ with input $h=$ `0101' -- more precisely, the error event is one in which the first symbol of $h$ is deleted only in $g$, the second symbol is deleted only in $f$ and the third and fourth symbols not deleted in either $f$ or $g$.}
\label{fig:editgraph_smap1}
\end{figure}

Let $p=((i_1,j_1),(i_2,j_2),...,(i_m,j_m))$ be a path in $\mathcal{G}(f,g)$. We define $ s(p)$ to be the sequence corresponding to the path. Intuitively, $s(p)$ is formed by appending symbols in the following
way: append the corresponding $f$ symbol for a vertical edge, $g$ symbol for horizontal edge, and $f$ or $g$ symbol for  diagonal edge (see example Fig.~\ref{fig:editgraph_smap1}). Any path from $(0,0)$ to $(|f|,|g|)$ corresponds to a supersequence of $f$ and $g$ and which is ``covered" by $f$ and $g$. More formally, define $ s(p)\triangleq x_1x_2...x_{m-1}$ where    
$$x_k = 
     \begin{cases}
       f_{i_{k+1}} \quad\text{if }j_{k}=j_{k+1},\\ 
       g_{j_{k+1}} \quad\text{if }i_{k}=i_{k+1},\\
       f_{i_{k+1}} \quad\text{else.}
    \end{cases}	
$$


The construct of edit graph can be extended to more than 2 sequences with the same idea. For sequences $f_1,f_2,...,f_t$, construct a $t$-dimensional grid with a number of vertices $(|f_1|+1)(|f_2|+1)...(|f_t|+1)$ labeled from $(0,0,...,0)$ to $(|f_1|,|f_2|,...,|f_t|)$. A vertex $u=(i_1,i_2,...,i_t)$ is connected to $v=(j_1,j_2,...,j_t)$ (we say $u \rightarrow v$) iff both of the following conditions are met:
\begin{itemize}
\item $j_l=i_l$ or $j_l=i_l+1$ $\forall\ l\in [t]$, i.e., $(i_1,...,i_t)$ and $(j_1,...,j_t)$ are vertices of a particular unit cube. Only these type of vertices can share an edge in the grid graph.
\item Let $\mathcal T \subseteq [t]$ be the collection of indices where $j_l=i_l+1$. Then $f_{i_l}$ is same $\forall\ l \in \mathcal T$. For instance, if $\mathcal T=\{1,3,5\}$, then $f_{i_1}=f_{i_3}=f_{i_5}$.
\end{itemize}
Define the vertex $(0,...,0)$ to be the origin of this graph and the vertex $(|f_1|,...,|f_t|)$ to be the destination. If $|f_j|=O(n)\ \forall\ j$, this graph has a number of vertices $O(n^t)$ and a maximum number of edges $O((2n)^t)$ since each vertex has at most $2^t$ outgoing edges.\\


\noindent\textbf{Infiltration product} (introduced in \cite{lothaire1997combinatorics}):
The infiltration product has been extensively used in \cite{lothaire1997combinatorics}, as a tool in non-commutative algebra. Here we give an edit-graph interpretation of this tool. We also give a formal definition later in this section. Using the edit graph we can construct the set of possible
supersequences $\mathcal{S}(f,g)$ of $f,g$ which are covered by
it. Clearly multiple paths could yield the same supersequence and we
can count the number of distinct ways  $\mathbf N(h;f,g)$ one can construct
the same supersequence $h$ from $f,g$.
We can  informally define the
\emph{infiltration product $f\uparrow g$} of $f$ and $g$, as a polynomial with monomials the supersequences $h$ in
$\mathcal{S}(f,g)$ and coefficients  $\langle f\uparrow g,h\rangle$ equal to $\mathbf N(h;f,g)$. In Fig.~\ref{fig:editgraph_smap1}, it is easy to verify that there is exactly one path corresponding to `101001' and hence $\langle 001\uparrow 101,101001 \rangle=1$ and similarly $\langle 001\uparrow 101,01001 \rangle=2$. One could find these coefficients for all relevant sequences and form the polynomial as described. More examples: Let $\mathcal{A}=\{a,b\}$, then
 %\vspace{-7pt}
\begin{itemize}[wide=2pt]
\item $ab\uparrow ab=ab+2aab+2abb+4aabb+2abab$,
\item $ab\uparrow ba=aba+bab+abab+2abba+2baab+baba.$
\end{itemize}
The  infiltration operation is commutative and associative, and infiltration of two sequences $f\uparrow g$ is a polynomial with variables of length (or \textit{degree}) at most $|f|+|g|$; see \cite{lothaire1997combinatorics}.
The definition of infiltration extends to two polynomials via distributivity (precisely defined in later), and consequently to multiple sequences as well. For multiple sequences, infiltration has the same edit graph interpretation: $\langle f_1\uparrow f_2 \uparrow...\uparrow f_t, w \rangle$ is the number of distinct ways of constructing $w$ as a supersequence of $f_1, f_2, ... ,f_t$ so that the construction covers $w$, i.e., construct the $t$-dimensional edit graph of $f_1, f_2, ... ,f_t$ and count the number of paths corresponding to $w$.

\subsection{Formal definition of infiltration product}
 We now give a more formal definition of the infiltration product (see \cite{lothaire1997combinatorics} for the equivalence of the two definitions and a more rigorous treatment). A \textit{formal series} with indeterminates (or variables) in a set $\mathcal A$ and coefficients in a commutative ring $\mathcal R$, is a mapping of $\mathcal A^*$ onto $\mathcal R$. Recall that a commutative ring is a set which forms an abelian group under an \textit{addition} operation, is a monoid under a \textit{multiplication} operation which commutes, and the multiplication operation distributes over addition. Here we consider $\mathbb Z$, the set of integers as the commutative ring  $\mathcal{R}$. A formal series is called a \textit{polynomial} if only a finite number of sequences are mapped to non-zero values, the rest of the sequences map to zero. Consider two polynomials $\sigma,\tau: \mathcal{A}^*\rightarrow \mathbb Z$. The value taken by a sequence $w\in \mathcal A^*$ on $\sigma$ (or the coefficient of $w$ in $\sigma$) is denoted by $\langle \sigma,w\rangle \in \mathbb R$. We also define binary addition ($\oplus$) and multiplication operations ($\times$) on the set of polynomials as follows:
\begin{align}
\langle \sigma\oplus \tau,w\rangle \triangleq \langle \sigma,w\rangle +  \langle \tau,w \rangle \quad \forall w\in \mathcal A^*,\label{eq:polynomial_add}\\
\langle \sigma\times \tau,w\rangle \triangleq \sum_{\substack{f,g\in \mathcal A^*:\\ f.g=w}}\langle \sigma,f\rangle  \langle \tau,g \rangle \quad \forall w\in \mathcal A^*.\label{eq:polynomial_prod}
\end{align}
We will use the usual symbols $+$ and $.$ in place of $\oplus$ and $\times$ in this work for convenience. The meaning of the operation would be clear depending on the operands. With these operations the set of polynomials form a non-commutative ring, and is denoted by $\mathbb Z\langle\mathcal A \rangle$, also called the free $\mathbb Z$-algebra on $\mathcal A$ in ring theory. Note that the addition and multiplication operations defined in \eqref{eq:polynomial_add} and \eqref{eq:polynomial_prod} are similar to the operations defined on commutative polynomials, except that the multiplication  operation under the summation in \eqref{eq:polynomial_prod} ($f.g=w$) is actually concatenation and is non-commutative.   The multiplication inside the summation in \eqref{eq:polynomial_prod} is multiplication in the real field and hence commutative. It is also easy to prove that the multiplication defined in \eqref{eq:polynomial_prod} distributes over addition defined in \eqref{eq:polynomial_add}. Thus, a polynomial in $\mathbb Z\langle\mathcal A \rangle$ can be represented as a sum of monomials in $\mathcal A^*$ each with an associated coefficient in $\mathbb Z$, i.e., $\sigma=\sum\limits_{w\in \mathcal A^*} \langle\sigma,w \rangle w$. Define the \textit{degree} of a polynomial to be equal to the length of a longest sequence with a non-zero coefficient in the polynomial and the \textit{number of terms} of a polynomial as the number of sequences with non-zero coefficients in the polynomial. Note that a degree $d$ polynomial could have a number of terms upto $2^{d+1}-1$.
 
With this, the \textit{infiltration product} (in general, for two polynomials) is defined as follows:

\begin{align}
\forall f\in \mathcal{A}^*,& \quad f\uparrow e = e\uparrow f=f.\nonumber \\
\forall f,g\in \mathcal{A}^*&,\quad  \forall a,b\in \mathcal{A}, \nonumber\\
fa\uparrow gb=(f\uparrow gb)a&+(fa\uparrow g)b+\mathbbm{1}_{a=b}(f\uparrow g)a.\nonumber \\
\forall \sigma,\tau \in \mathbb{Z}\langle\mathcal{A} \rangle, \quad &\sigma\uparrow \tau=\sum_{f,g\in \mathcal{A}^*} \langle \sigma,f \rangle \langle \tau,g \rangle (f\uparrow g). \label{def:infiltforseq}
\end{align}

%Note that infiltration is defined, in general, for two series, not just for two sequences.

\textbf{Summary of definitions and ideas introduced in this section:}
\begin{itemize}
\item The binomial coefficient captures the likelihood of observations for deletion channels. 
\item An extension of the binomial coefficient function where one of the parameters can take real values has been introduced; this function is pivotal for our results on the single-trace deletion channel.
\item For multiple deletion channels, the error events can be categorized into two groups -- one where an input symbol is deleted in all the traces, and second, the complement of this event. This categorization results in a natural decomposition of multiple deletion channel model into a cascade model involving the remnant channel.
\item The remnant channel disregards the error events where a symbol is deleted in all the traces.
\item The edit graph provides a way to visualize all the possible error events and input sequences to a remnant channel given its outputs. 
\item The infiltration product serves the same purpose as the edit graph, but has an algebraic flavor and provides rigor for proofs and analyses. The edit graph, on the other hand, is more helpful in designing reconstruction algorithms over deletion channels.
\end{itemize}



==> Sections/OLD/single_ML_Oct12.tex <==


\section{Maximum likelihood for the single-trace deletion channel}
\label{sec:1deletion_ML}
Consider the ML formulation for the single-trace deletion channel given non-empty trace $Y$ and all possible $n$-length inputs allowed, restated here for convenience:
\begin{equation}
\argmax_{x\in \{0,1\}^n} {x \choose Y}.
\label{eq:1deletion_ML}
\end{equation}
To the best of our knowledge, the only known method to solve \eqref{eq:1deletion_ML} involves iterating over all possible choices of $x$ and computing the objective value for each of the choices. We here show that it is sufficient to solve a continuous relaxation of above problem to obtain a solution to \eqref{eq:1deletion_ML}. Note that there could be multiple solutions to \eqref{eq:1deletion_ML}. Before going in the main result, we first state a useful lemma which factors out a given coordinate $p_i$ out of $\mathbf F(p,Y)$. The proof of the lemma is relegated to the appendix.
\begin{restatable}{lemma}{deletionMLrellemma}
For $p=[p_1,p_2,..,p_i,...,p_n]$ and $Y=Y_1Y_2...Y_m$ with $n \geq m > 0$, we have
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
\label{lemma:F_decomposition}
\end{restatable}


\begin{theorem} An alternative optimization to characterize ML for the single-trace deletion channel.
\begin{equation}
\max_{x\in \{0,1\}^n} {x \choose Y} = \max_{p\in [0,1]^n} \mathbf F(p,Y).
\label{eq:ml_opt_equiv}
\end{equation}
Furthermore, given any non-integral $p^* \in [0,1]^n$ that maximizes $\mathbf F(p,Y)$, one could construct a corresponding integral solution $x^* \in \{0,1\}^n$ that maximizes $\mathbf F(p,Y)$ and consequently is also a solution to $\max_{x\in \{0,1\}^n} {x \choose Y}$.

\end{theorem}
\begin{proof}
As noted earlier, we have ${x \choose Y} = \mathbf F(x,Y)$. Therefore, we are interested in proving the following:
\begin{align*}
\max_{x\in \{0,1\}^n} \mathbf F(x,Y) \equiv \max_{p\in [0,1]^n} \mathbf F(p,Y).\numberthis
\label{eq:ml_opt_equiv_proof1}
\end{align*}
To show this and also the second statement, we prove that given $p=(p_1,p_2,...,p_i,...,p_n)$, at least one of the following holds true:
\begin{itemize}
\item$\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},0,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 0.
\item $\mathbf F(p^{(i\rightarrow 1)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},1,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 1.
\end{itemize}
Thus if $p^*$ is an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ with $p_i\in (0,1)$, then at least one of $p^{(i\rightarrow 0)}$ or $p^{(i\rightarrow 1)}$ is also an optimal solution. Sequentially applying this argument for each coordinate of $p$ shows that there exists a point in $\{0,1\}^n$ which is also an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ and consequently to $\max_{x\in \{0,1\}^n} \mathbf F(x,Y)$.

Now to prove our claim, we use Lemma~\ref{lemma:F_decomposition} to factor out $p_i$ terms in $\mathbf F(p,Y)$:
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
There are 3 cases
\begin{enumerate}
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) = \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) = \mathbf F(p,Y) = \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) > \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \leq \mathbf F(p,Y) \leq \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) < \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y) \geq \mathbf F(p^{(i\rightarrow 1)},Y).$
\end{enumerate}
Thus in each of the 3 cases, we see that at least one of $\mathbf F(p^{(i\rightarrow 0)},Y)$ or $\mathbf F(p^{(i\rightarrow 1)},Y)$ is at least as large as $\mathbf F(p,Y)$ thus proving the theorem. Note that the proof gives a natural way to find an optimal lattice point $p_{lattice}^*$ given a non-lattice point $p^*$ by iterating through each coordinate of $p^*$ and switching them to $0$ or $1$ by comparing $\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})$ with $\sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$
\end{proof}


==> Sections/conclusions.tex <==

\section{Conclusions}

\label{sec:conclusions}
In this work we gave, to the best of our knowledge, the first results and techniques to compute posterior distributions over single and multiple deletion channels. We also provided a new perspective on the maximum-likelihood for the deletion channel by showing an equivalence between a discrete optimization problem and its relaxed version. In this process, we introduced a variety of tools (the relaxed binomial coefficient, edit graph and infiltration product) and demonstrated their use for analyzing deletion channels.  We also presented numerical evaluations of our algorithms.

%These tools could prove their use in other closely related problems concerning deletion channels (design of codes, trace reconstruction to name a few).


==> Sections/intro.tex <==


\section{Introduction}
\label{sec:intro}

Sequence reconstruction over deletion channels, both with and without a codebook, has received considerable attention in the information theory as well as in the theoretical computer science literature. From an information theory perspective, reconstruction over the deletion channel, or more specifically a  maximum-likelihood (ML) argument for the deletion channel, would give further insight on the capacity of the deletion channel, a long-standing open problem (see \cite{mitzenmacher2009survey}). To quote \cite{mitzenmacher2009survey} -- ``at the very least, progress in this direction would likely surpass previous results on the capacity of the deletion channels''. Yet, there are no results on reconstruction over a deletion channel with statistical guarantees. In this work, we take steps in this direction.

In this space, the problem of \textit{trace reconstruction}, as introduced in \cite{Batu2004}, has also received renewed interest in the past few years (see \cite{Holenstein2008,Peres2017}, \cite{De2017}, \cite{holden18}, \cite{Nazarov:2017}, \cite{holden2018lower}, \cite{chase2019new}). The problem of trace reconstruction can be stated simply as follows: consider a sequence $X$ which is simultaneously passed through $t$ independent deletion channels to yield $t$ output subsequences (also called \textit{traces}) of $X$ (see Fig.~\ref{fig:tdeletion}). How many such traces are needed to reconstruct $X$ perfectly? A variety of upper and lower bounds for this problem have been proposed, both for worst case and average case reconstruction. Our problem formulation is complementary to this, as we discuss next.
 
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.2]{tdeletion.pdf}
\caption{The $t$-trace deletion channel model: the  sequence $X$ is passed through $t$ independent deletion channels to yield $t$ \textit{traces}. We aim to estimate $X$ from the $Y^{(i)}$s.}
\label{fig:tdeletion}
\end{center}
\end{figure}
 
\noindent \textbf{Problem formulation.}  Given an input sequence of length $n$ (known apriori), the independently and identically distributed (i.i.d.) deletion channel deletes each input symbol indepedently with probability $\delta$, producing at its output a subsequence of the input sequence. Consider a sequence $X$ passed through $t$ ($t$ is fixed) such deletion
channels as shown in
Fig.~\ref{fig:tdeletion}. We call this the $t$-trace deletion channel model. We ask three main questions:
\begin{enumerate}
\item For $t=1$ (also called \textit{single-trace deletion channel}, see Fig.~\ref{fig:1deletion}), what is the maximum-likelihood estimate of $X$ having observed $Y$, i.e., a solution to $\argmax\limits_{x\in \{0,1\}^n}\Pr(Y|X)$.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.2]{1deletion.pdf}
\caption{The single-trace deletion channel model.}
\label{fig:1deletion}
\end{center}
\end{figure}
\item For $t=1$  and  $X_i \sim\ \text{ind. Ber}(p_i)$ in Fig.~\ref{fig:1deletion}, what are the posterior distributions of $X_i$ given the trace $Y$, i.e., compute $\Pr(X_i=\alpha|Y)$.
\item For a fixed $t$, with $t>1$   and $X_i \sim\ \text{i.i.d. Ber}(0.5)$  in Fig.~\ref{fig:tdeletion}, what are the posterior distributions of $X_i$ given all traces $Y^{(1)}, Y^{(2)},...,Y^{(t)}$, i.e., compute $\Pr(X_i=\alpha|Y^{(1)}, Y^{(2)},...,Y^{(t)})$.
\end{enumerate}

We make two observations:\\
{\bf I.} An answer to  2) above doesn't lead to a natural solution for 3) since the deletion channel is not memoryless. In particular, for a memoryless channel, we have $Y^{(j)}_i - X_i - Y^{(k)}_i$ and hence $\Pr(X_i=\alpha|Y^{(j)}, Y^{(k)}) = \Pr(X_i=\alpha|Y^{(j)}_i, Y^{(k)}_i) \propto \Pr(X_i=\alpha|Y^{(j)}_i) \Pr(X_i=\alpha|Y^{(k)}_i)$; so one could first obtain the posterior probabilities from each independent observation and combine them after. However, this is not the case for deletion channels since the markov chain $Y^{(j)}_i - X_i - Y^{(k)}_i$ no longer holds. As a result, one first needs to  ``align'' all the observations in order to compute the likelihoods. \\
{\bf II.} Solving 3) naturally leads to an algorithm for trace reconstruction, that selects the most likely value for each $X_i$. However, the problem formulation in 3) asks a question complementary to the trace reconstruction: given a fixed (possibly a few) number of traces, what is our ``best'' guess of $X$? Unlike trace reconstruction, we are not concerned with perfect reconstruction (since perfect reconstruction may not be possible with just a few traces). We also note that error rate guarantees for our algorithms (not a part of this work) would naturally lead to upper bounds for trace reconstruction.\\


\noindent \textbf{Contributions.}
Our main contributions are as follows. %\textcolor{blue}{We can update order once we finalize ordering of sections.}
%We consider a main contribution of this paper the tools we provide to visualize and analyze error events (described in Section~\ref{}) for the multiple deletion channel model in Fig.~\ref{fig:tdeletion}. We also provide algorithms to solve the problems stated in 1) and 2) earlier in the section. In particular:
\begin{itemize}[leftmargin=5mm]
\item We introduce mathematical tools and constructs to visualize and analyze single-trace and $t$-trace deletion error events (see Section~\ref{sec:notation}).  
\item For the single-trace deletion channel, we establish an equivalence between finding the optimal ML decoder and a continuous optimization problem we introduce (see Section~\ref{sec:1deletion_ML}).
\item In Section~\ref{sec:1deletion}, we prove the following:
\begin{theorem}
For the single-trace deletion channel model with priors $X_i \sim \text{ind. Ber}(p_i)$ and observed trace $Y$, the symbolwise posterior probabilities $\Pr(X_i=1|Y)\ \forall\ i$ can be computed in $O(n^2)$ time complexity.
\end{theorem}
 \item  In Section~\ref{sec:exactsmap}, we prove the following:
\begin{theorem}
For the $t$-trace deletion channel model with priors $X_i \sim \text{i.i.d. Ber}(0.5)$ and observed traces $Y^{(1)},...,Y^{(t)}$, the symbolwise posterior probabilities $\Pr(X_i = 1|Y^{(1)},...,Y^{(t)})\ \forall\ i$ can be computed in $O(2^t n^{t+2})$ time complexity.\\
\end{theorem}
\end{itemize}

\noindent \textbf{Tools and techniques.} In terms of theoretical tools, the series of books by Lothaire (\cite{lothaire1997combinatorics,lothaire2002algebraic,lothaire2005applied}) extensively use algebraic tools  for problems in the combinatorics of sequences (or \textit{words}), and our work is inspired by such techniques. We borrow some notation and leverage a few of their results in our work. \\

\noindent \textbf{Biological motivation.} Trace reconstruction in itself was motivated, in part, by problems in DNA sequence reconstruction. One such problem was to infer the DNA sequence of a common ancestor from the samples of its descendants. Our problem definition, that considers a fixed value of $t$, would fit naturally in a scenario with a fixed number of descendants where perfect reconstruction may not be possible.
Our motivation for considering this problem also comes from a recent DNA sequencing technology called \textit{nanopore sequencing}. The $t$-trace deletion channel model is a simplistic model to approximately capture the process of a DNA sequence passed through a nanopore sequencer\footnote{As seen in
  \cite{Mao2017},\cite{MDK17} there are more complicated effects of
  the nanopore reader not captured in this simple 
  representation.}.  \\




\noindent \textbf{More related work.}
Our work falls under the general umbrella of  sequence reconstruction over deletion channels, where we offer, to the best of our knowledge, the first non-trivial results on maximum likelihood and maximum aposteriori estimates for the single and multiple deletion channel. As mentioned earlier, the complementary problem of trace reconstruction falls closest to this work.


The deletion channel by itself is known to be notoriously difficult to analyse. As stated earlier, the capacity of a single deletion channel is still unknown (\cite{diggavi2007capacity,diggavi2006information,diggavi2001transmission}); as are optimal coding schemes. Prior works have looked at the design of codes for deletion channels (\cite{ratzer2005marker,ratzer2000codes,thomas2017polar}); these works consider use of a codebook (we do not). Statistical estimation over deletion channels is a difficult problem to analyze due its highly combinatorial nature. To the best of our knowledge, as yet there are no efficient estimation algorithms over deletion channels with statistical guarantees.

Very recently, a variant of the trace reconstruction problem called \textit{coded trace reconstruction} has been proposed, motivated by portable DNA-based data storage systems using DNA nanopores (see \cite{abroshan2019coding}, \cite{cheraghchi2019coded}, \cite{brakensiek2019coded}) and we believe that the ideas in this work may prove useful in such a setting.

There are other works on sequence assembly (see for example, \cite{Li09fastand}, \cite{Shomorony2016}),
where multiple short reads (from different segments of a sequence) are used to reconstruct the bigger
sequence. This work differs from sequence assembly since we are interested in inferring the entire length sequence and not  just small segments of it (which are then ``stitched'' together in sequence assembly).\\

\noindent \textbf{Paper Organization.} Section~\ref{sec:notation} introduces our notation and visualization tools for the single and $t$-trace  channel error events; Section~\ref{sec:1deletion_ML} provides a result concerning question 1) wherein we prove the equivalence of ML decoding to solving a continuous optimization problem; Section~\ref{sec:1deletion} answers question 2) for the single-trace channel;
 Section~\ref{sec:exactsmap}) answers question 3) for the  $t$-deletion channel;  Section~\ref{sec:Numerics} gives numerical evaluations; and Section~\ref{sec:conclusions} concludes the paper.


==> Sections/intro__Sundara_Rajan_s_conflicted_copy_2019-10-11_.tex <==


\section{Introduction}
\label{sec:intro}



Sequence reconstruction over deletion channels, both with and without a codebook, has received considerable attention in the information theory as well as in the theoretical computer science literature. From an information theory perspective, reconstruction over the deletion channel, or more specifically a  maximum-likelihood (ML) argument for the deletion channel, would give further insight on the capacity of the deletion channel, a long-standing open problem (see \cite{mitzenmacher2009survey}). To quote \cite{mitzenmacher2009survey} -- ``at the very least, progress in this direction would likely surpass previous results on the capacity of the deletion channels''. Yet, there are no results on reconstruction over a deletion channel with statistical guarantees -- in this work, we take a step in this direction.

On the other hand, the problem of \textit{trace reconstruction}, as introduced in \cite{Batu2004}, has received renewed interest in the past few years (see \cite{Holenstein2008}, \cite{Peres2017}, \cite{De2017}, \cite{holden18}, \cite{Nazarov:2017}, \cite{holden2018lower}, \cite{chase2019new}). The problem of trace reconstruction can be stated simply as follows: consider a sequence $X$ which is simultaneously passed through $t$ independent deletion channels to yield $t$ deleted observations (also called \textit{traces}) of $X$ (see Fig.~\ref{fig:tdeletion}). How many such traces are needed to reconstruct $X$ perfectly? A variety of upper and lower bounds for this problem have been proposed, both for worst case and average case reconstruction. Our problem definition, stated in the following paragraph, is closely related to the average case trace reconstruction.
 
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.2]{tdeletion.pdf}
\caption{$t$-deletion channel model:  sequence $X$ passed through $t$ independent deletion channels to yield $t$ \textit{traces}. We aim to estimate $X$ from the $Y^{(i)}$s.}
\label{fig:tdeletion}
\end{center}
\end{figure}
 
\noindent \textbf{Problem definition.}  Given an input sequence of length $n$ (known apriori), the independently and identically distributed (i.i.d.) deletion channel deletes each input symbol indepedently with probability $\delta$, producing at its output a subsequence of the input sequence. Consider a sequence $X$ passed through $t$ ($t$ is fixed) such deletion
channels as shown in
Fig.~\ref{fig:tdeletion}. We call this the $t$-deletion channel model. We ask two questions:
\begin{enumerate}
\item For $t=1$ (see Fig.~\ref{fig:1deletion}, also called the single deletion channel model), and when $X_i \sim\ \text{ind. Ber}(p_i)$, compute the posterior distributions of $X_i$ given the trace $Y$.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.25]{1deletion.pdf}
\caption{The single deletion channel model. We assume $X_i \sim\ \text{ind. Ber}(p_i)$.}
\label{fig:1deletion}
\end{center}
\end{figure}
\item In the $t$ deletion channel model, for a fixed $t$ assume that $X_i \sim\ \text{i.i.d. Ber}(0.5)$ and compute the posterior distributions of $X_i$ given all traces $Y^{(1)}, Y^{(2)},...,Y^{(t)}$. 
\end{enumerate}
Note that solving 1) above doesn't lead to a natural solution for 2). This is because for a memoryless channel, we have $Y^{(j)} - X_i - Y^{(k)}$ and hence $\Pr(X_i=\alpha|Y^{(j)}, Y^{(k)}) \propto \Pr(X_i=\alpha|Y^{(j)}) \Pr(X_i=\alpha|Y^{(k)})$; so one could independently combine the posterior probabilities from each noisy observation. This is not the case for deletion channels since the markov chain $Y^{(j)} - X_i - Y^{(k)}$ no longer holds. More intuitively, one needs to first ``align'' the traces for computing the likelihoods. 
%, where every channel independently deletes each bit with probability $\delta$.


We point out that the problem considered in 2) asks a question complementary to the trace reconstruction: given a fixed (possibly a few) number of traces, what is our ``best'' guess of $X$? We provide algorithms which do this. Unlike trace reconstruction, we are not concerned with perfect reconstruction (since perfect reconstruction may not be possible with just a few traces), although it should also be obvious that performance guarantees for our algorithms (not a part of this work) would naturally lead to upper bounds for trace reconstruction.

Deletion channel by itself is known to be notoriously difficult to analyse. As stated earlier, the capacity of a single deletion channel is still unknown (\cite{diggavi2007capacity,diggavi2006information,diggavi2001transmission}); as are optimal coding schemes. Recent works have looked at the design of codes for deletion channels (\cite{ratzer2005marker,ratzer2000codes,thomas2017polar}); these works consider use of a codebook (we do not). As a result, statistical estimation over deletion channels is also a difficult problem due its highly combinatorial nature. To the best of our knowledge, as yet there are no efficient estimation algorithms over deletion channels with statistical guarantees; not even for ML over a single deletion channel.


\noindent \textbf{Biological motivation.} Trace reconstruction in itself was motivated, in part, by problems DNA sequence reconstruction. One such problem was to infer the DNA sequence of a common ancestor from the samples of its descendants. We argue that our problem definition fits more naturally in such a scenario since perfect reconstruction may not be feasible or even possible. Our motivation for considering this problem also comes from a recent DNA sequencing technology called \textit{nanopore sequencing}. The $t$-deletion channel model is a simplistic model to approximately capture the process of a DNA sequence passed through a nanopore sequencer\footnote{As seen in
  \cite{Mao2017},\cite{MDK17} there are more complicated effects of
  the nanopore reader not captured in this simple 
  representation.}.  
  
Very recently, a variant of the trace reconstruction problem called \textit{coded trace reconstruction} has been proposed, motivated by portable DNA-based data storage systems using DNA nanopores (see \cite{abroshan2019coding}, \cite{cheraghchi2019coded}, \cite{brakensiek2019coded}) and we believe that the ideas in this work may prove useful in such a setting.

There are other works on sequence assembly (see for example, \cite{Li09fastand}, \cite{Shomorony2016}),
where multiple short reads (from different segments of a sequence) are used to reconstruct the bigger
sequence. This work differs from sequence assembly since we are interested to infer the entire length sequence and not  just small segments of it (which are then ``stitched'' together in sequence assembly).

\noindent \textbf{Tools and techniques.} In terms of theoretical tools, the series of books by Lothaire (\cite{lothaire1997combinatorics,lothaire2002algebraic,lothaire2005applied}) extensively use algebraic tools  for problems in the combinatorics of sequences (or \textit{words}), and our work is inspired by such techniques. We borrow many of their notations and results for our work.


\noindent \textbf{Contributions.} {\color{red}} Our main contribution is to provide tools to visualize and analyze error events (described in the next section) for the multiple deletion channel model in Fig.~\ref{fig:tdeletion}. We also provide algorithms to solve the problems stated in 1) and 2) earlier in the section.
\begin{itemize}[wide=5pt]
\item In section~\ref{sec:1deletion}, for the single deletion channel model, we provide an  $O(n^2)$  algorithm to calculate the symbolwise posterior probabilities  $\Pr(X_i=1|Y)\ \forall\ i$ when $X_i \sim \text{ind. Ber}(p_i)$.
 \item  In Section~\ref{sec:exactsmap}, for the $t$-deletion channel model, we give an $O(2^t n^{t+2})$ algorithm to calculate the symbolwise posterior probabilities $\Pr(X_i = 1|Y_1,...,Y_t)$ when $X_i \sim \text{ind. Ber}(0.5)$.
\end{itemize}





==> Sections/multiple.tex <==


\section{Symbolwise posterior probabilities for the $t$-trace deletion channel}
\label{sec:exactsmap}

In this section, we put to use the ideas and constructs introduced in section~\ref{sec:notation} to exactly compute the symbolwise posterior probabilities given $t$-traces, which in turn gives a symbolwise MAP estimate (with uniform priors) of the input sequence. In Appendix~\ref{app:remnant_postprob}, we also provide a method to compute the symbolwise posterior probabilities for the remnant channel -- we encourage the reader  to use this appendix as a warm-up. For the $t$-trace deletion channel, similar expressions arise due to the channel equivalence result of Theorem~\ref{thm:channel_equiv}.

Let $\mathcal A = \{0,1\}$, and  assume that $X\sim $ Uniform $\mathcal A^n$. Our goal is to compute the symbolwise posterior probabilities $\Pr(X_i{=}1|Y^{(1)},...,Y^{(t)})$, where $Y^{(j)}$ is the $j^{th}$ trace. Our proposed algorithm is provided in Alg.~\ref{alg:exact_smap} and estimates the symbolwise MAP  (with uniform priors). We can  directly leverage   Alg.~\ref{alg:exact_smap} to reconstruct the input as follows: for each index $i$, compute $\Pr(X_i{=}1|Y^{(1)},...,Y^{(t)})$ and decide
\begin{align*}
\hat{X}_i = \begin{cases}
 1,\quad &$if$\  \Pr(X_i{=}1|Y^{(1)},...,Y^{(t)})\geq 0.5 \\
0, \quad &$otherwise$.
\end{cases}
\end{align*}
Through the rest of this section, we show how to compute $\Pr(X_i{=}1|Y^{(1)},...,Y^{(t)})$\footnote{Symbolwise MAP with non-uniform priors is  part of on-going work.} in two steps:
\begin{itemize}
\item We first give an expression for $\Pr(X_i{=}1|Y^{(1)},...,Y^{(t)})$ which sums over potentially an exponential number of terms.
\item We then show that this summation can be computed in polynomial time (polynomial in the blocklength $n$).
\end{itemize}


\noindent \textbf{Step 1: An expression for $\Pr(X_i{=}1|Y^{(1)},...,Y^{(t)})$.}
\begin{theorem}
\label{thm:exactSMAP_posteriorprob}
Assume $X\sim $ Uniform $\mathcal A^n$ or equivalently $X_i \sim\ \text{Ber}(0.5)$. The posterior probability of the $i^{th}$ bit given the $t$ traces can be expressed as
\begin{align*}
\Pr(X_i=1|Y^{(1)},&...,Y^{(t)}) &\\ =
 & \Bigg[ \sum_{k=0}^n 2^{n-k-1}{n-1 \choose k} \sum_{w||w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \\
&+ \sum_{k=0}^n \sum_{j=1}^k 2^{n-k}{i-1 \choose j-1}{n-i \choose k-j} \sum_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \Bigg] \Big/ \\ 
 &\Bigg[ \sum_{k=0}^n 2^{n-k} {n \choose k} \sum_{\substack{w| |w|=k}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle  \Bigg]. \numberthis
 \label{eq:posterior_prob}
\end{align*}
\end{theorem}
Note that the summation index, $w| |w|{=}k$ is over all sequences $w$ of length $k$; this is an alternate expression for $w|w{\in}\mathcal A^k$. We follow this convention throughout the rest of the paper. 
\begin{proof}
\begin{align*}
\Pr(X_i=1&|Y^{(1)},...,Y^{(t)}) = \sum_{\substack{x||x|=n,\\x_i=1}} \Pr(x|Y^{(1)},...,Y^{(t)})\\
&\overset{(a)}{=} \frac{1}{2^n \Pr(Y^{(1)},...,Y^{(t)})} \sum_{\substack{x||x|=n,\\x_i=1}} \Pr(Y^{(1)},...,Y^{(t)}|x)\\
&\overset{(b)}{=} \frac{1}{2^n \Pr(Y^{(1)},...,Y^{(t)})} \sum_{\substack{x||x|=n,\\x_i=1}} \prod_{j=1}^t\Pr(Y^{(j)}|x),
\end{align*}
where $(a)$ uses Bayes' principle and $(b)$ is because each deletion channel acts independently. Recall that for  a deletion channel with deletion probability $\delta$, $\Pr(Y|X=x)={x \choose Y}\delta^{|x|-|Y|}(1-\delta)^{|Y|}$. Also, using the fact that $\Pr(Y^{(1)},...,Y^{(t)})=\sum\limits_{\substack{x||x|=n}}\Pr(x) \Pr(Y^{(1)},...,Y^{(t)}|x)$ we have,

\begin{align*}
\Pr(X_i=1|Y^{(1)},...,Y^{(t)})=  \frac{\sum\limits_{\substack{x||x|=n,\\x_i=1}} {x \choose Y^{(1)}}...{x \choose Y^{(t)}}}{\sum\limits_{\substack{x||x|=n}} {x \choose Y^{(1)}}...{x \choose Y^{(t)}}}. \numberthis \label{eq:thmexactsmap_proofterm0}
\end{align*}


We first simplify the numerator $\sum\limits_{\substack{x||x|=n,\\x_i=1}} {x \choose Y^{(1)}}...{x \choose Y^{(t)}}$; the denominator can be simplified using the same approach. Now,

\begin{align*}
\sum\limits_{\substack{x||x|=n,\\x_i=1}} {x \choose Y^{(1)}}...{x \choose Y^{(t)}}  &\overset{(a)}{=} \sum_{\substack{x||x|=n,\\x_i=1}}  \sum_{w\in \{0,1\}^*} {x \choose w} \langle Y^{(1)} \uparrow Y^{(2)} \uparrow ... \uparrow Y^{(t)},w \rangle \\
  &=\sum_{w\in \mathcal A^*} \langle Y^{(1)} \uparrow Y^{(2)} \uparrow ... \uparrow Y^{(t)},w \rangle  \sum_{\substack{x||x|=n,\\x_i=1}}{x \choose w}\\
&\overset{(b)}{=}\sum_{w\in \mathcal A^*} \langle Y^{(1)} \uparrow Y^{(2)} \uparrow ... \uparrow Y^{(t)},w \rangle \\
 & \hspace{2cm} \times  2^{n-|w|}\left(\frac{1}{2}{n-1 \choose |w|}+\sum_{j|w_j=1}{i-1 \choose j-1}{n-i \choose |w|-j}\right)
\end{align*}
where $(a)$ is due to Lemma~\ref{lemma:bin_inf_relation} and $(b)$ due to Lemma~\ref{lemma:smapsum} (both introduced in \cite{Srini2018}); see Appendix~\ref{app:bin_inf_lemma} and Appendix~\ref{app:smapsum} for the statement and proof. % Lemma~\ref{lemma:bin_inf_relation} and Lemma~\ref{lemma:smapsum} were introduced in \cite{Srini2018},%but they are restated with proofs in the appendix for convenience.
Note that  Lemma~\ref{lemma:bin_inf_relation} is an alternate mathematical outlook of the channel equivalence in Theorem~\ref{thm:channel_equiv} (see Appendix~\ref{app:channel_equiv}).

\noindent Therefore we have,
\begin{align*}
\sum\limits_{\substack{x||x|=n,\\x_i=1}} {x \choose Y^{(1)}}...{x \choose Y^{(t)}}
&\overset{(a)}{=} \sum_{k=0}^{\infty} 2^{n-k-1}{n-1 \choose k} \sum_{w| |w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \\
&\hspace{1cm}+ \sum_{k=0}^{\infty} \sum_{j=1}^k 2^{n-k}{i-1 \choose j-1}{n-i \choose k-j} \sum_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)}  \uparrow ... \uparrow Y^{(t)},w \rangle \\ 
&\overset{(b)}{=} \sum_{k=0}^n 2^{n-k-1}{n-1 \choose k} \sum_{w| |w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \\
&\hspace{1cm}+ \sum_{k=0}^n \sum_{j=1}^k 2^{n-k}{i-1 \choose j-1}{n-i \choose k-j} \sum_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)}  \uparrow ... \uparrow Y^{(t)},w \rangle, \numberthis
\label{eq:thmexactsmap_proofterm1}
\end{align*}
where in $(a)$ we first fix $|w|$ and then sum over all $w$ of the given length and $(b)$ holds because the combinatorial terms are $0$ when $k>n$. 
A similar analysis gives  \begin{align*}
\sum\limits_{x| |x|=n} &{x \choose Y^{(1)}}...{x \choose Y^{(t)}} = \sum_{k=0}^n 2^{n-k} {n \choose k} \sum_{\substack{w| |w|=k}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle.\numberthis
\label{eq:thmexactsmap_proofterm2}
\end{align*} 
Plugging \eqref{eq:thmexactsmap_proofterm1} and \eqref{eq:thmexactsmap_proofterm2} in \eqref{eq:thmexactsmap_proofterm0}, we get the expression in Theorem~\ref{thm:exactSMAP_posteriorprob},
\begin{align*}
\Pr(X_i=1|Y^{(1)},&...,Y^{(t)}) &\\ =
 & \Bigg[ \sum_{k=0}^n 2^{n-k-1}{n-1 \choose k} \sum_{w||w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \\
&+ \sum_{k=0}^n \sum_{j=1}^k 2^{n-k}{i-1 \choose j-1}{n-i \choose k-j} \sum_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \Bigg] \Big/ \\ 
 &\Bigg[ \sum_{k=0}^n 2^{n-k} {n \choose k} \sum_{\substack{w| |w|=k}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle  \Bigg].
\end{align*}
\end{proof}

\noindent \textbf{Step 2: Dynamic program to compute $\sum\limits_{w| |w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle$ and $\sum\limits_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle$.}
  Note that the number of sequences $w| |w|=k$ is $O(2^k)$ so a naive evaluation is exponential in the blocklength $n$. We can, however, exploit the edit graph to come up with a dynamic program resulting in an algorithm which is polynomial in $n$. 

Recall that in the edit graph, $\langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle$ is equal to the number of distinct paths from the origin $(0,...,0)$ to the destination $(|Y^{(1)}|,...,|Y^{(t)}|)$ and which correspond to $w$. Hence,
\begin{enumerate}[wide=0pt]
\item[(a)]  $\sum\limits_{w| |w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle$ is the number of distinct paths of length $k$ from origin to destination and,
\item[(b)]  $\sum\limits_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle$ is the number of such paths of length $k$ such that the $j^{th}$ edge of the path corresponds to a `1'.
\end{enumerate}

\noindent With this interpretation, the dynamic program for (a) follows naturally -- the number of  $k$-length paths from the origin to any vertex is the sum of the number of $(k{-}1)$-length paths from the origin to all incoming neighbors of the vertex. To make this formal, associate a  polynomial (in $\lambda$) for each vertex, such that the coefficient of $\lambda^k$ 
is equal to the number of paths of length $k$ from the origin to $v$: we call it the "forward-potential" polynomial $p^{for}_v(\lambda)$ for vertex $v$, the coefficient of $\lambda^k$ as earlier is denoted by $\langle p^{for}_v(\lambda),\lambda^k \rangle $. The dynamic program to compute $p^{for}_v(\lambda)$ for all $v$ can be expressed as:
\begin{equation}
p^{for}_v(\lambda) = \sum_{u|u\rightarrow v} \lambda p^{for}_u(\lambda).
\end{equation}
With this definition, we have $$\sum\limits_{w| |w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle =\langle p^{for}_{destination}(\lambda),\lambda^k \rangle.$$ In the example in Fig.~\ref{fig:editgraph_smap1}, one could do the following: order the vertices $(0,0)$ to $(3,3)$ lexicographically and then compute $p^{for}_v(\lambda)$ in the same order. Because of the directed grid nature of the edit graph, every vertex has incoming neighbors which are lexicographically ahead of itself. Also we initialize $p^{for}_{(0,0)}(\lambda)=1$.  For the example in Fig.~\ref{fig:editgraph_smap1}, the forward-potentials are shown in Fig.~\ref{fig:editgraph_smap2}. The complexity of this dynamic program is $O(2^tn^{t+1})$ as it goes over $O(n^t)$ vertices and for each vertex it sums $O(2^t)$ polynomials, each of degree $O(n)$.

 
\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap2.pdf}
\caption{The forward-potential $p^{for}_v(\lambda)$ at each vertex.} 
\label{fig:editgraph_smap2}
\end{figure}

We compute (b) as follows: pick an edge $(u{\rightarrow}v)$ which corresponds to `1', count the number of $(j{-}1)$-length paths from origin to $u$ and multiply it with the number of $(k{-}j)$-length paths from $v$ to the destination -- this is exactly the number of paths of length $k$ such that its $j^{th}$ edge is $(u{\rightarrow}v)$. Summing this term for all such edges which correspond to 1 gives us the term in (b). Note that we have already computed the number of $k$-length paths ($\forall k$) from origin to every vertex  in $p^{for}_v(\lambda)$ . We can similarly compute the number of $k$-length  paths ($\forall k$) from every vertex to the destination as $p^{rev}_v(\lambda)$ -- the "reverse potential" polynomial. The dynamic program for $p^{rev}_v(\lambda)$ is:
\begin{equation}
p^{rev}_v(\lambda) = \sum_{u|v\rightarrow u} \lambda p^{rev}_u(\lambda),
\end{equation}
with $p^{rev}_{destination}(\lambda)=1$.  The reverse potentials for the example in Fig.~\ref{fig:editgraph_smap1} is shown in Fig.~\ref{fig:editgraph_smap3}. Like in the case of forward potential, we first order the vertices reverse lexicographically and then invoke the dynamic program above sequentially to compute the reverse potential polynomial at each vertex.

\begin{algorithm}[t!]
\caption{Computing the forward-potentials $p^{for}_u(\lambda)$ }\label{alg:forward_pot}
\begin{algorithmic}[1]
\item Input: Edit graph {$\mathcal G(Y^{(1)},...,Y^{(t)})$}\\ Outputs: $p^{for}_v(\lambda)\ \forall\ v$
\State Order the vertices from $(0,0,...,0)$ to $(|Y^{(1)}|,|Y^{(2)}|,...,|Y^{(t)}|)$ lexicogaphically; let the ordered list be $\mathcal V$
\State Initialise $p^{for}_{(0,...,0)}(\lambda)\gets 1$
\For{$v\ \in\ \mathcal V$}
\State \textbf{assign} $p^{for}_v(\lambda)\gets  \sum_{u|u\rightarrow v} \lambda p^{for}_u(\lambda)$
\EndFor
%\State \textbf{return} $p^{for}_v(\lambda)\ \forall\ v$
\end{algorithmic}
\end{algorithm}


\begin{algorithm}[t!]
\caption{Computing the reverse-potentials $p^{rev}_u(\lambda)$ }\label{alg:reverse_pot}
\begin{algorithmic}[1]
\item Input: Edit graph {$\mathcal G(Y^{(1)},...,Y^{(t)})$}\\ Outputs: $p^{rev}_v(\lambda)\ \forall\ v$
\State Order the vertices from $(|Y^{(1)}|,|Y^{(2)}|,...,|Y^{(t)}|)$ to $(0,0,...,0)$ reverse lexicogaphically; let the ordered list be $\mathcal V$
\State Initialise $p^{rev}_{(|Y^{(1)}|,|Y^{(2)}|,...,|Y^{(t)}|)}(\lambda)\gets 1$
\For{$v\ \in\ \mathcal V$}
\State \textbf{assign} $p^{rev}_v(\lambda) \gets \sum_{u|v\rightarrow u} \lambda p^{rev}_u(\lambda)$
\EndFor
%\State \textbf{return} $p^{rev}_v(\lambda)\ \forall\ v$
\end{algorithmic}
\end{algorithm}


\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap3.pdf}
\caption{The reverse-potential $p^{rev}_v(\lambda)$ at each vertex.} 
\label{fig:editgraph_smap3}
\end{figure}

With this, the term in (b) can be expressed as:

\begin{align*}
\sum\limits_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle =\hspace{-2mm} \sum_{\substack{(u,v)|\\s(u\rightarrow v)=1}} \hspace{-2mm}\langle p^{for}_u(\lambda),\lambda^{j-1} \rangle \langle p^{rev}_v(\lambda),\lambda^{k-j} \rangle.
\end{align*}


Alg.~\ref{alg:exact_smap} now summarizes the computation of the posterior probabilities. This algorithm iterates over all the edges (we have $O((2n)^t)$ of these), and also $k,j$ ($O(n)$ each). The time complexity of Alg.~\ref{alg:exact_smap} hence is $O(2^tn^{t+2})$.
 

%======================================================================================
\begin{algorithm}[t!]
\caption{Symbolwise posterior probabilities with $t$ traces} % $\sum\limits_{w| |w|=k} \langle Y_1 {\uparrow} ... {\uparrow} Y_t,w \rangle\ \forall\ k$ and $\sum\limits_{{w| |w|=k,w_j=1}} \langle Y_1 {\uparrow} ... {\uparrow} Y_t,w \rangle $ $\forall\ j,k$ }
\label{alg:exact_smap}
\begin{algorithmic}[1]
\item Input: Traces {$Y^{(1)},Y^{(2)},...,Y^{(t)}$, input length $n$}\\ Output: $\Pr(X_i=1|Y^{(1)},Y^{(2)},...,Y^{(t)})\ \forall\ i$% $\sum\limits_{w| |w|=k} \langle Y_1 {\uparrow} ... {\uparrow} Y_t,w \rangle\ \forall\ k$ and $\sum\limits_{{w| |w|=k,w_j=1}} \langle Y_1 {\uparrow} ... {\uparrow} Y_t,w \rangle$
\State Construct edit graph $\mathcal G(Y^{(1)},...,Y^{(t)})$
\State Use Alg.~\ref{alg:forward_pot} and Alg.~\ref{alg:reverse_pot} on $\mathcal G(Y^{(1)},...,Y^{(t)})$ to calculate $p^{for}_v(\lambda)$ and $p^{rev}_v(\lambda)$ $\forall\ v$

\For{$k \in\ [0:n]$}
\State \textbf{assign} $\sum\limits_{w| |w|=k}  \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \gets \langle p^{for}_{destination}(\lambda),\lambda^k \rangle.$
\For{each $j \in\ [1:n]$}
\State Initialize $temp \leftarrow $   0
\For{each edge $u\rightarrow v\ \in\ \mathcal G$}
\If{$s(u{\rightarrow} v)=$ `1'}
\State $temp\ +=  \langle p^{for}_u(\lambda),\lambda^{j-1} \rangle \langle p^{rev}_v(\lambda),\lambda^{k-j} \rangle$
\EndIf
\EndFor
\State \textbf{assign} $\sum\limits_{\substack{w| |w|=k,\\w_j=1}} \langle Y^{(1)} \uparrow ... \uparrow Y^{(t)},w \rangle \gets temp$
\EndFor
\EndFor
\For{$i \in\ [1:n]$}
\State Use \eqref{eq:posterior_prob} to compute $\Pr(X_i=1|Y^{(1)},Y^{(2)},...,Y^{(t)})$
\EndFor
\end{algorithmic}
\end{algorithm}



==> Sections/notation.tex <==

\section{Notation and Tools}
\label{sec:notation}

\noindent \textbf{Basic notation:} We borrow some notation  from \cite{lothaire1997combinatorics} which deals with non-commutative algebra; we restate them here for convenience. Calligraphic letters refer to sets, capitalized letters
correspond to random variables and bold letters are used for functions.  Let $\mathcal{A}$ be the set of all
symbols. Throughout this work, we will focus on the case where $\mathcal{A}=\{0,1\}$,
though  our methods extend to arbitrarily large sets of finite size. Define
$\mathcal{A}^n$ to be the set of all $n$-length sequences and $\mathcal{A}^*$ to be the set of all finite length sequences with
symbols in $\mathcal{A}$. For a sequence $f$, $|f|$ denotes the length
of $f$. 

For integers $i,j$, we define $[i:j] \triangleq \{i,i+1,...,j\}$ if $j\geq i$ and $[i:j] \triangleq \emptyset$ otherwise. We also define $[i] \triangleq [1:i]$.

For a vector or sequence $x=(x_1,x_2,...,x_{i-1},x_i,x_{i+1},...,x_n)$, define $$x^{(i\rightarrow s)}\triangleq (x_1,x_2,...,x_{i-1},s,x_{i+1},...,x_n),$$ where the $i^{th}$ coordinate of $x$ is replaced by symbol $s$. 	\\

\noindent \textbf{Binomial coefficient  \cite{lothaire1997combinatorics}:} Given sequences $f$ and $g$ in $\mathcal{A}^*$, the number of
subsequence patterns of $f$ that are equal to $g$ is called the
\textit{binomial coefficient} of $g$ in $f$ and is denoted by $f\choose g$.  For example, ${'apple' \choose 'ape'} = 2$ since $'ape'$ can be obtained from two (overlapping) subsequences of $'apple'$.
When the alphabet $\mathcal{A}$ is of cardinality 1, ${f \choose g} = {|f| \choose |g|}$, the classical binomial coefficient with their respective lengths as the parameters. This definition hence
could be thought of as a generalization of the classical binomial
coefficients. We will denote by $e$ the sequence of length 0, and {define ${f
  \choose e} \triangleq 1\ \forall\ f\ \in\ \mathcal{A}^*$.} We also define the classical binomial coefficient ${a \choose b}\triangleq 0,$ whenever $b>a$ or $b<0$ for ease of use.


The binomial coefficient forms the backbone for the probabilistic analysis of deletion channels since the input-output relation for a deletion channel (with deletion probability $\delta$, input $X$ and output $Y$) can be expressed as 
\begin{equation}
\label{eq:in-out_relation}
\Pr(Y=y|X=x) = {x \choose y} \delta^{|x|-|y|} (1-\delta)^{|y|}.
\end{equation}
The proof is straightforward -- the number of distinct error events that give rise to $y$ from $x$ is exactly the number of  subsequences of $x$ which are equal to $y$. Each of these error events has a probability $\delta^{|x|-|y|} (1-\delta)^{|y|}$, wherein the exponent of $\delta$ corresponds to the deleted symbols and the exponent of  $1-\delta$ to the undeleted symbols. \\

\noindent \textbf{Maximum Likelihood (ML) estimate:}
Given the definition of the binomial coefficient, the maximum-likelihood (ML) estimate over a deletion channel with observed output $Y$ can be cast in the following form:
\begin{align*}
\argmax_{x \in \{0,1\}^n}  {x \choose Y}.\numberthis
\label{eq:ML_deletion}
\end{align*}
In the case of multiple deletion channels with observed traces $Y^{(1)},...,Y^{(t)}$, the ML formulation is similar:
\begin{align*}
\argmax_{x \in \{0,1\}^n}  \prod_{j=1}^{t} {x \choose Y^{(j)}}.\numberthis
\label{eq:ML_multiple_deletion}
\end{align*}
As yet, there is no known efficient way to come up with a solution for either of the above two formulations (see \cite{mitzenmacher2009survey}).\\
%In this work, we attempt to take a step in this direction by showing that a continuous relaxation of \eqref{eq:ML_deletion} is equivalent to \eqref{eq:ML_deletion}. However, an efficient algorithm to solve the optimization \eqref{eq:ML_deletion} remains open. In the context of trace reconstruction, the ultimate pursuit would be an algorithm for \eqref{eq:ML_multiple_deletion} with $\mathcal C = \{0,1\}^n$ and error analysis thereof.

\noindent \textbf{Relaxed binomial coefficient.}
We now introduce the function  $\mathbf F(\cdot)$  which can be thought of as a real-valued relaxation of the binomial coefficient. This function is used in sections~\ref{sec:1deletion_ML} and~\ref{sec:1deletion}.


An intuitive definition is as follows: Consider a random vector $Z\in\{0,1\}^n$ such that $Z_i\sim$ ind. Ber$(p_i)$, let $p$ be the vector of probabilities of length $n$, $\mathcal S\subseteq [n]$ a subset of the indices of size $m$, and ${v}$ a binary vector of length $m$. Then, $$\mathbf F(p,v)=\sum_{\substack{\mathcal S||\mathcal S|=m}} \Pr(Z_{\mathcal S}= v).$$ 

It is easy to see that $\mathbf F(p,v)=\mathbb E_{Z\sim p}\ {Z \choose v}$; in words, suppose $Z$ is sampled from a Bernoulli distribution parametrized by $p$, $\mathbf F(p,v)$ is the expected number of times $v$ appears as a subsequence of $Z$. Clearly if $p \in \{0,1\}^n$, then $Z=p$ with probability 1 and $\mathbf F(p,v) = {p \choose v}$.
More precisely, $\mathbf F(\cdot)$ is defined as:
\begin{definition}
\label{def:f}
\begin{align*}
&\mathbf F: [0,1]^n \times \{0,1\}^m \rightarrow \mathbb{R},\\
\mathbf F(p,  v)\triangleq &\begin{cases} 
      \sum\limits_{\substack{\mathcal S|\mathcal S\subseteq [n],\\|\mathcal S|=m}} \quad \prod\limits_{i=1}^m p_{\mathcal S_i}^{v_i} (1-p_{\mathcal S_i})^{1-v_i} & 1 \leq m\leq n \\
	  1 &  0=m\leq n \\
      0 & \text{else}.  
   \end{cases}
\end{align*}
%\noindent  Note that if $q$ is a vector of $0$'s and $1$'s, then $\mathbf F( q,  v)={q \choose v}$, the binomial coefficient of $v$ in $q$. Thus, $\mathbf F(\cdot)$ could be interpreted as an extension of the binomial coefficient where one of the parameters can take values in $[0,1]^n$ instead of $\{0,1\}^n$.
\end{definition}
Though at first sight $\mathbf F(p,v)$ sums over an exponential number of subsets, a dynamic programming approach can be used to compute it in $O(nm)$ time complexity (see Appendix~\ref{app:F_compute}).\\

\noindent \textbf{Decomposition of the $t$-trace deletion channel:}
 The following definitions and ideas are relevant only for Section \ref{sec:exactsmap} and can be omitted  for the sections on single-trace deletion channel. We first state a result of ours that aids in thinking about error events in multiple deletion channels.
%\subsection{An alternate interpretation of multiple deletion channel model}

The events occurring in the $t$-deletion channel model can be categorized into two groups:
\begin{enumerate}
\item an input symbol is deleted in \textit{all} the $t$-traces,
\item an input symbol is reflected in at least one of the traces.
\end{enumerate}
The error events of the first kind are in some sense ``not correctable'' or even ``detectable'' in any situation since it is impossible to tell with absolute certainty what and where the deleted symbol could have been (although the probabilities need not be uniform). The events of the second kind, however, can be detected and corrected in some situations. This thought process gives rise to a natural decomposition of the $t$-deletion channel model into a cascade of two channels: the first one being a deletion channel which captures error events of the first kind and the second one is what we call the \textit{remnant channel} which captures events of the second kind (see Fig.~\ref{fig:channel_equiv}). More precisely, we define the remnant channel as follows:
\begin{definition}
\textit{Remnant channel:} an input symbol to the remnant channel is reflected in $k>0$ given outputs and deleted in the rest with a probability $\frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}$. 
\end{definition}
It is easy to note that probability of the union of all possible events here is $\sum_{k=1}^t {t \choose k} \frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}=1$, validating our definition.

\begin{restatable}{theorem}{channelequiv}
\label{thm:channel_equiv}
The $t$-deletion channel model and the cascade of the deletion channel with remnant channel shown in Fig.~\ref{fig:channel_equiv} are probabilistically equivalent, i.e., 
$$\Pr({Y}^{(1)},{Y}^{(2)},...,{Y}^{(t)}|X = x) = \Pr(\tilde{Y}^{(1)},\tilde{Y}^{(2)},...,\tilde{Y}^{(t)}|X = x).$$
\end{restatable}
An algebraic proof of the theorem requires a few more definitions and is relegated to Appendix~\ref{app:channel_equiv}.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.4]{channel_equiv.pdf}
\caption{A channel equivalence result: the $t$-trace deletion channel model in (a) is probabilistically equivalent to the the cascade of a deletion channel with the \textit{remnant channel} ($ \mathcal C_2$) in (b).}
\label{fig:channel_equiv}
\end{center}
\end{figure}




\noindent\textbf{Edit graph} (\cite{Gusfield1997}): Similar graph constructs have been defined in related problems on common supersequences and subsequences (see \cite{Nicosia2001} for example). This graph is closely related to  the error events in the remnant channel. We start with a simple case and generalize subsequently. Define an \textit{edit graph} given two sequences $f$ and $g$, where every path connecting the ``origin'' to the ``destination'' on the edit graph yields a supersequence $h$ of $f,g$, where $h$ is ``covered'' by $f,g$ -- i.e.,  each symbol of $h$ comes from either $f$ or $g$ or
both. In other words, given that $f$ and $g$ are the outputs of the remnant channel (with two outputs), each path from the origin of the edit graph to the destination corresponds to a possible input $h$ to the remnant channel and to an error event  which resulted in outputs $f,g$ with  input $h$.


For $f$ and $g$ in $\mathcal
A^*$, we form a graph $\mathcal{G}(f,g)$ with $(|f|+1)(|g|+1)$
vertices each labelled with a distinct pair $(i,j), 0\leq i\leq
|f|,\ 0\leq j\leq |g|$. A directed edge
$(i_1,j_1)\rightarrow(i_2,j_2)$ exists iff at least one of the following
holds: 
%\vspace{-1mm}
\begin{enumerate}
\item$i_2-i_1=1$ and $j_1=j_2$, or
\item $j_2-j_1=1$ and $i_1=i_2$, or
\item  $i_2-i_1=1$, $j_2-j_1=1$ and $f_{i_2}=g_{j_2}$, 
\end{enumerate}
%\vspace{-1mm}
where $f_i$ is the $i^{th}$ symbol of the sequence $f$. The origin is the vertex $(0,0)$ and the destination $(|f|,|g|)$.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap1.pdf}
\caption{ Edit graph for sequences $f=$ `001' and $g=$ `101'. Make a grid so the vertical edges are aligned with a symbol in $f$ and horizontal edges with $g$ as shown. A diagonal edge $(i{-}1,j{-}1)\rightarrow (i,j)$ exists if $f_i = g_j$. The thick red edges form a path from the origin to the destination; this path corresponds to $h=$`0101' -- sequentially append the corresponding symbol to which each edge is aligned. It is also easy to verify that $h$ is a supersequence of both $f$ and $g$, and could be obtained as a covering of $f$ and $g$; the path itself gives one such covering. This covering also corresponds to an error event (or a deletion pattern) in the remnant channel which would result in outputs $f$ and $g$ with input $h=$ `0101' -- the deletion pattern is shown in the figure.}
\label{fig:editgraph_smap1}
\end{figure}

Let $p=((i_1,j_1),(i_2,j_2),...,(i_m,j_m))$ be a path in $\mathcal{G}(f,g)$. We define $ s(p)$ to be the sequence corresponding to the path. Intuitively, $s(p)$ is formed by appending symbols in the following
way: append the corresponding $f$ symbol for a vertical edge, $g$ symbol for horizontal edge, and $f$ or $g$ symbol for  diagonal edge (see example Fig.~\ref{fig:editgraph_smap1}). Any path from $(0,0)$ to $(|f|,|g|)$ corresponds to a supersequence of $f$ and $g$ and which is covered by $f$ and $g$. More formally, define $ s(p)\triangleq x_1x_2...x_{m-1}$ where    
$$x_k = 
     \begin{cases}
       f_{i_{k+1}} \quad\text{if }j_{k}=j_{k+1},\\ 
       g_{j_{k+1}} \quad\text{if }i_{k}=i_{k+1},\\
       f_{i_{k+1}} \quad\text{else.}
    \end{cases}	
$$


The construct of edit graph can be extended to more than 2 sequences with the same idea. For sequences $f_1,f_2,...,f_t$, construct a $t$-dimensional grid with a number of vertices $(|f_1|+1)(|f_2|+1)...(|f_t|+1)$ labeled from $(0,0,...,0)$ to $(|f_1|,|f_2|,...,|f_t|)$. A vertex $u=(i_1,i_2,...,i_t)$ is connected to $v=(j_1,j_2,...,j_t)$ (we say $u \rightarrow v$) iff both of the following conditions are met:
\begin{itemize}
\item $j_l=i_l$ or $j_l=i_l+1$ $\forall\ l\in [t]$, i.e., $(i_1,...,i_t)$ and $(j_1,...,j_t)$ are vertices of a particular unit cube. Only these type of vertices can share an edge in the grid graph.
\item  Let $\mathcal T \subseteq [t]$ be the collection of indices where $j_l=i_l+1$. Then ${f_l}_{j_l}$ is equal $\forall\ l \in \mathcal T$. For example in 4 dimensional grid, consider the two vertices $(10,5,8,2)$ and $(10,6,9,2)$. In this case $\mathcal T = \{2,3\}$ since the second and third coordinates differ by 1. Therefore $(10,5,8,2)\rightarrow (10,6,9,2)$ iff ${f_2}_{5}={f_3}_{9}$. Note that if only one coordinate differs by 1 in the two vertices, a directed edge always exists (in other words all non-diagonal edges exist).
\end{itemize}
Define the vertex $(0,...,0)$ to be the origin of this graph and the vertex $(|f_1|,...,|f_t|)$ to be the destination. If $|f_j|=O(n)\ \forall\ j$, this graph has a number of vertices $O(n^t)$ and a maximum number of edges $O((2n)^t)$ since each vertex has at most $2^t-1$ outgoing edges.\\


\noindent\textbf{Infiltration product} (introduced in \cite{lothaire1997combinatorics}):
The infiltration product has been extensively used in \cite{lothaire1997combinatorics}, as a tool in non-commutative algebra. Here, we give an edit-graph interpretation of this tool. A formal algebraic definition of the infiltration product is in Appendix~\ref{app:infil_def}. Using the edit graph we can construct the set of possible
supersequences $\mathcal{S}(f,g)$ of $f$, $g$ that are covered by the symbols in $f$ and $g$.
Clearly multiple paths could yield the same supersequence and we
can count the number of distinct ways  $\mathbf N(h;f,g)$ one can construct
the same supersequence $h$ from $f$, $g$.
We can  informally define the
\emph{infiltration product $f\uparrow g$} of $f$ and $g$, as a polynomial with monomials the supersequences $h$ in
$\mathcal{S}(f,g)$ and coefficients  $\langle f\uparrow g,h\rangle$ equal to $\mathbf N(h;f,g)$. For the example in Fig.~\ref{fig:editgraph_smap1}, it is easy to verify that there is exactly one path corresponding to `101001' and hence $\langle 001\uparrow 101,101001 \rangle=1$ and similarly $\langle 001\uparrow 101,01001 \rangle=2$. One could find these coefficients for all relevant sequences and form the polynomial as described. As additional examples, let $\mathcal{A}=\{a,b\}$, then
 %\vspace{-7pt}
\begin{itemize}[wide=2pt]
\item $ab\uparrow ab=ab+2aab+2abb+4aabb+2abab$,
\item $ab\uparrow ba=aba+bab+abab+2abba+2baab+baba.$
\end{itemize}
The  infiltration operation is commutative and associative, and infiltration of two sequences $f\uparrow g$ is a polynomial with variables of length (or \textit{degree}) at most $|f|+|g|$; see \cite{lothaire1997combinatorics}.
The definition of infiltration extends to two polynomials via distributivity (precisely defined in Appendix~\ref{app:infil_def}), and consequently to multiple sequences as well. For multiple sequences, infiltration has the same edit graph interpretation: $\langle f_1\uparrow f_2 \uparrow...\uparrow f_t, w \rangle$ is the number of distinct ways of constructing $w$ as a supersequence of $f_1, f_2, ... ,f_t$ so that the construction covers $w$, i.e., construct the $t$-dimensional edit graph of $f_1, f_2, ... ,f_t$ and count the number of paths corresponding to $w$.\\


%Note that infiltration is defined, in general, for two series, not just for two sequences.

\noindent \textbf{Summary of definitions and ideas introduced in this section:}
\begin{itemize}
\item The binomial coefficient captures the likelihood of observations for deletion channels. 
\item A real-valued extension of the binomial coefficient function is introduced; this function is pivotal to our results on the single-trace deletion channel.
\item For multiple deletion channels, the error events can be categorized into two groups -- one where an input symbol is deleted in all the traces, and second, the complement of this event. This categorization results in a natural decomposition of multiple deletion channel model into a cascade model involving the remnant channel.
\item The remnant channel disregards the error events where a symbol is deleted in all the traces.
\item The edit graph provides a way to visualize and construct all the possible error events and input sequences to a remnant channel given its outputs. 
\item The infiltration product serves the same purpose as the edit graph, but has an algebraic flavor and provides rigor for proofs and analysis. The edit graph, on the other hand, is more helpful in designing algorithms.
\end{itemize}



==> Sections/notation__Sundara_Rajan_s_conflicted_copy_2019-10-12_.tex <==

\section{Notation and Tools}
\label{sec:notations}
\noindent \textbf{Basic notations:} In this work, we borrow a majority of the notation and tools from \cite{lothaire1997combinatorics} which deals with non-commutative algebra. We restate the definitions here for convenience. Calligraphic letters refer to sets, capitalized letters
correspond to random variables and bold letters are used for functions.  Let $\mathcal{A}$ be the set of all
symbols. Throughout this work, we will focus on the case where $\mathcal{A}=\{0,1\}$,
though  our methods extend to arbitrarily large sets of finite size. Define
$\mathcal{A}^n$ to be the set of all $n$-length sequences and $\mathcal{A}^*$ to be the set of all finite length sequences with
symbols in $\mathcal{A}$. For a sequence $f$, $|f|$ denotes the length
of $f$. For integers $i,j$, we define $[i:j] \triangleq \{i,i+1,...,j\}$ if $j\geq i$ and $[i:j] \triangleq \emptyset$ otherwise. Also define $[i] \triangleq [1:i]$.\\

\noindent \textbf{Binomial coefficient:} Given sequences $f$ and $g$ in $\mathcal{A}^*$, the number of
subsequence patterns of $f$ that are equal to $g$ is called the
\textit{binomial coefficient} of $g$ in $f$ and is denoted by $f
\choose g$.  For example, ${'apple' \choose 'ape'} = 2$ since $'ape'$ can be obtained from two (overlapping) subsequences of $'apple'$.


When the alphabet $\mathcal{A}$ is of cardinality 1, ${f
  \choose g} = {|f| \choose |g|}$, the classical binomial coefficient
with their respective lengths as the parameters. This definition hence
could be thought of as a generalization of the classical binomial
coefficients. We will denote by $e$ the sequence of length 0, and {define ${f
  \choose e} \triangleq 1\ \forall\ f\ \in\ \mathcal{A}^*$.} We also define the classical binomial coefficient ${a \choose b}\triangleq 0,$ whenever $b>a$ or $b<0$ for ease of use.

The binomial coefficient is an integral aspect of this work and for analyzing error events in deletion channels because the input-output relation for a deletion channel (with deletion probability $\delta$, input $X$ and output $Y$) can be expressed as 
\begin{equation}
\label{eq:in-out_relation}
\Pr(Y=y|X=x) = {x \choose y} \delta^{|x|-|y|} (1-\delta)^{|y|}.
\end{equation}
The proof is straight-forward -- the number of distinct error events that give rise to $y$ from $x$ is exactly the number of  subsequences of $x$ which are equal to $y$. Each of these error events has a probability $\delta^{|x|-|y|} (1-\delta)^{|y|}$, wherein the exponent of $\delta$ corresponds to the deleted symbols and the exponent of  $1-\delta$ to the undeleted symbols. 

Given the definition of the binomial coefficient, the maximum-likelihood (ML) estimate over a deletion channel with observed output $Y$ can be cast in the following form:
\begin{align*}
\argmax_{x \in \mathcal C}  {x \choose Y},\numberthis
\label{eq:ML_deletion}
\end{align*}
where $\mathcal C$ is the chosen codebook. In the case of multiple deletion channels with observed traces $Y^{(1)},...,Y^{(t)}$, the ML formulation is similar:
\begin{align*}
\argmax_{x \in \mathcal C}  \prod_{j=1}^{t} {x \choose Y^{(j)}}.\numberthis
\label{eq:ML_multiple_deletion}
\end{align*}
As yet, there is no known efficient way to come up with a solution for the above two formulations, even for \eqref{eq:ML_deletion} with $\mathcal C = \{0,1\}^n$ (see \cite{mitzenmacher2009survey}). In this work, we attempt to take a step in this direction by showing that a continuous relaxation of \eqref{eq:ML_deletion} is equivalent to \eqref{eq:ML_deletion}. However, an efficient algorithm to solve the optimization \eqref{eq:ML_deletion} remains open. In the context of trace reconstruction, the ultimate pursuit would be an algorithm for \eqref{eq:ML_multiple_deletion} with $\mathcal C = \{0,1\}^n$ and error analysis thereof.


\noindent We now describe a function which can be thought of as a real-valued extension of the binomial coefficient. This function is used in sections~\ref{sec:1deletion_ML} and \ref{sec:1deletion}. Consider the function $\mathbf F(\cdot)$ defined as:
\begin{definition}
\label{def:f}
\begin{align*}
&\mathbf F: \mathbb{R}^k \times \{0,1\}^l \rightarrow \mathbb{R},\\
\mathbf F(q,  v)\triangleq &\begin{cases} 
      \sum\limits_{\substack{\mathcal S|\mathcal S\subseteq [k],\\|\mathcal S|=l}} \quad \prod\limits_{i=1}^l q_{\mathcal S_i}^{v_i} (1-q_{\mathcal S_i})^{1-v_i} & 1 \leq l\leq k \\
	  1 &  0=l\leq k \\
      0 & \text{else}.  
   \end{cases}
\end{align*}
\noindent An alternate definition is as follows: consider a random vector $Z\in\{0,1\}^k$ such that $Z_i\sim$ ind. Ber$(q_i)$, let $q$ be the vector of probabilities of length $k$, $\mathcal S\subseteq [k]$ a subset of the indices of size $l$, and ${v}$ a binary vector of length $l$. Then, $$\mathbf F(q,v)=\sum_{\substack{\mathcal S||\mathcal S|=l}} \Pr(Z_{\mathcal S}= v).$$ Note that if $q$ is a vector of $0$'s and $1$'s, then $\mathbf F( q,  v)={q \choose v}$, the binomial coefficient of $v$ in $q$. Thus, $\mathbf F(\cdot)$ could be interpreted as an extension of the binomial coefficient where one of the parameters can take values in $[0,1]^n$ instead of $\{0,1\}^n$.
\end{definition}
Though at first sight, $\mathbf F(q,v)$ sums over an exponential number of subsets, a dynamic programming approach can be used to compute it in $O(|v|^2)$ time complexity. The dynamic program is described in section~\ref{sec:1deletion}.

\iffalse
%\subsection{Definitions and preliminary results}
\noindent \textbf{Edit distance:} The edit distance  $d_e(f,g)$  measures similarity between two sequences of
possibly different lengths \cite{Navarro2001}. $d_e(f,g)$ is the minimum number of operations
needed to transform $f$ to $g$, where the permitted operations are
insertion, deletion or substitution of a symbol. In this work, we
quantify the performance of algorithms in Section \ref{sec:Numerics}
using the edit distance metric.

\fi

The following definitions and ideas are relevant only for \ref{sec:exactsmap} and can be omitted  for the sections on single deletion channel. Before getting to the mathematical definitions, we first state a result of ours that aids in thinking about error events in multiple deletion channels. 

\subsection{An alternate interpretation of multiple deletion channel model}

The events occurring in the $t$-deletion channel model can be categorized into two groups:
\begin{enumerate}
\item an input symbol is deleted in \textit{all} the $t$-traces,
\item an input symbol is reflected in at least one of the traces.
\end{enumerate}
The error events of the first kind are in some sense ``not correctable" or even ``detectable" since it is impossible to tell what and where the deleted symbol could have been (although the probabilities need not be uniform). The events of the second kind, however, can still be detected although they could likely be confused with a large set of similar events. This thought process gives rise to a natural decomposition of the $t$-deletion channel model into a cascade of two channels: the first one being a deletion channel which captures error events of the first kind and the second one is what we call the \textit{remnant channel} which captures events of the second kind (see Fig.~\ref{fig:channel_equiv}). More precisely, the remnant channel is defined as follows:
\begin{definition}
\textit{Remnant channel:} an input symbol to the remnant channel is reflected in $k>0$ given outputs and deleted in the rest with a probability $\frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}$. 
\end{definition}
It is easy to note that probability of the union of all possible events here is $\sum_{k=1}^t {t \choose k} \frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}=1$, validating our definition.

\begin{restatable}{theorem}{channelequiv}
\label{thm:channel_equiv}
The $t$-deletion channel model and the cascade of the deletion channel with remnant channel shown in Fig.~\ref{fig:channel_equiv} are probabilistically equivalent, i.e., 
$$\Pr({Y}^{(1)},{Y}^{(2)},...,{Y}^{(t)}|X = x) = \Pr(\tilde{Y}^{(1)},\tilde{Y}^{(2)},...,\tilde{Y}^{(t)}|X = x).$$
\end{restatable}
The formal proof of the theorem requires few more definitions and is relegated to the appendix.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.4]{channel_equiv.pdf}
\caption{A channel equivalence result: the $t$-deletion channel model in (a) is probabilistically equivalent to the the cascade of a deletion channel with the \textit{remnant channel} ($ \mathcal C_2$) in (b).}
\label{fig:channel_equiv}
\end{center}
\end{figure}




\noindent\textbf{Edit graph} (as defined in \cite{Gusfield1997}): We now define a graph construct which is closely related to  the error events in the remnant channel. We start with a simple case and generalize subsequently. Define an \textit{edit graph} given two sequences $f$ and $g$, where every path connecting the ``origin'' to the ``destination'' on the edit graph yields a supersequence $h$ of $f,g$, where $h$ is ``covered'' by $f,g$ -- i.e.,  each symbol of $h$ comes from either $f$ or $g$ or
both. In other words, given that $f$ and $g$ are the outputs of the remnant channel (with two outputs), each path from the origin of the edit graph to the destination corresponds to a possible input $h$ to the remnant channel and to an error event  which resulted in $f$ and $g$ with  input $h$.


For $f$ and $g$ in $\mathcal
A^*$, we form a graph $\mathcal{G}(f,g)$ with $(|f|+1)(|g|+1)$
vertices each labelled with a distinct pair $(i,j), 0\leq i\leq
|f|,\ 0\leq j\leq |g|$. A directed edge
$(i_1,j_1)\rightarrow(i_2,j_2)$ exists iff at least one of the following
holds: 
%\vspace{-1mm}
\begin{enumerate}
\item$i_2-i_1=1$ and $j_1=j_2$, or
\item $j_2-j_1=1$ and $i_1=i_2$, or
\item  $i_2-i_1=1$, $j_2-j_1=1$ and $f_{i_2}=g_{j_2}$, 
\end{enumerate}
%\vspace{-1mm}
where $f_i$ is the $i^{th}$ symbol of the sequence $f$. The origin is the vertex $(0,0)$ and the destination $(|f|,|g|)$.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap1.pdf}
\caption{ Edit graph for sequences $f=$ `001' and $g=$ `101'. An easy way to think about this is to write down $f$ vertically with each symbol aligned to a vertical set of edges and $g$ horizontally likewise. A diagonal edge in a small square exists if the corresponding $f$ and $g$ symbols are equal. The thick red edges form a path from the origin to the destination; this path corresponds to the sequence `0101' -- append the corresponding symbol at the left of an edge if it's vertical or diagonal, otherwise append the symbol at the top. It is also easy to verify that 0101 is a supersequence of both $f$ and $g$, and could be obtained as a covering of $f$ and $g$; the path itself gives one such covering. This covering also corresponds to an error event in the remnant channel which would result in outputs $f$ and $g$ with input $h=$ `0101' -- more precisely, the error event is one in which the first symbol of $h$ is deleted only in $g$, the second symbol is deleted only in $f$ and the third and fourth symbols not deleted in either $f$ or $g$.}
\label{fig:editgraph_smap1}
\end{figure}

Let $p=((i_1,j_1),(i_2,j_2),...,(i_m,j_m))$ be a path in $\mathcal{G}(f,g)$. We define $ s(p)$ to be the sequence corresponding to the path. Intuitively, $s(p)$ is formed by appending symbols in the following
way: append the corresponding $f$ symbol for a vertical edge, $g$ symbol for horizontal edge, and $f$ or $g$ symbol for  diagonal edge (see example Fig.~\ref{fig:editgraph_smap1}). Any path from $(0,0)$ to $(|f|,|g|)$ corresponds to a supersequence of $f$ and $g$ and which is ``covered" by $f$ and $g$. More formally, define $ s(p)\triangleq x_1x_2...x_{m-1}$ where    
$$x_k = 
     \begin{cases}
       f_{i_{k+1}} \quad\text{if }j_{k}=j_{k+1},\\ 
       g_{j_{k+1}} \quad\text{if }i_{k}=i_{k+1},\\
       f_{i_{k+1}} \quad\text{else.}
    \end{cases}	
$$


The construct of edit graph can be extended to more than 2 sequences with the same idea. For sequences $f_1,f_2,...,f_t$, construct a $t$-dimensional grid with a number of vertices $(|f_1|+1)(|f_2|+1)...(|f_t|+1)$ labeled from $(0,0,...,0)$ to $(|f_1|,|f_2|,...,|f_t|)$. A vertex $u=(i_1,i_2,...,i_t)$ is connected to $v=(j_1,j_2,...,j_t)$ (we say $u \rightarrow v$) iff both of the following conditions are met:
\begin{itemize}
\item $j_l=i_l$ or $j_l=i_l+1$ $\forall\ l\in [t]$, i.e., $(i_1,...,i_t)$ and $(j_1,...,j_t)$ are vertices of a particular unit cube. Only these type of vertices can share an edge in the grid graph.
\item Let $\mathcal T \subseteq [t]$ be the collection of indices where $j_l=i_l+1$. Then $f_{i_l}$ is same $\forall\ l \in \mathcal T$. For instance, if $\mathcal T=\{1,3,5\}$, then $f_{i_1}=f_{i_3}=f_{i_5}$.
\end{itemize}
Define the vertex $(0,...,0)$ to be the origin of this graph and the vertex $(|f_1|,...,|f_t|)$ to be the destination. If $|f_j|=O(n)\ \forall\ j$, this graph has a number of vertices $O(n^t)$ and a maximum number of edges $O((2n)^t)$ since each vertex has at most $2^t$ outgoing edges.\\


\noindent\textbf{Infiltration product} (introduced in \cite{lothaire1997combinatorics}):
The infiltration product has been extensively used in \cite{lothaire1997combinatorics}, as a tool in non-commutative algebra. Here we give an edit-graph interpretation of this tool. We also give a formal definition later in this section. Using the edit graph we can construct the set of possible
supersequences $\mathcal{S}(f,g)$ of $f,g$ which are covered by
it. Clearly multiple paths could yield the same supersequence and we
can count the number of distinct ways  $\mathbf N(h;f,g)$ one can construct
the same supersequence $h$ from $f,g$.
We can  informally define the
\emph{infiltration product $f\uparrow g$} of $f$ and $g$, as a polynomial with monomials the supersequences $h$ in
$\mathcal{S}(f,g)$ and coefficients  $\langle f\uparrow g,h\rangle$ equal to $\mathbf N(h;f,g)$. In Fig.~\ref{fig:editgraph_smap1}, it is easy to verify that there is exactly one path corresponding to `101001' and hence $\langle 001\uparrow 101,101001 \rangle=1$ and similarly $\langle 001\uparrow 101,01001 \rangle=2$. One could find these coefficients for all relevant sequences and form the polynomial as described. More examples: Let $\mathcal{A}=\{a,b\}$, then
 %\vspace{-7pt}
\begin{itemize}[wide=2pt]
\item $ab\uparrow ab=ab+2aab+2abb+4aabb+2abab$,
\item $ab\uparrow ba=aba+bab+abab+2abba+2baab+baba.$
\end{itemize}
The  infiltration operation is commutative and associative, and infiltration of two sequences $f\uparrow g$ is a polynomial with variables of length (or \textit{degree}) at most $|f|+|g|$; see \cite{lothaire1997combinatorics}.
The definition of infiltration extends to two polynomials via distributivity (precisely defined in later), and consequently to multiple sequences as well. For multiple sequences, infiltration has the same edit graph interpretation: $\langle f_1\uparrow f_2 \uparrow...\uparrow f_t, w \rangle$ is the number of distinct ways of constructing $w$ as a supersequence of $f_1, f_2, ... ,f_t$ so that the construction covers $w$, i.e., construct the $t$-dimensional edit graph of $f_1, f_2, ... ,f_t$ and count the number of paths corresponding to $w$.

\subsection{Formal definition of infiltration product}
 We now give a more formal definition of the infiltration product (see \cite{lothaire1997combinatorics} for the equivalence of the two definitions and a more rigorous treatment). A \textit{formal series} with indeterminates (or variables) in a set $\mathcal A$ and coefficients in a commutative ring $\mathcal R$, is a mapping of $\mathcal A^*$ onto $\mathcal R$. Recall that a commutative ring is a set which forms an abelian group under an \textit{addition} operation, is a monoid under a \textit{multiplication} operation which commutes, and the multiplication operation distributes over addition. Here we consider $\mathbb Z$, the set of integers as the commutative ring  $\mathcal{R}$. A formal series is called a \textit{polynomial} if only a finite number of sequences are mapped to non-zero values, the rest of the sequences map to zero. Consider two polynomials $\sigma,\tau: \mathcal{A}^*\rightarrow \mathbb Z$. The value taken by a sequence $w\in \mathcal A^*$ on $\sigma$ (or the coefficient of $w$ in $\sigma$) is denoted by $\langle \sigma,w\rangle \in \mathbb R$. We also define binary addition ($\oplus$) and multiplication operations ($\times$) on the set of polynomials as follows:
\begin{align}
\langle \sigma\oplus \tau,w\rangle \triangleq \langle \sigma,w\rangle +  \langle \tau,w \rangle \quad \forall w\in \mathcal A^*,\label{eq:polynomial_add}\\
\langle \sigma\times \tau,w\rangle \triangleq \sum_{\substack{f,g\in \mathcal A^*:\\ f.g=w}}\langle \sigma,f\rangle  \langle \tau,g \rangle \quad \forall w\in \mathcal A^*.\label{eq:polynomial_prod}
\end{align}
We will use the usual symbols $+$ and $.$ in place of $\oplus$ and $\times$ in this work for convenience. The meaning of the operation would be clear depending on the operands. With these operations the set of polynomials form a non-commutative ring, and is denoted by $\mathbb Z\langle\mathcal A \rangle$, also called the free $\mathbb Z$-algebra on $\mathcal A$ in ring theory. Note that the addition and multiplication operations defined in \eqref{eq:polynomial_add} and \eqref{eq:polynomial_prod} are similar to the operations defined on commutative polynomials, except that the multiplication  operation under the summation in \eqref{eq:polynomial_prod} ($f.g=w$) is actually concatenation and is non-commutative.   The multiplication inside the summation in \eqref{eq:polynomial_prod} is multiplication in the real field and hence commutative. It is also easy to prove that the multiplication defined in \eqref{eq:polynomial_prod} distributes over addition defined in \eqref{eq:polynomial_add}. Thus, a polynomial in $\mathbb Z\langle\mathcal A \rangle$ can be represented as a sum of monomials in $\mathcal A^*$ each with an associated coefficient in $\mathbb Z$, i.e., $\sigma=\sum\limits_{w\in \mathcal A^*} \langle\sigma,w \rangle w$. Define the \textit{degree} of a polynomial to be equal to the length of a longest sequence with a non-zero coefficient in the polynomial and the \textit{number of terms} of a polynomial as the number of sequences with non-zero coefficients in the polynomial. Note that a degree $d$ polynomial could have a number of terms upto $2^{d+1}-1$.
 
With this, the \textit{infiltration product} (in general, for two polynomials) is defined as follows:

\begin{align}
\forall f\in \mathcal{A}^*,& \quad f\uparrow e = e\uparrow f=f.\nonumber \\
\forall f,g\in \mathcal{A}^*&,\quad  \forall a,b\in \mathcal{A}, \nonumber\\
fa\uparrow gb=(f\uparrow gb)a&+(fa\uparrow g)b+\mathbbm{1}_{a=b}(f\uparrow g)a.\nonumber \\
\forall \sigma,\tau \in \mathbb{Z}\langle\mathcal{A} \rangle, \quad &\sigma\uparrow \tau=\sum_{f,g\in \mathcal{A}^*} \langle \sigma,f \rangle \langle \tau,g \rangle (f\uparrow g). \label{def:infiltforseq}
\end{align}

%Note that infiltration is defined, in general, for two series, not just for two sequences.

\textbf{Summary of definitions and ideas introduced in this section:}
\begin{itemize}
\item The binomial coefficient captures the likelihood of observations for deletion channels. 
\item An extension of the binomial coefficient function where one of the parameters can take real values has been introduced; this function is pivotal for our results on the single-trace deletion channel.
\item For multiple deletion channels, the error events can be categorized into two groups -- one where an input symbol is deleted in all the traces, and second, the complement of this event. This categorization results in a natural decomposition of multiple deletion channel model into a cascade model involving the remnant channel.
\item The remnant channel disregards the error events where a symbol is deleted in all the traces.
\item The edit graph provides a way to visualize all the possible error events and input sequences to a remnant channel given its outputs. 
\item The infiltration product serves the same purpose as the edit graph, but has an algebraic flavor and provides rigor for proofs and analyses. The edit graph, on the other hand, is more helpful in designing reconstruction algorithms over deletion channels.
\end{itemize}



==> Sections/numerical.tex <==

\section{Numerical results}
\label{sec:Numerics}

In this section we show numerics supporting our theoretical results. The metric we use to measure the performance of different reconstruction algorithms is \textit{Hamming error rate}, which is defined as the average Hamming distance (the Hamming distance between the actual and estimated input sequence divided by the input sequence length).\\

\noindent \textbf{Single-trace deletion channel.}
\begin{itemize}[leftmargin=3mm]
\item Fig.~\ref{fig:numerics_single1} compares the error rate for reconstruction via ML heuristic (Alg.~\ref{alg:cood_switch}) when the initialization is a random lattice point and when the initialization is a random interior point, and also the symbolwise MAP via Alg.~\ref{alg:apprx_smap_dp} for a small blocklength $n=10$. For Alg.~\ref{alg:cood_switch}, we start with 5 random initializations and choose the one that gives the maximum objective value. As can be seen, initialization with an interior point far outperforms initialization with lattice point, thus validating the usefulness of our relaxation.
%
%\item Fig.~\ref{fig:numerics_single2} compares the error rate for reconstruction via ML heuristic (Alg.~\ref{alg:cood_switch}) with random interior point initializations with the symbolwise MAP via Alg.~\ref{alg:apprx_smap_dp} for a blocklength of $n=100$. For Alg.~\ref{alg:cood_switch}, we start with 5 random initializations and choose the one that gives the maximum objective value. We observe that the symbolwise MAP far outperforms the ML heuristic. This is expected since Alg.~\ref{alg:apprx_smap_dp} is an exact algorithm while Alg.~\ref{alg:cood_switch} is a heuristic. Moreover, the performance of Alg.~\ref{alg:cood_switch} relies on the number of random initializations (we use 5 here) and it is fair to expect that larger blocklengths could warrant more random initializations.
\end{itemize}

\begin{figure}[t!]
\centering
\includegraphics[scale=0.48]{ml_int_vs_ver_error.eps}
\caption{Hamming error rate for reconstruction via coordinate switch ML heuristic (Alg.~\ref{alg:cood_switch}) when the initialization is a random lattice point and when the initialization is a random interior point, and reconstruction via symbolwise MAP (Alg.~\ref{alg:apprx_smap_dp}) for a blocklength $n=10$.}
\label{fig:numerics_single1}
\end{figure}
%\begin{figure}[h!]
%\centering
%\includegraphics[scale=0.48]{ml_heur_vs_MAP.pdf}
%\label{fig:numerics_single2}
%\caption{Blocklenth $n=100$.}
%\label{fig:numerics_single2}
%\end{figure}

\vspace{10pt} \noindent \textbf{$t$-trace deletion channel model.}

Fig.~\ref{fig:numerics1} and Fig.~\ref{fig:numerics2} show results comparing reconstruction via symbolwise MAP for $t$-trace deletion channel model (Alg.~\ref{alg:exact_smap}), reconstruction via sequentially updating posterior probabilities over the traces (Alg.~\ref{alg:apprx_smap}),  reconstruction via independently combining posteriors  from each of the traces (described as Alg.~\ref{alg:ind_comb}) and a trace reconstruction algorithm from \cite{Batu2004} called the \textit{Bitwise Majority Alignment (BMA)} reproduced here as Alg.~\ref{alg:bitwise_majority}. We next make two observations, related to two of these algorithms.

\noindent \textbf{Independent posterior combination:} As pointed in the introduction, computing the posterior probabilities for  each deletion channel and combining them as if they came from independent observations does not provide a natural solution for computing the posterior probabilities for the $t$-trace deletion channel. One could, however, check how such a naive combination of posteriors compares with our reconstruction algorithms for $t$-traces.

\noindent \textbf{Bitwise Majority Alignment:} BMA reconstructs the input sequence by first ``aligning'' the traces using a pointer for each trace, and then taking the majority of the pointed symbols. We note that the state-of-the-art trace reconstruction algorithms in the literature are applicable in the asymptotic regime where the blocklength $n$ and the number of traces $t$ approach $\infty$; it is not clear how to adapt such algorithms for a finite blocklength and a small number of traces.

\begin{algorithm}[t!]
\caption{Trace reconstruction via independent posterior combination}\label{alg:ind_comb}
\begin{algorithmic}[1]
\item Input: Traces {$Y^{(1)},...,Y^{(t)}$}, input length $n$ \\ Outputs: Estimate of the input $\hat X$
\State Initialize priors $p^{old} \gets (0.5,0.5,...,0.5)$
\For {$l=1:t$}
\State Use Alg.~\ref{alg:apprx_smap_dp} with $p^{old}$ and $Y^{(l)}$ to compute posteriors $p^{(l),new}$
\EndFor
\For {$i=1:n$}
\If {$\prod_{l=1}^t p^{(l),new}_i \geq \prod_{l=1}^t (1-p^{(l),new}_i)$}
 $\ \hat X_i \gets 1$
\Else
 $\ \hat X_i \gets 0$
\EndIf
\EndFor
\State \textbf{return} $\hat X_1 \hat X_2 ... \hat X_n$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[!t]
\caption{Bitwise Majority Alignment} 
\label{alg:bitwise_majority}
\begin{algorithmic}[1]
\item Input: Traces {$Y^{(1)},Y^{(2)},...,Y^{(t)}$, input length $n$}\\ Output: estimate of input $\hat X = \hat X_1 \hat X_2...\hat X_n$.
\State Initialize $c_j=1$ for $j\in [t]$.
\State Initialize $\hat X_i = 1$ for $i \in [n]$.
\For{$i \in\ [0:n]$}
\State Let $b$ be the majority over all $t$ of $Y^{(j)}_{c_j}$
\State $\hat X_i \gets b$
\State Increment $c_j$ for each $j$ such that $Y^{(j)}_{c_j} = b$ 
\EndFor
\State \textbf{return} $\hat X_1 \hat X_2 ... \hat X_n$
\end{algorithmic}
\end{algorithm}


Our numerical evaluation results are as follows.
\begin{itemize}[leftmargin=3mm]
\item Fig.~\ref{fig:numerics1} compares symbolwise MAP for the $t$-trace deletion channel model (Alg.~\ref{alg:exact_smap}), trace reconstruction heuristic via sequentially updating posterior probabilities (Alg.~\ref{alg:apprx_smap}) with BMA (Alg.~\ref{alg:bitwise_majority}) for a small blocklength $n=10$. As seen, both of our algorithms significantly outperform BMA. Moreover,  the heuristic Alg.~\ref{alg:apprx_smap} is not much worse than Alg.~\ref{alg:exact_smap}, at least for this blocklength. Note that  Alg.~\ref{alg:apprx_smap} is polynomial in $n$ and $t$ ($O(tn^2)$) while Alg.~\ref{alg:exact_smap}  is exponential in $t$ ($O(2^tn^{t+2})$).

\item Fig.~\ref{fig:numerics2} compares the reconstruction heuristic via sequentially updating posterior probabilities (Alg.~\ref{alg:apprx_smap}) with reconstruction via independently combining posteriors  from each of the traces (Alg.~\ref{alg:ind_comb}) and BMA (Alg.~\ref{alg:bitwise_majority}), over a larger blocklength of $n=100$. Clearly, Alg.~\ref{alg:apprx_smap} outperforms both the others, indicating that it is an interesting heuristic for trace reconstruction.
\begin{figure}[t!]
\centering
 \includegraphics[width=16cm]{errors_BL10.eps}
 \caption{Hamming error rate  comparison for symbolwise MAP for the $t$-trace deletion channel model (Alg.~\ref{alg:exact_smap}), trace reconstruction heuristic via sequentially updating posterior probabilities (Alg.~\ref{alg:apprx_smap}) with BMA (Alg.~\ref{alg:bitwise_majority}) for a blocklength $n=10$.}
 \label{fig:numerics1}
\end{figure}

\item We note that with the number of traces, though the performance of all algorithms improves, the returns tend to diminish. This intuitively makes sense because not all the information in each additional trace is ``new''; some of it is already conveyed by  existing traces.
\item Even when the deletion probability is $\delta = 0.5$, the error rate is still less than $0.5$. This is not unexpected since the observed deleted sequence still carries some information about each of the input bits.
\end{itemize}


 \begin{figure}[t!]
\centering
 \includegraphics[width=16cm]{errors_BL100.eps}
 \caption{Hamming error rate comparison for reconstruction heuristic via sequentially updating posterior probabilities (Alg.~\ref{alg:apprx_smap}) with reconstruction via independently combining posteriors  from each of the traces (Alg.~\ref{alg:ind_comb}) and BMA (Alg.~\ref{alg:bitwise_majority}) for a larger blocklength of $n=100$.}
 \label{fig:numerics2}
\end{figure}




==> Sections/single.tex <==


\section{Symbolwise posterior probabilities for the single-trace deletion channel}
\label{sec:1deletion}

We here develop an algorithm to compute the symbolwise posterior probabilities for the single-trace deletion channel when the input symbols are independently generated with arbitrary priors. Consider the single deletion channel model in Fig.~\ref{fig:1deletion}, where $X=X_1...X_n$, each input symbol is generated $X_i \sim \text{ind. Ber}\ (p_i)$, and we observe at the output the trace $Y = Y_1Y_2...Y_m$ with $m\leq n$. Define the vector of priors as  $p\triangleq(p_1,p_2,...,p_n)$. We first give an $O(n^2)$ algorithm to calculate the posterior probabilities $\Pr(X_i=1|Y)$, which in turn provides the symbolwise MAP estimate for the considered model. We then show how this algorithm can be used for trace reconstruction. We take three steps to present the algorithm.


\noindent \textbf{An expression for $\Pr(X_i=1|Y)$.} 
Let $\Pr(X_i=1)=p_i$. As a first step, we have
\vspace{6pt}
\begin{align*}
\Pr(X_i=1|{Y}) &= \frac{\Pr(X_i=1,Y)}{\Pr(Y)}
 = \frac{ \sum\limits_{\substack{ x| x_i=1}}  \Pr({X=x}) \Pr(Y|X=x)}{ \sum_{\substack{x}}  \Pr({X=x}) \Pr(Y|X=x)} \\
 &\overset{(a)}{=} \frac{ \sum\limits_{\substack{ x| x_i=1}}  \Pr({X=x}) { x \choose  Y}}{ \sum_{\substack{x}}  \Pr({X=x}) { x \choose  Y}}, \numberthis
\label{eq:approx_smap_1}
\end{align*}
where $(a)$ is because for a deletion channel $\Pr(Y|X=x)={x \choose Y} \delta^{|x|-|Y|}(1-\delta)^{|Y|}$.
To proceed, we need to evaluate the summation in the numerator and the denominator.
Theorem~\ref{thm:approx_smap_postprob} expresses \eqref{eq:approx_smap_1} in terms of relaxed binomial coefficient terms $\mathbf F(\cdot)$. Recall one  way to define $\mathbf F(p,Y) \triangleq \mathbb E_{X\sim p} {X \choose Y}$, which is the denominator term in \eqref{eq:approx_smap_1}.
%======================================================================================

\begin{theorem}
\label{thm:approx_smap_postprob}
Let $X=X_1...X_n$ where $X_i \sim \text{ind. Ber}\ (p_i)$, and let $Y$ be the observed trace when $X$ is passed through a deletion channel. Then,
\begin{align*}
\Pr(X_i&=1|{Y}) = \frac{p_i}{\mathbf F( p,  Y)} \left( \mathbf F( p_{[n]\backslash \{i\}},  Y) +  \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) \right) \numberthis
\label{eq:smap_postprob_thm}
\end{align*}
where $\mathbf F(\cdot)$ is as given in Definition~\ref{def:f}.
\end{theorem}

\begin{proof}
The proof of this theorem employs the same trick used in the proof of Lemma~\ref{lemma:F_decomposition}.  Let $|Y|=m$. From \eqref{eq:approx_smap_1}
\begin{align*}
\Pr(X_i = 1 | Y) = \frac{ \sum\limits_{\substack{ x| x_i=1}} \Pr({X=x}) { x \choose  Y}}{\mathbf F(p,Y)}.
\end{align*}
Now,
\begin{align*}
\sum_{\substack{ x| x_i=1}} & \Pr({X=x}) { x \choose  Y}
=\sum_{\substack{ x|x_i=1}} \Pr({X=x}) \sum_{\substack{\mathcal S\subseteq [n]\\ |\mathcal S|=m}} \mathbbm{1}\{ x_{\mathcal S}= Y\}\\
&=\sum_{\substack{\mathcal S\subseteq [n]\\ |\mathcal S|=m}} \sum_{\substack{ x|x_i=1\\x_{\mathcal S}=Y}}  \Pr({X=x}).\numberthis \label{eq:smapiter1}
\end{align*}
We first separate the outer summation into two cases: (a)  $\mathcal S|i \notin \mathcal S$ and (b)  $\mathcal S|i\in \mathcal S$.
%\begin{figure}[!th]
%\centering
%\includegraphics[scale=0.4]{Smapiterfig.pdf}
%\caption{ Figure illustrating the intuition to simplify \eqref{eq:smapiter1}. The double summation can be thought of as first fixing a subset $S$ of $[n]$, and then summing over all $n$ length sequences whose  $i^{th}$ bit is $1$ and whose subsequence corresponding to the indices in  $S$ is $ Y$. The mapping of $ Y$ onto $S$ is illustrated through the arrows; a key point here is that no two arrows intersect.  Consider (a), when $i\notin S$ -- no arrow from $Y$ goes to $x$. In (b),  $Y_k$  for some $k$ ($S_k=i$ equivalently) maps to $x_i$. Note that this is possible only if $Y_k=1$. For no two arrows to cross, $ Y_{[1:k-1]}$ is mapped into $ x_{[1:i-1]}$ and $ Y_{[k+1:m]}$ is mapped into $ x_{i+1:n}$. This is equivalent to splitting $S$ into three parts; $S'\subseteq [1:i-1]:|S'|=k-1$, $S_k=i$ and $S''\subseteq [i+1:n]:|S''|=m-k$.}
%\label{fig:approx_smap_fig}
%\end{figure}
We can express the first case as
\begin{align*}
&\hspace{-1cm}\sum_{\substack{\mathcal S\subseteq [n] \\ |\mathcal S|=m,i\notin \mathcal S}}\sum_{\substack{ x|x_i=1\\x_{\mathcal S}=Y}}  \Pr({X=x})
=\sum_{\substack{\mathcal S\subseteq [n]\backslash \{i\}\\ |\mathcal S|=m}} \sum_{\substack{ x|x_i=1\\x_{\mathcal S}=Y}}  \Pr({X=x})\\
&=\sum_{\substack{S\subseteq [n]\backslash \{i\}\\ |\mathcal S|=m}} \sum_{\substack{ x|x_i=1\\  x_{\mathcal S}= Y}} \Big(\Pr(X_i=1)\Pr( X_{\mathcal S}= Y)    \Pr( X_{[n]\backslash \mathcal S\cup\{i\}}= x_{[n]\backslash \mathcal S\cup\{i\}}) \Big)\\  
&=\sum_{\substack{\mathcal S\subseteq [n]\backslash \{i\}\\ |\mathcal S|=m}} p_i \Pr( X_{\mathcal S}= Y)  \left(\sum_{\substack{ x|x_i=1\\  x_{\mathcal S}= Y}}   \Pr( X_{[n]\backslash \mathcal S\cup\{i\}}= x_{[n]\backslash \mathcal S\cup\{i\}})\right)\\ 
&=\sum_{\substack{\mathcal S\subseteq [n]\backslash \{i\}\\ |\mathcal S|=m}} p_i \Pr( X_{\mathcal S}= Y) \left(\sum_{(x_j|j\in [n]\backslash \mathcal S\cup \{i\})}   \Pr( X_{[n]\backslash \mathcal S\cup\{i\}}= x_{[n]\backslash \mathcal S\cup\{i\}})\right)\\
&=p_i \sum_{\substack{\mathcal S\subseteq [n]\backslash \{i\}\\ |\mathcal S|=m}}  \Pr( X_{\mathcal S}= Y) = p_i \mathbf F( p_{[n]\backslash \{i\}},  Y).\numberthis \label{eq:lemma3proof1}
\end{align*}

For the second term, we express the set $\mathcal S$ as a union  $\mathcal S = \mathcal S' \cup \{i\} \cup \mathcal S''$ such that $\mathcal S' \subseteq [i-1]$ and $\mathcal S'' \subseteq [i+1:n]$ to get:
\begin{align*}
&\sum_{\substack{\mathcal S\subseteq [n]\\ |\mathcal S|=m,\\i\in \mathcal S}} \sum_{\substack{ x|x_i=1\\x_{\mathcal S}=Y}}  \Pr({X=x})= \sum_{k=1}^m\sum\limits_{\substack{\mathcal S\subseteq [n],\\|\mathcal S|=m,\\ \mathcal S_k = i}} \sum_{\substack{ x|x_i=1\\x_{\mathcal S}=Y}}  \Pr({X=x})\\
&=\sum_{k=1}^m\sum_{\substack{\mathcal S'\subseteq [i-1]\\ |\mathcal S'|=k-1}}\sum_{\substack{\mathcal S''\subseteq [i+1:n]\\ |\mathcal S''|=m-k}} \sum_{\substack{ x|x_i=1\\x_{\mathcal S}=Y}}\mathbbm{1}_{\{Y_k=1\}}   \Pr({X=x}) \\
&=\sum_{k:Y_k=1}\sum_{\substack{\mathcal S'\subseteq [i-1]\\ |\mathcal S'|=k-1}}\sum_{\substack{\mathcal S''\subseteq [i+1:n]\\ |\mathcal S''|=m-k}} \sum_{\substack{ x|x_i=1\\  x_{\mathcal S'}= Y_{[1:k-1]}\\ x_{\mathcal S''}= Y_{[k+1:m]}}} \Bigg ( \Pr(X_i=1) \Pr( X_{\mathcal S'}= Y_{[1:k-1]})  
	\Pr( X_{\mathcal S''}= Y_{[k+1:m]}) \\&\hspace{7cm} \Pr( X_{[n]\backslash \mathcal S'\cup \mathcal S''\cup \{i\}}= x_{[n]\backslash \mathcal S'\cup \mathcal S'' \cup\{i\}})\Bigg )\\
	&=p_i\sum_{k:Y_k=1}\Bigg ( \Big( \sum_{\substack{\mathcal S'\subseteq [i-1]\\ |\mathcal S'|=k-1}}\Pr( X_{\mathcal S'}= Y_{[1:k-1]})\Big) \Big(\sum_{\substack{\mathcal S''\subseteq [i+1:n]\\ |\mathcal S''|=m-k}}\Pr( X_{\mathcal S''}= Y_{[k+1:m]})\Big ) \\
 & \hspace{5cm} \Big( \sum_{\substack{ x|x_i=1\\  x_{\mathcal S'}= Y_{[1:k-1]}\\ x_{\mathcal S''}= Y_{[k+1:m]}}} \Pr( X_{[n]\backslash \mathcal S'\cup \mathcal S''\cup \{i\}}= x_{[n]\backslash \mathcal S'\cup \mathcal S'' \cup\{i\}})\Big) \Bigg )\\ 
	&=p_i\sum_{k|Y_k=1}\Bigg(\Big( \sum_{\substack{\mathcal S'\subseteq [i-1]\\ |\mathcal S'|=k-1}}\Pr( X_{\mathcal S'}= Y_{[1:k-1]})\Big)	\Big( \sum_{\substack{\mathcal S''\subseteq [i+1:n]\\ |\mathcal S''|=m-k}}\Pr( X_{\mathcal S''}= Y_{[k+1:m]}) \Big)\Bigg)\\
	&=p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}). \numberthis \label{eq:lemma3proof2}
\end{align*}
Plugging in \eqref{eq:lemma3proof1} and \eqref{eq:lemma3proof2} in \eqref{eq:approx_smap_1} proves the theorem.
\end{proof}


Alg.~\ref{alg:apprx_smap_dp} summarizes the computation of $\Pr(X_i=1|Y)$. The complexity of the algorithm is $O(n^2)$ which is also the complexity of computing $\mathbf F(p,Y)$; note that $m=O(n)$ since $Y$ is a deleted version of the input.

\begin{algorithm}[t!]
\caption{Symbolwise posterior probabilities with one trace}\label{alg:apprx_smap_dp}
\begin{algorithmic}[1]
\item Input: Trace {$Y$}, priors $p$\\ Outputs: Posteriors $\Pr(X_i=1|Y)\ \forall\ i$
\State Compute $\mathbf F(p_{[1:k]},Y_{[1:j]})\ \forall\ k,j$ and $\mathbf F(p_{[k:n]},Y_{[j:m]})\ \forall\ k,j$ via Alg.~\ref{alg:F_comp}
\For {$i=1:n$}
\State Use \eqref{eq:smap_postprob_thm} to compute $\Pr(X_i=1|Y)$
\EndFor
\end{algorithmic}
\end{algorithm}

\noindent\textbf{A trace reconstruction heuristic with $t$ traces.}
The posterior probability computation in Alg.~\ref{alg:apprx_smap_dp} naturally gives rise to a trace reconstruction heuristic that  updates the symbolwise statistics sequentially on the traces, where we use Alg.~\ref{alg:apprx_smap_dp} with one trace at a time to continually update $\Pr(X_i=1|Y)$. The overall heuristic  is described in Alg.~\ref{alg:apprx_smap}. The complexity of the algorithm is $O(tn^2)$ since Alg.~\ref{alg:apprx_smap} amounts to just $t$ uses of Alg.~\ref{alg:apprx_smap_dp}.

\begin{algorithm}[t!]
\caption{Trace reconstruction via iterative single-trace posterior probabilities}\label{alg:apprx_smap}
\begin{algorithmic}[1]
\item Input: Traces {$Y^{(1)},...,Y^{(t)}$}, input length $n$ \\ Outputs: Estimate of the input $\hat X$
\State Initialize priors $p^{old}=p^{new} \gets (0.5,0.5,...,0.5)$
\For {$l=1:t$}
\State Use Alg.~\ref{alg:apprx_smap_dp} with $p^{old}$ and $Y^{(l)}$ to update $p^{new}$
\State $p^{old}\gets p^{new}$
\EndFor
\For {$i=1:n$}
\If {$p^{new}_i\geq 0.5$}
 $\ \hat X_i \gets 1$
\Else
 $\ \hat X_i \gets 0$
\EndIf
\EndFor
\State \textbf{return} $\hat X_1 \hat X_2 ... \hat X_n$
\end{algorithmic}
\end{algorithm}



==> Sections/single_ML.tex <==


\section{On Maximum Likelihood Decoding For The Single-Trace Deletion Channel}
\label{sec:1deletion_ML}
%==================================================================

We here consider the single-trace  ML decoding in (\ref{eq:ML_deletion}),
assuming that the output sequence $Y$ is non-empty. 
To the best of our knowledge, the only known method to solve \eqref{eq:ML_deletion} involves solving a combinatorial optimization, essentially iterating over all possible choices of $x$ and computing the objective value for each of the choices. We here show that one could equivalently solve the continuous relaxation of \eqref{eq:ML_deletion} to obtain a solution of \eqref{eq:ML_deletion}. %Note that there could be multiple solutions to \eqref{eq:1deletion_ML}.
Before presenting the main result, we first state a useful lemma which factors a given coordinate $p_i$ out of the relaxed binomial coefficient $\mathbf F(p,Y)$ we introduced in Definition~\ref{def:f}. 
\begin{restatable}{lemma}{deletionMLrellemma}
For $p=(p_1,p_2,..,p_i,...,p_n)$ and $Y=Y_1Y_2...Y_m$ with $n \geq m > 0$, we have
\begin{align*}
  \mathbf F(p,Y) = \mathbf F( p_{
   [n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
\label{lemma:F_decomposition}
\end{restatable}
Recall that $\mathbf F(p,Y)$ sums over all $m$-length subsets $\mathcal S$ and associates $p_{\mathcal S}$ with $Y.$ Intuitively, this recursive relationship considers separately the cases where
\begin{itemize}
\item $i \notin \mathcal S$,
\item $i \in \mathcal S$ and is associated with a particular $Y_k$ where $Y_k = 1$,
\item $i \in \mathcal S$ and is associated with a particular $Y_k$ where $Y_k = 0$.
\end{itemize}
The detailed proof can be found in Appendix~\ref{app:F_lemma_proof}. It is clear from Lemma~\ref{lemma:F_decomposition} that $\mathbf F(p,Y)$ is affine when projected onto each coordinate $p_i$. Thus, the extrema of $\mathbf F(p,Y)$ must occur at the boundary of the support set of $p_i$; i.e., at either $p_i = 0$ or $p_i = 1$. Combining this with the fact that  $\mathbf F(\cdot)$ is a relaxed version of the binomial coefficient, we observe that the maximization problem in \eqref{eq:ML_deletion} is equivalent to its real-valued relaxation. The following result makes this precise.

\begin{theorem} The ML decoding problem for the single-trace deletion channel
\begin{equation}
\max_{x\in \{0,1\}^n} {x \choose Y} 
\label{eq:ml_opt_equiv1}
\end{equation}
is equivalent to the problem
\begin{equation}
\max_{p\in [0,1]^n} \mathbf F(p,Y).
\label{eq:ml_opt_equiv2}
\end{equation}
Furthermore, given any non-integral $p^* \in [0,1]^n$ that maximizes $\mathbf F(p,Y)$, we can construct a corresponding integral solution $x^* \in \{0,1\}^n$ that maximizes $\mathbf F(x,Y)$ and consequently also maximizes ${x \choose Y}$.
\label{thm:ML_relaxation}
\end{theorem}

\begin{proof}
As noted earlier, we have ${x \choose Y} = \mathbf F(x,Y)$. Therefore, we are interested in proving the following:
\begin{align*}
\max_{x\in \{0,1\}^n} \mathbf F(x,Y) \equiv \max_{p\in [0,1]^n} \mathbf F(p,Y),\numberthis
\label{eq:ml_opt_equiv_proof1}
\end{align*}
where $\equiv$ refers to that the two problems are equivalent (have the same optimal objective value).
We prove this by applying the following claim.\\
\textbf{Claim:} Given any feasible $p=(p_1,p_2,...,p_i,...,p_n)$, at least one of the following holds true:
\begin{itemize}
\item$\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y)$. Recall from notation that $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},0,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by $0$.
\item $\mathbf F(p^{(i\rightarrow 1)},Y) \geq \mathbf F(p,Y)$.
\end{itemize}
Thus if $p^*$ is an optimal solution to \eqref{eq:ml_opt_equiv2} with $p_i\in (0,1)$, then at least one of $p^{(i\rightarrow 0)}$ or $p^{(i\rightarrow 1)}$ is also an optimal solution. Sequentially applying this argument for each coordinate of $p$ shows that there exists a point in $\{0,1\}^n$ which is an optimal solution to \eqref{eq:ml_opt_equiv2} and consequently to \eqref{eq:ml_opt_equiv1}.

It remains to prove our claim. We use Lemma~\ref{lemma:F_decomposition} to factor out $p_i$ terms in $\mathbf F(p,Y)$:
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
Now we express $\mathbf F(p^{(i\rightarrow 0)},Y)$ and $\mathbf F(p^{(i\rightarrow 1)},Y)$ as
$$\mathbf F(p^{(i\rightarrow 0)},Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}),$$
$$\mathbf F(p^{(i\rightarrow 1)},Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$

\noindent Because $0\leq p_i\leq 1$ it directly follows that $$\min \left\{\mathbf F(p^{(i\rightarrow 0)},Y),\mathbf F(p^{(i\rightarrow 1)},Y)\right\} \leq \mathbf F(p,Y) \leq  \max \left\{\mathbf F(p^{(i\rightarrow 0)},Y),\mathbf F(p^{(i\rightarrow 1)},Y)\right\},$$
thus proving our claim.

Note that the proof gives a natural way to find an optimal lattice point $p_{lattice}^*$ given an optimal interior point $p^*$ by iterating through each coordinate of $p^*$ and switching them to $0$ or $1$ by comparing $\mathbf F(p^{(i\rightarrow 0)},Y)$ and $\mathbf F(p^{(i\rightarrow 1)},Y)$.
\end{proof}

The real-valued optimization problem in \eqref{eq:ml_opt_equiv2} falls under the umbrella of signomial optimization which is, in general, NP-hard (see for example, \cite{xu2014signomial}, \cite{chand2016signomial}). With a slight change of variables, \eqref{eq:ml_opt_equiv2} could also be expressed as a maximization of a convex function in a convex set. However, it is unclear if \eqref{eq:ml_opt_equiv2} is solvable in polynomial time or inherently hard to solve.

\begin{algorithm}[t!]
\caption{Coordinate switch ML heuristic}\label{alg:cood_switch}
\begin{algorithmic}[1]
\item Input: Blocklength $n$, Trace {$Y$}, Initial point $p = (p_1,p_2,...,p_n)$ \\ Outputs: Estimated sequence $\hat X$
\State Initialize visited set $\mathcal V = \emptyset$
\While {True} 
\State Compute $\mathcal F_i = |\mathbf F(p^{(i\rightarrow 1)},Y)- \mathbf F(p^{(i\rightarrow 0)},Y)|\ \forall\ i$ and let $\mathcal F = (\mathcal F_1,\mathcal F_2,...,\mathcal F_n)$.
\State Define the ordered list $\mathcal S =$ \texttt{argsort}$(\mathcal F)$ where \texttt{argsort}$(\mathcal F)$ returns the index set $[n]$ sorted by descending order of $\mathcal F$, i.e., $\mathcal F_{\mathcal S_1}\geq \mathcal F_{\mathcal S_2}\geq ... \geq \mathcal F_{\mathcal S_n}$.
\For {$i \in \mathcal S$ (ordered traversal)}
\If {$\mathbf F(p^{(i\rightarrow 1)},Y)- \mathbf F(p^{(i\rightarrow 0)},Y) \geq 0$}
\State update $p \leftarrow p^{(i\rightarrow 1)}$
\Else
\State update $p \leftarrow p^{(i\rightarrow 0)}$
\EndIf
\EndFor
\If {$p \in \mathcal{V}$} break
\EndIf
\State $\mathcal V = \mathcal V \cup \{p\}$
\EndWhile
\State \textbf{return} $\hat X = p$
\end{algorithmic}
\end{algorithm}

The proof of Theorem~\ref{thm:ML_relaxation} inspires a heuristic for sequence reconstruction (see Alg.~\ref{alg:cood_switch}):
\begin{itemize}
\item Start from a given point $p = (p_1,...,p_n) \in [0,1]^n$.
\item One round of iteration is defined as follows: fix a traversal order for the indices $\{1,2,...,n\}$. Traverse through the indices $i$ in order and make $p_i$ either 0 or 1 depending on whether $\mathbf F(p^{(i\rightarrow 0)},Y)$ or $\mathbf F(p^{(i\rightarrow 1)},Y)$ is larger. This ensures that $\mathbf F(p,Y)$ never decreases.
\item At the end of the round, check if the resultant $p$ was already obtained at the end of a previous round: if so, end the algorithm (to prevent it from going into an endless cycle). Otherwise, start a new round from the resultant $p$.
\end{itemize}
Clearly the resultant $p$ at the end of a round  is a lattice point since we make each $p_i$ to be 0 or 1. Therefore, the algorithm will end after a finite number of steps; in the worst case it will iterate through all $2^n$ sequences, although in practice we observe that it ends in 4-5 rounds (tested upto a blocklength of 100). We also note that the complexity of each round is $O(n^3)$ since it iterates through $n$ coordinates and for each coordinate computes $\mathbf F(\cdot)$, which is $O(n^2)$.

%starting from a random point $p = (p_1,...,p_n) \in [0,1]^n$ -- sequentially make each coordinate of $p$ either $0$ or $1$ by comparing whether $\mathbf F(p^{(i\rightarrow 0)},Y)$ or $\mathbf F(p^{(i\rightarrow 1)},Y)$ is larger, until convergence. Note that this procedure ensures that the value of the objective $\mathbf F(p,Y)$ never decreases. Convergence to a local maxima is also guaranteed since an interior point $p$ is transformed to a lattice point  after switching all the coordinates once, and subsequent rounds can just transform once lattice point to another. Thereon, the switching process attempts to find lattice points with larger objective value. Each round of this algorithms involves computing   The worst case time complexity of such an algorithm is $O(n^3 2^n)$ since it could potentially iterate over all lattice points until convergence, but in practice it is observed to converge within 4-5 steps (for $n = 100$).

A natural question  is whether it makes a difference if Alg.~\ref{alg:cood_switch} starts from an interior point ($p = (p_1,...,p_n) \in [0,1]^n$ where $\exists\ p_i \in (0,1)$) as compared to starting from a lattice point ($p = (p_1,...,p_n) \in \{0,1\}^n$). In Section~\ref{sec:Numerics} we show that starting from an interior point results in better estimation accuracy, thus supporting the usefulness of the ML relaxation.  
%\begin{figure}[!h]
%\centering
%\includegraphics[scale=0.5]{ml_heuristic_perf.pdf}
%\caption{Comparison of optimal ML objective value versus the objective value via Alg.~\ref{alg:cood_switch} when the initialization is an interior point and and when it is a lattice point when $n=14$ and $|Y|=7$. Although both initializations }
%\end{figure}




==> Sections/single_ML__Sundara_Rajan_s_conflicted_copy_2019-10-12_.tex <==


\section{Maximum likelihood for the single-trace deletion channel}
\label{sec:1deletion_ML}
Consider the ML formulation for the single-trace deletion channel given non-empty trace $Y$ and all possible $n$-length inputs allowed, restated here for convenience:
\begin{equation}
\argmax_{x\in \{0,1\}^n} {x \choose Y}.
\label{eq:1deletion_ML}
\end{equation}
To the best of our knowledge, the only known method to solve \eqref{eq:1deletion_ML} involves iterating over all possible choices of $x$ and computing the objective value for each of the choices. We here show that it is sufficient to solve a continuous relaxation of above problem to obtain a solution to \eqref{eq:1deletion_ML}. Note that there could be multiple solutions to \eqref{eq:1deletion_ML}. Before going in the main result, we first state a useful lemma which factors out a given coordinate $p_i$ out of $\mathbf F(p,Y)$. The proof of the lemma is relegated to the appendix.
\begin{restatable}{lemma}{deletionMLrellemma}
For $p=[p_1,p_2,..,p_i,...,p_n]$ and $Y=Y_1Y_2...Y_m$ with $n \geq m > 0$, we have
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
\label{lemma:F_decomposition}
\end{restatable}


\begin{theorem} An alternative optimization to characterize ML for the single-trace deletion channel.
\begin{equation}
\max_{x\in \{0,1\}^n} {x \choose Y} = \max_{p\in [0,1]^n} \mathbf F(p,Y).
\label{eq:ml_opt_equiv}
\end{equation}
Furthermore, given any non-integral $p^* \in [0,1]^n$ that maximizes $\mathbf F(p,Y)$, one could construct a corresponding integral solution $x^* \in \{0,1\}^n$ that maximizes $\mathbf F(p,Y)$ and consequently is also a solution to $\max_{x\in \{0,1\}^n} {x \choose Y}$.

\end{theorem}
\begin{proof}
As noted earlier, we have ${x \choose Y} = \mathbf F(x,Y)$. Therefore, we are interested in proving the following:
\begin{align*}
\max_{x\in \{0,1\}^n} \mathbf F(x,Y) \equiv \max_{p\in [0,1]^n} \mathbf F(p,Y).\numberthis
\label{eq:ml_opt_equiv_proof1}
\end{align*}
To show this and also the second statement, we prove that given $p=(p_1,p_2,...,p_i,...,p_n)$, at least one of the following holds true:
\begin{itemize}
\item$\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},0,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 0.
\item $\mathbf F(p^{(i\rightarrow 1)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},1,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 1.
\end{itemize}
Thus if $p^*$ is an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ with $p_i\in (0,1)$, then at least one of $p^{(i\rightarrow 0)}$ or $p^{(i\rightarrow 1)}$ is also an optimal solution. Sequentially applying this argument for each coordinate of $p$ shows that there exists a point in $\{0,1\}^n$ which is also an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ and consequently to $\max_{x\in \{0,1\}^n} \mathbf F(x,Y)$.

Now to prove our claim, we use Lemma~\ref{lemma:F_decomposition} to factor out $p_i$ terms in $\mathbf F(p,Y)$:
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
There are 3 cases
\begin{enumerate}
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) = \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) = \mathbf F(p,Y) = \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) > \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \leq \mathbf F(p,Y) \leq \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) < \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y) \geq \mathbf F(p^{(i\rightarrow 1)},Y).$
\end{enumerate}
Thus in each of the 3 cases, we see that at least one of $\mathbf F(p^{(i\rightarrow 0)},Y)$ or $\mathbf F(p^{(i\rightarrow 1)},Y)$ is at least as large as $\mathbf F(p,Y)$ thus proving the theorem. Note that the proof gives a natural way to find an optimal lattice point $p_{lattice}^*$ given a non-lattice point $p^*$ by iterating through each coordinate of $p^*$ and switching them to $0$ or $1$ by comparing $\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})$ with $\sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$
\end{proof}


==> Sections_revised/OLD/intro_Oct11.tex <==


\section{Introduction}
\label{sec:intro}



Sequence reconstruction over deletion channels, both with and without a codebook, has received considerable attention in the information theory as well as in the theoretical computer science literature. From an information theory perspective, reconstruction over the deletion channel, or more specifically a  maximum-likelihood (ML) argument for the deletion channel, would give further insight on the capacity of the deletion channel, a long-standing open problem (see \cite{mitzenmacher2009survey}). To quote \cite{mitzenmacher2009survey} -- ``at the very least, progress in this direction would likely surpass previous results on the capacity of the deletion channels''. Yet, there are no results on reconstruction over a deletion channel with statistical guarantees -- in this work, we take a step in this direction.

On the other hand, the problem of \textit{trace reconstruction}, as introduced in \cite{Batu2004}, has received renewed interest in the past few years (see \cite{Holenstein2008}, \cite{Peres2017}, \cite{De2017}, \cite{holden18}, \cite{Nazarov:2017}, \cite{holden2018lower}, \cite{chase2019new}). The problem of trace reconstruction can be stated simply as follows: consider a sequence $X$ which is simultaneously passed through $t$ independent deletion channels to yield $t$ deleted observations (also called \textit{traces}) of $X$ (see Fig.~\ref{fig:tdeletion}). How many such traces are needed to reconstruct $X$ perfectly? A variety of upper and lower bounds for this problem have been proposed, both for worst case and average case reconstruction. Our problem definition, stated in the following paragraph, is closely related to the average case trace reconstruction.
 
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.2]{tdeletion.pdf}
\caption{$t$-deletion channel model:  sequence $X$ passed through $t$ independent deletion channels to yield $t$ \textit{traces}. We aim to estimate $X$ from the $Y^{(i)}$s.}
\label{fig:tdeletion}
\end{center}
\end{figure}
 
\noindent \textbf{Problem definition.}  Given an input sequence of length $n$ (known apriori), the independently and identically distributed (i.i.d.) deletion channel deletes each input symbol indepedently with probability $\delta$, producing at its output a subsequence of the input sequence. Consider a sequence $X$ passed through $t$ ($t$ is fixed) such deletion
channels as shown in
Fig.~\ref{fig:tdeletion}. We call this the $t$-deletion channel model. We ask two questions:
\begin{enumerate}
\item For $t=1$ (see Fig.~\ref{fig:1deletion}, also called the single deletion channel model), and when $X_i \sim\ \text{ind. Ber}(p_i)$, compute the posterior distributions of $X_i$ given the trace $Y$.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.25]{1deletion.pdf}
\caption{The single deletion channel model. We assume $X_i \sim\ \text{ind. Ber}(p_i)$.}
\label{fig:1deletion}
\end{center}
\end{figure}
\item In the $t$ deletion channel model, for a fixed $t$ assume that $X_i \sim\ \text{i.i.d. Ber}(0.5)$ and compute the posterior distributions of $X_i$ given all traces $Y^{(1)}, Y^{(2)},...,Y^{(t)}$. 
\end{enumerate}
Note that solving 1) above doesn't lead to a natural solution for 2). This is because for a memoryless channel, we have $Y^{(j)} - X_i - Y^{(k)}$ and hence $\Pr(X_i=\alpha|Y^{(j)}, Y^{(k)}) \propto \Pr(X_i=\alpha|Y^{(j)}) \Pr(X_i=\alpha|Y^{(k)})$; so one could independently combine the posterior probabilities from each noisy observation. This is not the case for deletion channels since the markov chain $Y^{(j)} - X_i - Y^{(k)}$ no longer holds. More intuitively, one needs to first ``align'' the traces for computing the likelihoods. 
%, where every channel independently deletes each bit with probability $\delta$.


We point out that the problem considered in 2) asks a question complementary to the trace reconstruction: given a fixed (possibly a few) number of traces, what is our ``best'' guess of $X$? We provide algorithms which do this. Unlike trace reconstruction, we are not concerned with perfect reconstruction (since perfect reconstruction may not be possible with just a few traces), although it should also be obvious that performance guarantees for our algorithms (not a part of this work) would naturally lead to upper bounds for trace reconstruction.

Deletion channel by itself is known to be notoriously difficult to analyse. As stated earlier, the capacity of a single deletion channel is still unknown (\cite{diggavi2007capacity,diggavi2006information,diggavi2001transmission}); as are optimal coding schemes. Recent works have looked at the design of codes for deletion channels (\cite{ratzer2005marker,ratzer2000codes,thomas2017polar}); these works consider use of a codebook (we do not). As a result, statistical estimation over deletion channels is also a difficult problem due its highly combinatorial nature. To the best of our knowledge, as yet there are no efficient estimation algorithms over deletion channels with statistical guarantees; not even for ML over a single deletion channel.


\noindent \textbf{Biological motivation.} Trace reconstruction in itself was motivated, in part, by problems DNA sequence reconstruction. One such problem was to infer the DNA sequence of a common ancestor from the samples of its descendants. We argue that our problem definition fits more naturally in such a scenario since perfect reconstruction may not be feasible or even possible. Our motivation for considering this problem also comes from a recent DNA sequencing technology called \textit{nanopore sequencing}. The $t$-deletion channel model is a simplistic model to approximately capture the process of a DNA sequence passed through a nanopore sequencer\footnote{As seen in
  \cite{Mao2017},\cite{MDK17} there are more complicated effects of
  the nanopore reader not captured in this simple 
  representation.}.  
  
Very recently, a variant of the trace reconstruction problem called \textit{coded trace reconstruction} has been proposed, motivated by portable DNA-based data storage systems using DNA nanopores (see \cite{abroshan2019coding}, \cite{cheraghchi2019coded}, \cite{brakensiek2019coded}) and we believe that the ideas in this work may prove useful in such a setting.

There are other works on sequence assembly (see for example, \cite{Li09fastand}, \cite{Shomorony2016}),
where multiple short reads (from different segments of a sequence) are used to reconstruct the bigger
sequence. This work differs from sequence assembly since we are interested to infer the entire length sequence and not  just small segments of it (which are then ``stitched'' together in sequence assembly).

\noindent \textbf{Tools and techniques.} In terms of theoretical tools, the series of books by Lothaire (\cite{lothaire1997combinatorics,lothaire2002algebraic,lothaire2005applied}) extensively use algebraic tools  for problems in the combinatorics of sequences (or \textit{words}), and our work is inspired by such techniques. We borrow many of their notations and results for our work.


\noindent \textbf{Contributions.} {\color{red}} Our main contribution is to provide tools to visualize and analyze error events (described in the next section) for the multiple deletion channel model in Fig.~\ref{fig:tdeletion}. We also provide algorithms to solve the problems stated in 1) and 2) earlier in the section.
\begin{itemize}[wide=5pt]
\item In section~\ref{sec:1deletion}, for the single deletion channel model, we provide an  $O(n^2)$  algorithm to calculate the symbolwise posterior probabilities  $\Pr(X_i=1|Y)\ \forall\ i$ when $X_i \sim \text{ind. Ber}(p_i)$.
 \item  In Section~\ref{sec:exactsmap}, for the $t$-deletion channel model, we give an $O(2^t n^{t+2})$ algorithm to calculate the symbolwise posterior probabilities $\Pr(X_i = 1|Y_1,...,Y_t)$ when $X_i \sim \text{ind. Ber}(0.5)$.
\end{itemize}





==> Sections_revised/OLD/notation_Oct12.tex <==

\section{Notation and Tools}
\label{sec:notations}
\noindent \textbf{Basic notations:} In this work, we borrow a majority of the notation and tools from \cite{lothaire1997combinatorics} which deals with non-commutative algebra. We restate the definitions here for convenience. Calligraphic letters refer to sets, capitalized letters
correspond to random variables and bold letters are used for functions.  Let $\mathcal{A}$ be the set of all
symbols. Throughout this work, we will focus on the case where $\mathcal{A}=\{0,1\}$,
though  our methods extend to arbitrarily large sets of finite size. Define
$\mathcal{A}^n$ to be the set of all $n$-length sequences and $\mathcal{A}^*$ to be the set of all finite length sequences with
symbols in $\mathcal{A}$. For a sequence $f$, $|f|$ denotes the length
of $f$. For integers $i,j$, we define $[i:j] \triangleq \{i,i+1,...,j\}$ if $j\geq i$ and $[i:j] \triangleq \emptyset$ otherwise. Also define $[i] \triangleq [1:i]$.\\

\noindent \textbf{Binomial coefficient:} Given sequences $f$ and $g$ in $\mathcal{A}^*$, the number of
subsequence patterns of $f$ that are equal to $g$ is called the
\textit{binomial coefficient} of $g$ in $f$ and is denoted by $f
\choose g$.  For example, ${'apple' \choose 'ape'} = 2$ since $'ape'$ can be obtained from two (overlapping) subsequences of $'apple'$.


When the alphabet $\mathcal{A}$ is of cardinality 1, ${f
  \choose g} = {|f| \choose |g|}$, the classical binomial coefficient
with their respective lengths as the parameters. This definition hence
could be thought of as a generalization of the classical binomial
coefficients. We will denote by $e$ the sequence of length 0, and {define ${f
  \choose e} \triangleq 1\ \forall\ f\ \in\ \mathcal{A}^*$.} We also define the classical binomial coefficient ${a \choose b}\triangleq 0,$ whenever $b>a$ or $b<0$ for ease of use.

The binomial coefficient is an integral aspect of this work and for analyzing error events in deletion channels because the input-output relation for a deletion channel (with deletion probability $\delta$, input $X$ and output $Y$) can be expressed as 
\begin{equation}
\label{eq:in-out_relation}
\Pr(Y=y|X=x) = {x \choose y} \delta^{|x|-|y|} (1-\delta)^{|y|}.
\end{equation}
The proof is straight-forward -- the number of distinct error events that give rise to $y$ from $x$ is exactly the number of  subsequences of $x$ which are equal to $y$. Each of these error events has a probability $\delta^{|x|-|y|} (1-\delta)^{|y|}$, wherein the exponent of $\delta$ corresponds to the deleted symbols and the exponent of  $1-\delta$ to the undeleted symbols. 

Given the definition of the binomial coefficient, the maximum-likelihood (ML) estimate over a deletion channel with observed output $Y$ can be cast in the following form:
\begin{align*}
\argmax_{x \in \mathcal C}  {x \choose Y},\numberthis
\label{eq:ML_deletion}
\end{align*}
where $\mathcal C$ is the chosen codebook. In the case of multiple deletion channels with observed traces $Y^{(1)},...,Y^{(t)}$, the ML formulation is similar:
\begin{align*}
\argmax_{x \in \mathcal C}  \prod_{j=1}^{t} {x \choose Y^{(j)}}.\numberthis
\label{eq:ML_multiple_deletion}
\end{align*}
As yet, there is no known efficient way to come up with a solution for the above two formulations, even for \eqref{eq:ML_deletion} with $\mathcal C = \{0,1\}^n$ (see \cite{mitzenmacher2009survey}). In this work, we attempt to take a step in this direction by showing that a continuous relaxation of \eqref{eq:ML_deletion} is equivalent to \eqref{eq:ML_deletion}. However, an efficient algorithm to solve the optimization \eqref{eq:ML_deletion} remains open. In the context of trace reconstruction, the ultimate pursuit would be an algorithm for \eqref{eq:ML_multiple_deletion} with $\mathcal C = \{0,1\}^n$ and error analysis thereof.


\noindent We now describe a function which can be thought of as a real-valued extension of the binomial coefficient. This function is used in sections~\ref{sec:1deletion_ML} and \ref{sec:1deletion}. Consider the function $\mathbf F(\cdot)$ defined as:
\begin{definition}
\label{def:f}
\begin{align*}
&\mathbf F: \mathbb{R}^k \times \{0,1\}^l \rightarrow \mathbb{R},\\
\mathbf F(q,  v)\triangleq &\begin{cases} 
      \sum\limits_{\substack{\mathcal S|\mathcal S\subseteq [k],\\|\mathcal S|=l}} \quad \prod\limits_{i=1}^l q_{\mathcal S_i}^{v_i} (1-q_{\mathcal S_i})^{1-v_i} & 1 \leq l\leq k \\
	  1 &  0=l\leq k \\
      0 & \text{else}.  
   \end{cases}
\end{align*}
\noindent An alternate definition is as follows: consider a random vector $Z\in\{0,1\}^k$ such that $Z_i\sim$ ind. Ber$(q_i)$, let $q$ be the vector of probabilities of length $k$, $\mathcal S\subseteq [k]$ a subset of the indices of size $l$, and ${v}$ a binary vector of length $l$. Then, $$\mathbf F(q,v)=\sum_{\substack{\mathcal S||\mathcal S|=l}} \Pr(Z_{\mathcal S}= v).$$ Note that if $q$ is a vector of $0$'s and $1$'s, then $\mathbf F( q,  v)={q \choose v}$, the binomial coefficient of $v$ in $q$. Thus, $\mathbf F(\cdot)$ could be interpreted as an extension of the binomial coefficient where one of the parameters can take values in $[0,1]^n$ instead of $\{0,1\}^n$.
\end{definition}
Though at first sight, $\mathbf F(q,v)$ sums over an exponential number of subsets, a dynamic programming approach can be used to compute it in $O(|v|^2)$ time complexity. The dynamic program is described in section~\ref{sec:1deletion}.

\iffalse
%\subsection{Definitions and preliminary results}
\noindent \textbf{Edit distance:} The edit distance  $d_e(f,g)$  measures similarity between two sequences of
possibly different lengths \cite{Navarro2001}. $d_e(f,g)$ is the minimum number of operations
needed to transform $f$ to $g$, where the permitted operations are
insertion, deletion or substitution of a symbol. In this work, we
quantify the performance of algorithms in Section \ref{sec:Numerics}
using the edit distance metric.

\fi

The following definitions and ideas are relevant only for \ref{sec:exactsmap} and can be omitted  for the sections on single deletion channel. Before getting to the mathematical definitions, we first state a result of ours that aids in thinking about error events in multiple deletion channels. 

\subsection{An alternate interpretation of multiple deletion channel model}

The events occurring in the $t$-deletion channel model can be categorized into two groups:
\begin{enumerate}
\item an input symbol is deleted in \textit{all} the $t$-traces,
\item an input symbol is reflected in at least one of the traces.
\end{enumerate}
The error events of the first kind are in some sense ``not correctable" or even ``detectable" since it is impossible to tell what and where the deleted symbol could have been (although the probabilities need not be uniform). The events of the second kind, however, can still be detected although they could likely be confused with a large set of similar events. This thought process gives rise to a natural decomposition of the $t$-deletion channel model into a cascade of two channels: the first one being a deletion channel which captures error events of the first kind and the second one is what we call the \textit{remnant channel} which captures events of the second kind (see Fig.~\ref{fig:channel_equiv}). More precisely, the remnant channel is defined as follows:
\begin{definition}
\textit{Remnant channel:} an input symbol to the remnant channel is reflected in $k>0$ given outputs and deleted in the rest with a probability $\frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}$. 
\end{definition}
It is easy to note that probability of the union of all possible events here is $\sum_{k=1}^t {t \choose k} \frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}=1$, validating our definition.

\begin{restatable}{theorem}{channelequiv}
\label{thm:channel_equiv}
The $t$-deletion channel model and the cascade of the deletion channel with remnant channel shown in Fig.~\ref{fig:channel_equiv} are probabilistically equivalent, i.e., 
$$\Pr({Y}^{(1)},{Y}^{(2)},...,{Y}^{(t)}|X = x) = \Pr(\tilde{Y}^{(1)},\tilde{Y}^{(2)},...,\tilde{Y}^{(t)}|X = x).$$
\end{restatable}
The formal proof of the theorem requires few more definitions and is relegated to the appendix.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.4]{channel_equiv.pdf}
\caption{A channel equivalence result: the $t$-deletion channel model in (a) is probabilistically equivalent to the the cascade of a deletion channel with the \textit{remnant channel} ($ \mathcal C_2$) in (b).}
\label{fig:channel_equiv}
\end{center}
\end{figure}




\noindent\textbf{Edit graph} (as defined in \cite{Gusfield1997}): We now define a graph construct which is closely related to  the error events in the remnant channel. We start with a simple case and generalize subsequently. Define an \textit{edit graph} given two sequences $f$ and $g$, where every path connecting the ``origin'' to the ``destination'' on the edit graph yields a supersequence $h$ of $f,g$, where $h$ is ``covered'' by $f,g$ -- i.e.,  each symbol of $h$ comes from either $f$ or $g$ or
both. In other words, given that $f$ and $g$ are the outputs of the remnant channel (with two outputs), each path from the origin of the edit graph to the destination corresponds to a possible input $h$ to the remnant channel and to an error event  which resulted in $f$ and $g$ with  input $h$.


For $f$ and $g$ in $\mathcal
A^*$, we form a graph $\mathcal{G}(f,g)$ with $(|f|+1)(|g|+1)$
vertices each labelled with a distinct pair $(i,j), 0\leq i\leq
|f|,\ 0\leq j\leq |g|$. A directed edge
$(i_1,j_1)\rightarrow(i_2,j_2)$ exists iff at least one of the following
holds: 
%\vspace{-1mm}
\begin{enumerate}
\item$i_2-i_1=1$ and $j_1=j_2$, or
\item $j_2-j_1=1$ and $i_1=i_2$, or
\item  $i_2-i_1=1$, $j_2-j_1=1$ and $f_{i_2}=g_{j_2}$, 
\end{enumerate}
%\vspace{-1mm}
where $f_i$ is the $i^{th}$ symbol of the sequence $f$. The origin is the vertex $(0,0)$ and the destination $(|f|,|g|)$.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap1.pdf}
\caption{ Edit graph for sequences $f=$ `001' and $g=$ `101'. An easy way to think about this is to write down $f$ vertically with each symbol aligned to a vertical set of edges and $g$ horizontally likewise. A diagonal edge in a small square exists if the corresponding $f$ and $g$ symbols are equal. The thick red edges form a path from the origin to the destination; this path corresponds to the sequence `0101' -- append the corresponding symbol at the left of an edge if it's vertical or diagonal, otherwise append the symbol at the top. It is also easy to verify that 0101 is a supersequence of both $f$ and $g$, and could be obtained as a covering of $f$ and $g$; the path itself gives one such covering. This covering also corresponds to an error event in the remnant channel which would result in outputs $f$ and $g$ with input $h=$ `0101' -- more precisely, the error event is one in which the first symbol of $h$ is deleted only in $g$, the second symbol is deleted only in $f$ and the third and fourth symbols not deleted in either $f$ or $g$.}
\label{fig:editgraph_smap1}
\end{figure}

Let $p=((i_1,j_1),(i_2,j_2),...,(i_m,j_m))$ be a path in $\mathcal{G}(f,g)$. We define $ s(p)$ to be the sequence corresponding to the path. Intuitively, $s(p)$ is formed by appending symbols in the following
way: append the corresponding $f$ symbol for a vertical edge, $g$ symbol for horizontal edge, and $f$ or $g$ symbol for  diagonal edge (see example Fig.~\ref{fig:editgraph_smap1}). Any path from $(0,0)$ to $(|f|,|g|)$ corresponds to a supersequence of $f$ and $g$ and which is ``covered" by $f$ and $g$. More formally, define $ s(p)\triangleq x_1x_2...x_{m-1}$ where    
$$x_k = 
     \begin{cases}
       f_{i_{k+1}} \quad\text{if }j_{k}=j_{k+1},\\ 
       g_{j_{k+1}} \quad\text{if }i_{k}=i_{k+1},\\
       f_{i_{k+1}} \quad\text{else.}
    \end{cases}	
$$


The construct of edit graph can be extended to more than 2 sequences with the same idea. For sequences $f_1,f_2,...,f_t$, construct a $t$-dimensional grid with a number of vertices $(|f_1|+1)(|f_2|+1)...(|f_t|+1)$ labeled from $(0,0,...,0)$ to $(|f_1|,|f_2|,...,|f_t|)$. A vertex $u=(i_1,i_2,...,i_t)$ is connected to $v=(j_1,j_2,...,j_t)$ (we say $u \rightarrow v$) iff both of the following conditions are met:
\begin{itemize}
\item $j_l=i_l$ or $j_l=i_l+1$ $\forall\ l\in [t]$, i.e., $(i_1,...,i_t)$ and $(j_1,...,j_t)$ are vertices of a particular unit cube. Only these type of vertices can share an edge in the grid graph.
\item Let $\mathcal T \subseteq [t]$ be the collection of indices where $j_l=i_l+1$. Then $f_{i_l}$ is same $\forall\ l \in \mathcal T$. For instance, if $\mathcal T=\{1,3,5\}$, then $f_{i_1}=f_{i_3}=f_{i_5}$.
\end{itemize}
Define the vertex $(0,...,0)$ to be the origin of this graph and the vertex $(|f_1|,...,|f_t|)$ to be the destination. If $|f_j|=O(n)\ \forall\ j$, this graph has a number of vertices $O(n^t)$ and a maximum number of edges $O((2n)^t)$ since each vertex has at most $2^t$ outgoing edges.\\


\noindent\textbf{Infiltration product} (introduced in \cite{lothaire1997combinatorics}):
The infiltration product has been extensively used in \cite{lothaire1997combinatorics}, as a tool in non-commutative algebra. Here we give an edit-graph interpretation of this tool. We also give a formal definition later in this section. Using the edit graph we can construct the set of possible
supersequences $\mathcal{S}(f,g)$ of $f,g$ which are covered by
it. Clearly multiple paths could yield the same supersequence and we
can count the number of distinct ways  $\mathbf N(h;f,g)$ one can construct
the same supersequence $h$ from $f,g$.
We can  informally define the
\emph{infiltration product $f\uparrow g$} of $f$ and $g$, as a polynomial with monomials the supersequences $h$ in
$\mathcal{S}(f,g)$ and coefficients  $\langle f\uparrow g,h\rangle$ equal to $\mathbf N(h;f,g)$. In Fig.~\ref{fig:editgraph_smap1}, it is easy to verify that there is exactly one path corresponding to `101001' and hence $\langle 001\uparrow 101,101001 \rangle=1$ and similarly $\langle 001\uparrow 101,01001 \rangle=2$. One could find these coefficients for all relevant sequences and form the polynomial as described. More examples: Let $\mathcal{A}=\{a,b\}$, then
 %\vspace{-7pt}
\begin{itemize}[wide=2pt]
\item $ab\uparrow ab=ab+2aab+2abb+4aabb+2abab$,
\item $ab\uparrow ba=aba+bab+abab+2abba+2baab+baba.$
\end{itemize}
The  infiltration operation is commutative and associative, and infiltration of two sequences $f\uparrow g$ is a polynomial with variables of length (or \textit{degree}) at most $|f|+|g|$; see \cite{lothaire1997combinatorics}.
The definition of infiltration extends to two polynomials via distributivity (precisely defined in later), and consequently to multiple sequences as well. For multiple sequences, infiltration has the same edit graph interpretation: $\langle f_1\uparrow f_2 \uparrow...\uparrow f_t, w \rangle$ is the number of distinct ways of constructing $w$ as a supersequence of $f_1, f_2, ... ,f_t$ so that the construction covers $w$, i.e., construct the $t$-dimensional edit graph of $f_1, f_2, ... ,f_t$ and count the number of paths corresponding to $w$.

\subsection{Formal definition of infiltration product}
 We now give a more formal definition of the infiltration product (see \cite{lothaire1997combinatorics} for the equivalence of the two definitions and a more rigorous treatment). A \textit{formal series} with indeterminates (or variables) in a set $\mathcal A$ and coefficients in a commutative ring $\mathcal R$, is a mapping of $\mathcal A^*$ onto $\mathcal R$. Recall that a commutative ring is a set which forms an abelian group under an \textit{addition} operation, is a monoid under a \textit{multiplication} operation which commutes, and the multiplication operation distributes over addition. Here we consider $\mathbb Z$, the set of integers as the commutative ring  $\mathcal{R}$. A formal series is called a \textit{polynomial} if only a finite number of sequences are mapped to non-zero values, the rest of the sequences map to zero. Consider two polynomials $\sigma,\tau: \mathcal{A}^*\rightarrow \mathbb Z$. The value taken by a sequence $w\in \mathcal A^*$ on $\sigma$ (or the coefficient of $w$ in $\sigma$) is denoted by $\langle \sigma,w\rangle \in \mathbb R$. We also define binary addition ($\oplus$) and multiplication operations ($\times$) on the set of polynomials as follows:
\begin{align}
\langle \sigma\oplus \tau,w\rangle \triangleq \langle \sigma,w\rangle +  \langle \tau,w \rangle \quad \forall w\in \mathcal A^*,\label{eq:polynomial_add}\\
\langle \sigma\times \tau,w\rangle \triangleq \sum_{\substack{f,g\in \mathcal A^*:\\ f.g=w}}\langle \sigma,f\rangle  \langle \tau,g \rangle \quad \forall w\in \mathcal A^*.\label{eq:polynomial_prod}
\end{align}
We will use the usual symbols $+$ and $.$ in place of $\oplus$ and $\times$ in this work for convenience. The meaning of the operation would be clear depending on the operands. With these operations the set of polynomials form a non-commutative ring, and is denoted by $\mathbb Z\langle\mathcal A \rangle$, also called the free $\mathbb Z$-algebra on $\mathcal A$ in ring theory. Note that the addition and multiplication operations defined in \eqref{eq:polynomial_add} and \eqref{eq:polynomial_prod} are similar to the operations defined on commutative polynomials, except that the multiplication  operation under the summation in \eqref{eq:polynomial_prod} ($f.g=w$) is actually concatenation and is non-commutative.   The multiplication inside the summation in \eqref{eq:polynomial_prod} is multiplication in the real field and hence commutative. It is also easy to prove that the multiplication defined in \eqref{eq:polynomial_prod} distributes over addition defined in \eqref{eq:polynomial_add}. Thus, a polynomial in $\mathbb Z\langle\mathcal A \rangle$ can be represented as a sum of monomials in $\mathcal A^*$ each with an associated coefficient in $\mathbb Z$, i.e., $\sigma=\sum\limits_{w\in \mathcal A^*} \langle\sigma,w \rangle w$. Define the \textit{degree} of a polynomial to be equal to the length of a longest sequence with a non-zero coefficient in the polynomial and the \textit{number of terms} of a polynomial as the number of sequences with non-zero coefficients in the polynomial. Note that a degree $d$ polynomial could have a number of terms upto $2^{d+1}-1$.
 
With this, the \textit{infiltration product} (in general, for two polynomials) is defined as follows:

\begin{align}
\forall f\in \mathcal{A}^*,& \quad f\uparrow e = e\uparrow f=f.\nonumber \\
\forall f,g\in \mathcal{A}^*&,\quad  \forall a,b\in \mathcal{A}, \nonumber\\
fa\uparrow gb=(f\uparrow gb)a&+(fa\uparrow g)b+\mathbbm{1}_{a=b}(f\uparrow g)a.\nonumber \\
\forall \sigma,\tau \in \mathbb{Z}\langle\mathcal{A} \rangle, \quad &\sigma\uparrow \tau=\sum_{f,g\in \mathcal{A}^*} \langle \sigma,f \rangle \langle \tau,g \rangle (f\uparrow g). \label{def:infiltforseq}
\end{align}

%Note that infiltration is defined, in general, for two series, not just for two sequences.

\textbf{Summary of definitions and ideas introduced in this section:}
\begin{itemize}
\item The binomial coefficient captures the likelihood of observations for deletion channels. 
\item An extension of the binomial coefficient function where one of the parameters can take real values has been introduced; this function is pivotal for our results on the single-trace deletion channel.
\item For multiple deletion channels, the error events can be categorized into two groups -- one where an input symbol is deleted in all the traces, and second, the complement of this event. This categorization results in a natural decomposition of multiple deletion channel model into a cascade model involving the remnant channel.
\item The remnant channel disregards the error events where a symbol is deleted in all the traces.
\item The edit graph provides a way to visualize all the possible error events and input sequences to a remnant channel given its outputs. 
\item The infiltration product serves the same purpose as the edit graph, but has an algebraic flavor and provides rigor for proofs and analyses. The edit graph, on the other hand, is more helpful in designing reconstruction algorithms over deletion channels.
\end{itemize}



==> Sections_revised/OLD/single_ML_Oct12.tex <==


\section{Maximum likelihood for the single-trace deletion channel}
\label{sec:1deletion_ML}
Consider the ML formulation for the single-trace deletion channel given non-empty trace $Y$ and all possible $n$-length inputs allowed, restated here for convenience:
\begin{equation}
\argmax_{x\in \{0,1\}^n} {x \choose Y}.
\label{eq:1deletion_ML}
\end{equation}
To the best of our knowledge, the only known method to solve \eqref{eq:1deletion_ML} involves iterating over all possible choices of $x$ and computing the objective value for each of the choices. We here show that it is sufficient to solve a continuous relaxation of above problem to obtain a solution to \eqref{eq:1deletion_ML}. Note that there could be multiple solutions to \eqref{eq:1deletion_ML}. Before going in the main result, we first state a useful lemma which factors out a given coordinate $p_i$ out of $\mathbf F(p,Y)$. The proof of the lemma is relegated to the appendix.
\begin{restatable}{lemma}{deletionMLrellemma}
For $p=[p_1,p_2,..,p_i,...,p_n]$ and $Y=Y_1Y_2...Y_m$ with $n \geq m > 0$, we have
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
\label{lemma:F_decomposition}
\end{restatable}


\begin{theorem} An alternative optimization to characterize ML for the single-trace deletion channel.
\begin{equation}
\max_{x\in \{0,1\}^n} {x \choose Y} = \max_{p\in [0,1]^n} \mathbf F(p,Y).
\label{eq:ml_opt_equiv}
\end{equation}
Furthermore, given any non-integral $p^* \in [0,1]^n$ that maximizes $\mathbf F(p,Y)$, one could construct a corresponding integral solution $x^* \in \{0,1\}^n$ that maximizes $\mathbf F(p,Y)$ and consequently is also a solution to $\max_{x\in \{0,1\}^n} {x \choose Y}$.

\end{theorem}
\begin{proof}
As noted earlier, we have ${x \choose Y} = \mathbf F(x,Y)$. Therefore, we are interested in proving the following:
\begin{align*}
\max_{x\in \{0,1\}^n} \mathbf F(x,Y) \equiv \max_{p\in [0,1]^n} \mathbf F(p,Y).\numberthis
\label{eq:ml_opt_equiv_proof1}
\end{align*}
To show this and also the second statement, we prove that given $p=(p_1,p_2,...,p_i,...,p_n)$, at least one of the following holds true:
\begin{itemize}
\item$\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},0,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 0.
\item $\mathbf F(p^{(i\rightarrow 1)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},1,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 1.
\end{itemize}
Thus if $p^*$ is an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ with $p_i\in (0,1)$, then at least one of $p^{(i\rightarrow 0)}$ or $p^{(i\rightarrow 1)}$ is also an optimal solution. Sequentially applying this argument for each coordinate of $p$ shows that there exists a point in $\{0,1\}^n$ which is also an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ and consequently to $\max_{x\in \{0,1\}^n} \mathbf F(x,Y)$.

Now to prove our claim, we use Lemma~\ref{lemma:F_decomposition} to factor out $p_i$ terms in $\mathbf F(p,Y)$:
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
There are 3 cases
\begin{enumerate}
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) = \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) = \mathbf F(p,Y) = \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) > \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \leq \mathbf F(p,Y) \leq \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) < \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y) \geq \mathbf F(p^{(i\rightarrow 1)},Y).$
\end{enumerate}
Thus in each of the 3 cases, we see that at least one of $\mathbf F(p^{(i\rightarrow 0)},Y)$ or $\mathbf F(p^{(i\rightarrow 1)},Y)$ is at least as large as $\mathbf F(p,Y)$ thus proving the theorem. Note that the proof gives a natural way to find an optimal lattice point $p_{lattice}^*$ given a non-lattice point $p^*$ by iterating through each coordinate of $p^*$ and switching them to $0$ or $1$ by comparing $\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})$ with $\sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$
\end{proof}


==> Sections_revised/intro__Sundara_Rajan_s_conflicted_copy_2019-10-11_.tex <==


\section{Introduction}
\label{sec:intro}



Sequence reconstruction over deletion channels, both with and without a codebook, has received considerable attention in the information theory as well as in the theoretical computer science literature. From an information theory perspective, reconstruction over the deletion channel, or more specifically a  maximum-likelihood (ML) argument for the deletion channel, would give further insight on the capacity of the deletion channel, a long-standing open problem (see \cite{mitzenmacher2009survey}). To quote \cite{mitzenmacher2009survey} -- ``at the very least, progress in this direction would likely surpass previous results on the capacity of the deletion channels''. Yet, there are no results on reconstruction over a deletion channel with statistical guarantees -- in this work, we take a step in this direction.

On the other hand, the problem of \textit{trace reconstruction}, as introduced in \cite{Batu2004}, has received renewed interest in the past few years (see \cite{Holenstein2008}, \cite{Peres2017}, \cite{De2017}, \cite{holden18}, \cite{Nazarov:2017}, \cite{holden2018lower}, \cite{chase2019new}). The problem of trace reconstruction can be stated simply as follows: consider a sequence $X$ which is simultaneously passed through $t$ independent deletion channels to yield $t$ deleted observations (also called \textit{traces}) of $X$ (see Fig.~\ref{fig:tdeletion}). How many such traces are needed to reconstruct $X$ perfectly? A variety of upper and lower bounds for this problem have been proposed, both for worst case and average case reconstruction. Our problem definition, stated in the following paragraph, is closely related to the average case trace reconstruction.
 
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.2]{tdeletion.pdf}
\caption{$t$-deletion channel model:  sequence $X$ passed through $t$ independent deletion channels to yield $t$ \textit{traces}. We aim to estimate $X$ from the $Y^{(i)}$s.}
\label{fig:tdeletion}
\end{center}
\end{figure}
 
\noindent \textbf{Problem definition.}  Given an input sequence of length $n$ (known apriori), the independently and identically distributed (i.i.d.) deletion channel deletes each input symbol indepedently with probability $\delta$, producing at its output a subsequence of the input sequence. Consider a sequence $X$ passed through $t$ ($t$ is fixed) such deletion
channels as shown in
Fig.~\ref{fig:tdeletion}. We call this the $t$-deletion channel model. We ask two questions:
\begin{enumerate}
\item For $t=1$ (see Fig.~\ref{fig:1deletion}, also called the single deletion channel model), and when $X_i \sim\ \text{ind. Ber}(p_i)$, compute the posterior distributions of $X_i$ given the trace $Y$.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.25]{1deletion.pdf}
\caption{The single deletion channel model. We assume $X_i \sim\ \text{ind. Ber}(p_i)$.}
\label{fig:1deletion}
\end{center}
\end{figure}
\item In the $t$ deletion channel model, for a fixed $t$ assume that $X_i \sim\ \text{i.i.d. Ber}(0.5)$ and compute the posterior distributions of $X_i$ given all traces $Y^{(1)}, Y^{(2)},...,Y^{(t)}$. 
\end{enumerate}
Note that solving 1) above doesn't lead to a natural solution for 2). This is because for a memoryless channel, we have $Y^{(j)} - X_i - Y^{(k)}$ and hence $\Pr(X_i=\alpha|Y^{(j)}, Y^{(k)}) \propto \Pr(X_i=\alpha|Y^{(j)}) \Pr(X_i=\alpha|Y^{(k)})$; so one could independently combine the posterior probabilities from each noisy observation. This is not the case for deletion channels since the markov chain $Y^{(j)} - X_i - Y^{(k)}$ no longer holds. More intuitively, one needs to first ``align'' the traces for computing the likelihoods. 
%, where every channel independently deletes each bit with probability $\delta$.


We point out that the problem considered in 2) asks a question complementary to the trace reconstruction: given a fixed (possibly a few) number of traces, what is our ``best'' guess of $X$? We provide algorithms which do this. Unlike trace reconstruction, we are not concerned with perfect reconstruction (since perfect reconstruction may not be possible with just a few traces), although it should also be obvious that performance guarantees for our algorithms (not a part of this work) would naturally lead to upper bounds for trace reconstruction.

Deletion channel by itself is known to be notoriously difficult to analyse. As stated earlier, the capacity of a single deletion channel is still unknown (\cite{diggavi2007capacity,diggavi2006information,diggavi2001transmission}); as are optimal coding schemes. Recent works have looked at the design of codes for deletion channels (\cite{ratzer2005marker,ratzer2000codes,thomas2017polar}); these works consider use of a codebook (we do not). As a result, statistical estimation over deletion channels is also a difficult problem due its highly combinatorial nature. To the best of our knowledge, as yet there are no efficient estimation algorithms over deletion channels with statistical guarantees; not even for ML over a single deletion channel.


\noindent \textbf{Biological motivation.} Trace reconstruction in itself was motivated, in part, by problems DNA sequence reconstruction. One such problem was to infer the DNA sequence of a common ancestor from the samples of its descendants. We argue that our problem definition fits more naturally in such a scenario since perfect reconstruction may not be feasible or even possible. Our motivation for considering this problem also comes from a recent DNA sequencing technology called \textit{nanopore sequencing}. The $t$-deletion channel model is a simplistic model to approximately capture the process of a DNA sequence passed through a nanopore sequencer\footnote{As seen in
  \cite{Mao2017},\cite{MDK17} there are more complicated effects of
  the nanopore reader not captured in this simple 
  representation.}.  
  
Very recently, a variant of the trace reconstruction problem called \textit{coded trace reconstruction} has been proposed, motivated by portable DNA-based data storage systems using DNA nanopores (see \cite{abroshan2019coding}, \cite{cheraghchi2019coded}, \cite{brakensiek2019coded}) and we believe that the ideas in this work may prove useful in such a setting.

There are other works on sequence assembly (see for example, \cite{Li09fastand}, \cite{Shomorony2016}),
where multiple short reads (from different segments of a sequence) are used to reconstruct the bigger
sequence. This work differs from sequence assembly since we are interested to infer the entire length sequence and not  just small segments of it (which are then ``stitched'' together in sequence assembly).

\noindent \textbf{Tools and techniques.} In terms of theoretical tools, the series of books by Lothaire (\cite{lothaire1997combinatorics,lothaire2002algebraic,lothaire2005applied}) extensively use algebraic tools  for problems in the combinatorics of sequences (or \textit{words}), and our work is inspired by such techniques. We borrow many of their notations and results for our work.


\noindent \textbf{Contributions.} {\color{red}} Our main contribution is to provide tools to visualize and analyze error events (described in the next section) for the multiple deletion channel model in Fig.~\ref{fig:tdeletion}. We also provide algorithms to solve the problems stated in 1) and 2) earlier in the section.
\begin{itemize}[wide=5pt]
\item In section~\ref{sec:1deletion}, for the single deletion channel model, we provide an  $O(n^2)$  algorithm to calculate the symbolwise posterior probabilities  $\Pr(X_i=1|Y)\ \forall\ i$ when $X_i \sim \text{ind. Ber}(p_i)$.
 \item  In Section~\ref{sec:exactsmap}, for the $t$-deletion channel model, we give an $O(2^t n^{t+2})$ algorithm to calculate the symbolwise posterior probabilities $\Pr(X_i = 1|Y_1,...,Y_t)$ when $X_i \sim \text{ind. Ber}(0.5)$.
\end{itemize}





==> Sections_revised/notation__Sundara_Rajan_s_conflicted_copy_2019-10-12_.tex <==

\section{Notation and Tools}
\label{sec:notations}
\noindent \textbf{Basic notations:} In this work, we borrow a majority of the notation and tools from \cite{lothaire1997combinatorics} which deals with non-commutative algebra. We restate the definitions here for convenience. Calligraphic letters refer to sets, capitalized letters
correspond to random variables and bold letters are used for functions.  Let $\mathcal{A}$ be the set of all
symbols. Throughout this work, we will focus on the case where $\mathcal{A}=\{0,1\}$,
though  our methods extend to arbitrarily large sets of finite size. Define
$\mathcal{A}^n$ to be the set of all $n$-length sequences and $\mathcal{A}^*$ to be the set of all finite length sequences with
symbols in $\mathcal{A}$. For a sequence $f$, $|f|$ denotes the length
of $f$. For integers $i,j$, we define $[i:j] \triangleq \{i,i+1,...,j\}$ if $j\geq i$ and $[i:j] \triangleq \emptyset$ otherwise. Also define $[i] \triangleq [1:i]$.\\

\noindent \textbf{Binomial coefficient:} Given sequences $f$ and $g$ in $\mathcal{A}^*$, the number of
subsequence patterns of $f$ that are equal to $g$ is called the
\textit{binomial coefficient} of $g$ in $f$ and is denoted by $f
\choose g$.  For example, ${'apple' \choose 'ape'} = 2$ since $'ape'$ can be obtained from two (overlapping) subsequences of $'apple'$.


When the alphabet $\mathcal{A}$ is of cardinality 1, ${f
  \choose g} = {|f| \choose |g|}$, the classical binomial coefficient
with their respective lengths as the parameters. This definition hence
could be thought of as a generalization of the classical binomial
coefficients. We will denote by $e$ the sequence of length 0, and {define ${f
  \choose e} \triangleq 1\ \forall\ f\ \in\ \mathcal{A}^*$.} We also define the classical binomial coefficient ${a \choose b}\triangleq 0,$ whenever $b>a$ or $b<0$ for ease of use.

The binomial coefficient is an integral aspect of this work and for analyzing error events in deletion channels because the input-output relation for a deletion channel (with deletion probability $\delta$, input $X$ and output $Y$) can be expressed as 
\begin{equation}
\label{eq:in-out_relation}
\Pr(Y=y|X=x) = {x \choose y} \delta^{|x|-|y|} (1-\delta)^{|y|}.
\end{equation}
The proof is straight-forward -- the number of distinct error events that give rise to $y$ from $x$ is exactly the number of  subsequences of $x$ which are equal to $y$. Each of these error events has a probability $\delta^{|x|-|y|} (1-\delta)^{|y|}$, wherein the exponent of $\delta$ corresponds to the deleted symbols and the exponent of  $1-\delta$ to the undeleted symbols. 

Given the definition of the binomial coefficient, the maximum-likelihood (ML) estimate over a deletion channel with observed output $Y$ can be cast in the following form:
\begin{align*}
\argmax_{x \in \mathcal C}  {x \choose Y},\numberthis
\label{eq:ML_deletion}
\end{align*}
where $\mathcal C$ is the chosen codebook. In the case of multiple deletion channels with observed traces $Y^{(1)},...,Y^{(t)}$, the ML formulation is similar:
\begin{align*}
\argmax_{x \in \mathcal C}  \prod_{j=1}^{t} {x \choose Y^{(j)}}.\numberthis
\label{eq:ML_multiple_deletion}
\end{align*}
As yet, there is no known efficient way to come up with a solution for the above two formulations, even for \eqref{eq:ML_deletion} with $\mathcal C = \{0,1\}^n$ (see \cite{mitzenmacher2009survey}). In this work, we attempt to take a step in this direction by showing that a continuous relaxation of \eqref{eq:ML_deletion} is equivalent to \eqref{eq:ML_deletion}. However, an efficient algorithm to solve the optimization \eqref{eq:ML_deletion} remains open. In the context of trace reconstruction, the ultimate pursuit would be an algorithm for \eqref{eq:ML_multiple_deletion} with $\mathcal C = \{0,1\}^n$ and error analysis thereof.


\noindent We now describe a function which can be thought of as a real-valued extension of the binomial coefficient. This function is used in sections~\ref{sec:1deletion_ML} and \ref{sec:1deletion}. Consider the function $\mathbf F(\cdot)$ defined as:
\begin{definition}
\label{def:f}
\begin{align*}
&\mathbf F: \mathbb{R}^k \times \{0,1\}^l \rightarrow \mathbb{R},\\
\mathbf F(q,  v)\triangleq &\begin{cases} 
      \sum\limits_{\substack{\mathcal S|\mathcal S\subseteq [k],\\|\mathcal S|=l}} \quad \prod\limits_{i=1}^l q_{\mathcal S_i}^{v_i} (1-q_{\mathcal S_i})^{1-v_i} & 1 \leq l\leq k \\
	  1 &  0=l\leq k \\
      0 & \text{else}.  
   \end{cases}
\end{align*}
\noindent An alternate definition is as follows: consider a random vector $Z\in\{0,1\}^k$ such that $Z_i\sim$ ind. Ber$(q_i)$, let $q$ be the vector of probabilities of length $k$, $\mathcal S\subseteq [k]$ a subset of the indices of size $l$, and ${v}$ a binary vector of length $l$. Then, $$\mathbf F(q,v)=\sum_{\substack{\mathcal S||\mathcal S|=l}} \Pr(Z_{\mathcal S}= v).$$ Note that if $q$ is a vector of $0$'s and $1$'s, then $\mathbf F( q,  v)={q \choose v}$, the binomial coefficient of $v$ in $q$. Thus, $\mathbf F(\cdot)$ could be interpreted as an extension of the binomial coefficient where one of the parameters can take values in $[0,1]^n$ instead of $\{0,1\}^n$.
\end{definition}
Though at first sight, $\mathbf F(q,v)$ sums over an exponential number of subsets, a dynamic programming approach can be used to compute it in $O(|v|^2)$ time complexity. The dynamic program is described in section~\ref{sec:1deletion}.

\iffalse
%\subsection{Definitions and preliminary results}
\noindent \textbf{Edit distance:} The edit distance  $d_e(f,g)$  measures similarity between two sequences of
possibly different lengths \cite{Navarro2001}. $d_e(f,g)$ is the minimum number of operations
needed to transform $f$ to $g$, where the permitted operations are
insertion, deletion or substitution of a symbol. In this work, we
quantify the performance of algorithms in Section \ref{sec:Numerics}
using the edit distance metric.

\fi

The following definitions and ideas are relevant only for \ref{sec:exactsmap} and can be omitted  for the sections on single deletion channel. Before getting to the mathematical definitions, we first state a result of ours that aids in thinking about error events in multiple deletion channels. 

\subsection{An alternate interpretation of multiple deletion channel model}

The events occurring in the $t$-deletion channel model can be categorized into two groups:
\begin{enumerate}
\item an input symbol is deleted in \textit{all} the $t$-traces,
\item an input symbol is reflected in at least one of the traces.
\end{enumerate}
The error events of the first kind are in some sense ``not correctable" or even ``detectable" since it is impossible to tell what and where the deleted symbol could have been (although the probabilities need not be uniform). The events of the second kind, however, can still be detected although they could likely be confused with a large set of similar events. This thought process gives rise to a natural decomposition of the $t$-deletion channel model into a cascade of two channels: the first one being a deletion channel which captures error events of the first kind and the second one is what we call the \textit{remnant channel} which captures events of the second kind (see Fig.~\ref{fig:channel_equiv}). More precisely, the remnant channel is defined as follows:
\begin{definition}
\textit{Remnant channel:} an input symbol to the remnant channel is reflected in $k>0$ given outputs and deleted in the rest with a probability $\frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}$. 
\end{definition}
It is easy to note that probability of the union of all possible events here is $\sum_{k=1}^t {t \choose k} \frac{\delta^{t-k}(1-\delta)^k}{1-\delta^t}=1$, validating our definition.

\begin{restatable}{theorem}{channelequiv}
\label{thm:channel_equiv}
The $t$-deletion channel model and the cascade of the deletion channel with remnant channel shown in Fig.~\ref{fig:channel_equiv} are probabilistically equivalent, i.e., 
$$\Pr({Y}^{(1)},{Y}^{(2)},...,{Y}^{(t)}|X = x) = \Pr(\tilde{Y}^{(1)},\tilde{Y}^{(2)},...,\tilde{Y}^{(t)}|X = x).$$
\end{restatable}
The formal proof of the theorem requires few more definitions and is relegated to the appendix.
\begin{figure}[!h]
\begin{center}
\includegraphics[scale=0.4]{channel_equiv.pdf}
\caption{A channel equivalence result: the $t$-deletion channel model in (a) is probabilistically equivalent to the the cascade of a deletion channel with the \textit{remnant channel} ($ \mathcal C_2$) in (b).}
\label{fig:channel_equiv}
\end{center}
\end{figure}




\noindent\textbf{Edit graph} (as defined in \cite{Gusfield1997}): We now define a graph construct which is closely related to  the error events in the remnant channel. We start with a simple case and generalize subsequently. Define an \textit{edit graph} given two sequences $f$ and $g$, where every path connecting the ``origin'' to the ``destination'' on the edit graph yields a supersequence $h$ of $f,g$, where $h$ is ``covered'' by $f,g$ -- i.e.,  each symbol of $h$ comes from either $f$ or $g$ or
both. In other words, given that $f$ and $g$ are the outputs of the remnant channel (with two outputs), each path from the origin of the edit graph to the destination corresponds to a possible input $h$ to the remnant channel and to an error event  which resulted in $f$ and $g$ with  input $h$.


For $f$ and $g$ in $\mathcal
A^*$, we form a graph $\mathcal{G}(f,g)$ with $(|f|+1)(|g|+1)$
vertices each labelled with a distinct pair $(i,j), 0\leq i\leq
|f|,\ 0\leq j\leq |g|$. A directed edge
$(i_1,j_1)\rightarrow(i_2,j_2)$ exists iff at least one of the following
holds: 
%\vspace{-1mm}
\begin{enumerate}
\item$i_2-i_1=1$ and $j_1=j_2$, or
\item $j_2-j_1=1$ and $i_1=i_2$, or
\item  $i_2-i_1=1$, $j_2-j_1=1$ and $f_{i_2}=g_{j_2}$, 
\end{enumerate}
%\vspace{-1mm}
where $f_i$ is the $i^{th}$ symbol of the sequence $f$. The origin is the vertex $(0,0)$ and the destination $(|f|,|g|)$.

\begin{figure}[!h]
\centering
\includegraphics[scale=0.25]{editgraph_smap1.pdf}
\caption{ Edit graph for sequences $f=$ `001' and $g=$ `101'. An easy way to think about this is to write down $f$ vertically with each symbol aligned to a vertical set of edges and $g$ horizontally likewise. A diagonal edge in a small square exists if the corresponding $f$ and $g$ symbols are equal. The thick red edges form a path from the origin to the destination; this path corresponds to the sequence `0101' -- append the corresponding symbol at the left of an edge if it's vertical or diagonal, otherwise append the symbol at the top. It is also easy to verify that 0101 is a supersequence of both $f$ and $g$, and could be obtained as a covering of $f$ and $g$; the path itself gives one such covering. This covering also corresponds to an error event in the remnant channel which would result in outputs $f$ and $g$ with input $h=$ `0101' -- more precisely, the error event is one in which the first symbol of $h$ is deleted only in $g$, the second symbol is deleted only in $f$ and the third and fourth symbols not deleted in either $f$ or $g$.}
\label{fig:editgraph_smap1}
\end{figure}

Let $p=((i_1,j_1),(i_2,j_2),...,(i_m,j_m))$ be a path in $\mathcal{G}(f,g)$. We define $ s(p)$ to be the sequence corresponding to the path. Intuitively, $s(p)$ is formed by appending symbols in the following
way: append the corresponding $f$ symbol for a vertical edge, $g$ symbol for horizontal edge, and $f$ or $g$ symbol for  diagonal edge (see example Fig.~\ref{fig:editgraph_smap1}). Any path from $(0,0)$ to $(|f|,|g|)$ corresponds to a supersequence of $f$ and $g$ and which is ``covered" by $f$ and $g$. More formally, define $ s(p)\triangleq x_1x_2...x_{m-1}$ where    
$$x_k = 
     \begin{cases}
       f_{i_{k+1}} \quad\text{if }j_{k}=j_{k+1},\\ 
       g_{j_{k+1}} \quad\text{if }i_{k}=i_{k+1},\\
       f_{i_{k+1}} \quad\text{else.}
    \end{cases}	
$$


The construct of edit graph can be extended to more than 2 sequences with the same idea. For sequences $f_1,f_2,...,f_t$, construct a $t$-dimensional grid with a number of vertices $(|f_1|+1)(|f_2|+1)...(|f_t|+1)$ labeled from $(0,0,...,0)$ to $(|f_1|,|f_2|,...,|f_t|)$. A vertex $u=(i_1,i_2,...,i_t)$ is connected to $v=(j_1,j_2,...,j_t)$ (we say $u \rightarrow v$) iff both of the following conditions are met:
\begin{itemize}
\item $j_l=i_l$ or $j_l=i_l+1$ $\forall\ l\in [t]$, i.e., $(i_1,...,i_t)$ and $(j_1,...,j_t)$ are vertices of a particular unit cube. Only these type of vertices can share an edge in the grid graph.
\item Let $\mathcal T \subseteq [t]$ be the collection of indices where $j_l=i_l+1$. Then $f_{i_l}$ is same $\forall\ l \in \mathcal T$. For instance, if $\mathcal T=\{1,3,5\}$, then $f_{i_1}=f_{i_3}=f_{i_5}$.
\end{itemize}
Define the vertex $(0,...,0)$ to be the origin of this graph and the vertex $(|f_1|,...,|f_t|)$ to be the destination. If $|f_j|=O(n)\ \forall\ j$, this graph has a number of vertices $O(n^t)$ and a maximum number of edges $O((2n)^t)$ since each vertex has at most $2^t$ outgoing edges.\\


\noindent\textbf{Infiltration product} (introduced in \cite{lothaire1997combinatorics}):
The infiltration product has been extensively used in \cite{lothaire1997combinatorics}, as a tool in non-commutative algebra. Here we give an edit-graph interpretation of this tool. We also give a formal definition later in this section. Using the edit graph we can construct the set of possible
supersequences $\mathcal{S}(f,g)$ of $f,g$ which are covered by
it. Clearly multiple paths could yield the same supersequence and we
can count the number of distinct ways  $\mathbf N(h;f,g)$ one can construct
the same supersequence $h$ from $f,g$.
We can  informally define the
\emph{infiltration product $f\uparrow g$} of $f$ and $g$, as a polynomial with monomials the supersequences $h$ in
$\mathcal{S}(f,g)$ and coefficients  $\langle f\uparrow g,h\rangle$ equal to $\mathbf N(h;f,g)$. In Fig.~\ref{fig:editgraph_smap1}, it is easy to verify that there is exactly one path corresponding to `101001' and hence $\langle 001\uparrow 101,101001 \rangle=1$ and similarly $\langle 001\uparrow 101,01001 \rangle=2$. One could find these coefficients for all relevant sequences and form the polynomial as described. More examples: Let $\mathcal{A}=\{a,b\}$, then
 %\vspace{-7pt}
\begin{itemize}[wide=2pt]
\item $ab\uparrow ab=ab+2aab+2abb+4aabb+2abab$,
\item $ab\uparrow ba=aba+bab+abab+2abba+2baab+baba.$
\end{itemize}
The  infiltration operation is commutative and associative, and infiltration of two sequences $f\uparrow g$ is a polynomial with variables of length (or \textit{degree}) at most $|f|+|g|$; see \cite{lothaire1997combinatorics}.
The definition of infiltration extends to two polynomials via distributivity (precisely defined in later), and consequently to multiple sequences as well. For multiple sequences, infiltration has the same edit graph interpretation: $\langle f_1\uparrow f_2 \uparrow...\uparrow f_t, w \rangle$ is the number of distinct ways of constructing $w$ as a supersequence of $f_1, f_2, ... ,f_t$ so that the construction covers $w$, i.e., construct the $t$-dimensional edit graph of $f_1, f_2, ... ,f_t$ and count the number of paths corresponding to $w$.

\subsection{Formal definition of infiltration product}
 We now give a more formal definition of the infiltration product (see \cite{lothaire1997combinatorics} for the equivalence of the two definitions and a more rigorous treatment). A \textit{formal series} with indeterminates (or variables) in a set $\mathcal A$ and coefficients in a commutative ring $\mathcal R$, is a mapping of $\mathcal A^*$ onto $\mathcal R$. Recall that a commutative ring is a set which forms an abelian group under an \textit{addition} operation, is a monoid under a \textit{multiplication} operation which commutes, and the multiplication operation distributes over addition. Here we consider $\mathbb Z$, the set of integers as the commutative ring  $\mathcal{R}$. A formal series is called a \textit{polynomial} if only a finite number of sequences are mapped to non-zero values, the rest of the sequences map to zero. Consider two polynomials $\sigma,\tau: \mathcal{A}^*\rightarrow \mathbb Z$. The value taken by a sequence $w\in \mathcal A^*$ on $\sigma$ (or the coefficient of $w$ in $\sigma$) is denoted by $\langle \sigma,w\rangle \in \mathbb R$. We also define binary addition ($\oplus$) and multiplication operations ($\times$) on the set of polynomials as follows:
\begin{align}
\langle \sigma\oplus \tau,w\rangle \triangleq \langle \sigma,w\rangle +  \langle \tau,w \rangle \quad \forall w\in \mathcal A^*,\label{eq:polynomial_add}\\
\langle \sigma\times \tau,w\rangle \triangleq \sum_{\substack{f,g\in \mathcal A^*:\\ f.g=w}}\langle \sigma,f\rangle  \langle \tau,g \rangle \quad \forall w\in \mathcal A^*.\label{eq:polynomial_prod}
\end{align}
We will use the usual symbols $+$ and $.$ in place of $\oplus$ and $\times$ in this work for convenience. The meaning of the operation would be clear depending on the operands. With these operations the set of polynomials form a non-commutative ring, and is denoted by $\mathbb Z\langle\mathcal A \rangle$, also called the free $\mathbb Z$-algebra on $\mathcal A$ in ring theory. Note that the addition and multiplication operations defined in \eqref{eq:polynomial_add} and \eqref{eq:polynomial_prod} are similar to the operations defined on commutative polynomials, except that the multiplication  operation under the summation in \eqref{eq:polynomial_prod} ($f.g=w$) is actually concatenation and is non-commutative.   The multiplication inside the summation in \eqref{eq:polynomial_prod} is multiplication in the real field and hence commutative. It is also easy to prove that the multiplication defined in \eqref{eq:polynomial_prod} distributes over addition defined in \eqref{eq:polynomial_add}. Thus, a polynomial in $\mathbb Z\langle\mathcal A \rangle$ can be represented as a sum of monomials in $\mathcal A^*$ each with an associated coefficient in $\mathbb Z$, i.e., $\sigma=\sum\limits_{w\in \mathcal A^*} \langle\sigma,w \rangle w$. Define the \textit{degree} of a polynomial to be equal to the length of a longest sequence with a non-zero coefficient in the polynomial and the \textit{number of terms} of a polynomial as the number of sequences with non-zero coefficients in the polynomial. Note that a degree $d$ polynomial could have a number of terms upto $2^{d+1}-1$.
 
With this, the \textit{infiltration product} (in general, for two polynomials) is defined as follows:

\begin{align}
\forall f\in \mathcal{A}^*,& \quad f\uparrow e = e\uparrow f=f.\nonumber \\
\forall f,g\in \mathcal{A}^*&,\quad  \forall a,b\in \mathcal{A}, \nonumber\\
fa\uparrow gb=(f\uparrow gb)a&+(fa\uparrow g)b+\mathbbm{1}_{a=b}(f\uparrow g)a.\nonumber \\
\forall \sigma,\tau \in \mathbb{Z}\langle\mathcal{A} \rangle, \quad &\sigma\uparrow \tau=\sum_{f,g\in \mathcal{A}^*} \langle \sigma,f \rangle \langle \tau,g \rangle (f\uparrow g). \label{def:infiltforseq}
\end{align}

%Note that infiltration is defined, in general, for two series, not just for two sequences.

\textbf{Summary of definitions and ideas introduced in this section:}
\begin{itemize}
\item The binomial coefficient captures the likelihood of observations for deletion channels. 
\item An extension of the binomial coefficient function where one of the parameters can take real values has been introduced; this function is pivotal for our results on the single-trace deletion channel.
\item For multiple deletion channels, the error events can be categorized into two groups -- one where an input symbol is deleted in all the traces, and second, the complement of this event. This categorization results in a natural decomposition of multiple deletion channel model into a cascade model involving the remnant channel.
\item The remnant channel disregards the error events where a symbol is deleted in all the traces.
\item The edit graph provides a way to visualize all the possible error events and input sequences to a remnant channel given its outputs. 
\item The infiltration product serves the same purpose as the edit graph, but has an algebraic flavor and provides rigor for proofs and analyses. The edit graph, on the other hand, is more helpful in designing reconstruction algorithms over deletion channels.
\end{itemize}



==> Sections_revised/single_ML__Sundara_Rajan_s_conflicted_copy_2019-10-12_.tex <==


\section{Maximum likelihood for the single-trace deletion channel}
\label{sec:1deletion_ML}
Consider the ML formulation for the single-trace deletion channel given non-empty trace $Y$ and all possible $n$-length inputs allowed, restated here for convenience:
\begin{equation}
\argmax_{x\in \{0,1\}^n} {x \choose Y}.
\label{eq:1deletion_ML}
\end{equation}
To the best of our knowledge, the only known method to solve \eqref{eq:1deletion_ML} involves iterating over all possible choices of $x$ and computing the objective value for each of the choices. We here show that it is sufficient to solve a continuous relaxation of above problem to obtain a solution to \eqref{eq:1deletion_ML}. Note that there could be multiple solutions to \eqref{eq:1deletion_ML}. Before going in the main result, we first state a useful lemma which factors out a given coordinate $p_i$ out of $\mathbf F(p,Y)$. The proof of the lemma is relegated to the appendix.
\begin{restatable}{lemma}{deletionMLrellemma}
For $p=[p_1,p_2,..,p_i,...,p_n]$ and $Y=Y_1Y_2...Y_m$ with $n \geq m > 0$, we have
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
\label{lemma:F_decomposition}
\end{restatable}


\begin{theorem} An alternative optimization to characterize ML for the single-trace deletion channel.
\begin{equation}
\max_{x\in \{0,1\}^n} {x \choose Y} = \max_{p\in [0,1]^n} \mathbf F(p,Y).
\label{eq:ml_opt_equiv}
\end{equation}
Furthermore, given any non-integral $p^* \in [0,1]^n$ that maximizes $\mathbf F(p,Y)$, one could construct a corresponding integral solution $x^* \in \{0,1\}^n$ that maximizes $\mathbf F(p,Y)$ and consequently is also a solution to $\max_{x\in \{0,1\}^n} {x \choose Y}$.

\end{theorem}
\begin{proof}
As noted earlier, we have ${x \choose Y} = \mathbf F(x,Y)$. Therefore, we are interested in proving the following:
\begin{align*}
\max_{x\in \{0,1\}^n} \mathbf F(x,Y) \equiv \max_{p\in [0,1]^n} \mathbf F(p,Y).\numberthis
\label{eq:ml_opt_equiv_proof1}
\end{align*}
To show this and also the second statement, we prove that given $p=(p_1,p_2,...,p_i,...,p_n)$, at least one of the following holds true:
\begin{itemize}
\item$\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},0,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 0.
\item $\mathbf F(p^{(i\rightarrow 1)},Y) \geq \mathbf F(p,Y)$, where $p^{(i\rightarrow 0)}=(p_1,p_2,...,p_{i-1},1,p_{i+1}...,p_n)$ is the vector where the $i^{th}$ coordinate is replaced by 1.
\end{itemize}
Thus if $p^*$ is an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ with $p_i\in (0,1)$, then at least one of $p^{(i\rightarrow 0)}$ or $p^{(i\rightarrow 1)}$ is also an optimal solution. Sequentially applying this argument for each coordinate of $p$ shows that there exists a point in $\{0,1\}^n$ which is also an optimal solution to $\max_{p\in [0,1]^n} \mathbf F(p,Y)$ and consequently to $\max_{x\in \{0,1\}^n} \mathbf F(x,Y)$.

Now to prove our claim, we use Lemma~\ref{lemma:F_decomposition} to factor out $p_i$ terms in $\mathbf F(p,Y)$:
\begin{align*}
\mathbf F(p,Y) = \mathbf F( p_{[n]\backslash \{i\}},Y) +  p_i \sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})\\ + (1-p_i) \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).
\end{align*}
There are 3 cases
\begin{enumerate}
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) = \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) = \mathbf F(p,Y) = \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) > \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \leq \mathbf F(p,Y) \leq \mathbf F(p^{(i\rightarrow 1)},Y).$
\item $$\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}) < \sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$$ \\In this case it is easy to verify that $\mathbf F(p^{(i\rightarrow 0)},Y) \geq \mathbf F(p,Y) \geq \mathbf F(p^{(i\rightarrow 1)},Y).$
\end{enumerate}
Thus in each of the 3 cases, we see that at least one of $\mathbf F(p^{(i\rightarrow 0)},Y)$ or $\mathbf F(p^{(i\rightarrow 1)},Y)$ is at least as large as $\mathbf F(p,Y)$ thus proving the theorem. Note that the proof gives a natural way to find an optimal lattice point $p_{lattice}^*$ given a non-lattice point $p^*$ by iterating through each coordinate of $p^*$ and switching them to $0$ or $1$ by comparing $\sum\limits_{k|Y_k=1}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]})$ with $\sum\limits_{k|Y_k=0}\mathbf F( p_{[1:i-1]},  Y_{[1:k-1]})\mathbf F( p_{[i+1:n]},  Y_{[k+1,m]}).$
\end{proof}

